Posterior Cram\'er-Rao Bounds on Localization and Mapping Errors in Distributed MIMO SLAM

Radio-frequency simultaneous localization and mapping (RF-SLAM) methods jointly infer the position of mobile transmitters and receivers in wireless networks, together with a geometric map of the propagation environment. An inferred map of specular surfaces can be used to exploit non-line-of-sight components of the multipath channel to increase robustness, bypass obstructions, and improve overall communication and positioning performance. While performance bounds for user location are well established, the literature lacks performance bounds for map information. This paper derives the mapping error bound (MEB), i.e., the posterior Cram\'er-Rao lower bound on the position and orientation of specular surfaces, for RF-SLAM. In particular, we consider a very general scenario with single- and double-bounce reflections, as well as distributed anchors. We demonstrate numerically that a state-of-the-art RF-SLAM algorithm asymptotically converges to this MEB. The bounds assess not only the localization (position and orientation) but also the mapping performance of RF-SLAM algorithms in terms of global features.

==> IEEEabrv.tex <==
journal = IEEE_J_AC,
@STRING{IEEE_J_ANNE = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AES = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_AS = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL = "{IEEE} Trans. Mil. Electron."}
@STRING{IEEE_J_ITS = "{IEEE} Trans. Intell. Transp. Syst."}
@STRING{IEEE_J_IV = "{IEEE} Trans. Intell. Veh."}
@STRING{IEEE_J_TTE = "{IEEE} Trans. Transport. Electrific."}
@STRING{IEEE_J_VC = "{IEEE} Trans. Veh. Commun."}
@STRING{IEEE_J_VT = "{IEEE} Trans. Veh. Technol."}
@STRING{IEEE_J_STSP = "{IEEE} J. Sel. Topics Signal Process."}
@STRING{IEEE_J_SPL = "{IEEE} Signal Process. Lett."}
@STRING{IEEE_J_SYST = "{IEEE} Syst. J."}
@STRING{IEEE_J_ASSP = "{IEEE} Trans. Acoust., Speech, Signal Process."}
@STRING{IEEE_J_AU = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA = "{IEEE} Trans. Audio Electroacoust."}
@STRING{IEEE_J_ASLP = "{IEEE/ACM} Trans. Audio, Speech, Language Process."}
@STRING{IEEE_J_ASL = "{IEEE} Audio, Speech, Language Process."}
@STRING{IEEE_J_AC = "{IEEE} Trans. Autom. Control"}
@STRING{IEEE_J_CAS = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CASI_RP = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII_EB = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST = "{IEEE} Trans. Control Syst. Technol."}
@STRING{IEEE_J_ETCAS = "{IEEE} Trans. Emerg. Sel. Topics Circuits Syst."}
@STRING{IEEE_J_SP = "{IEEE} Trans. Signal Process."}
@STRING{IEEE_J_SU = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP = "{IEEE} Trans. Speech Audio Process."}
@STRING{IEEE_J_UE = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC = "{IEEE} Trans. Ultrason., Ferroelectr., Freq. Control"}
@STRING{IEEE_J_COML = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC = "{IEEE} J. Sel. Areas Commun."}
@STRING{IEEE_J_COM = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM = "{IEEE} Trans. Wireless Commun."}
@STRING{IEEE_J_WCOML = "{IEEE} Wireless Commun. Lett."}
@STRING{IEEE_J_ADVP = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT = "{IEEE} Trans. Compon., Hybrids, Manuf. Technol."}
@STRING{IEEE_J_CPMT = "{IEEE} Trans. Compon. Packag. Manuf. Technol."}
@STRING{IEEE_J_CPMTA = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {A}"}
@STRING{IEEE_J_CPMTB = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {B}"}
@STRING{IEEE_J_CPMTC = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {C}"}
@STRING{IEEE_J_CAPTS = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CAPT = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CPART = "{IEEE} Trans. Compon. Parts"}
@STRING{IEEE_J_EPM = "{IEEE} Trans. Electron. Packag. Manuf."}
@STRING{IEEE_J_MFT = "{IEEE} Trans. Manuf. Technol."}
@STRING{IEEE_J_PHP = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP = "{IEEE} Trans. Parts, Mater., Packag."}
@STRING{IEEE_J_TCAD = "{IEEE} J. Technol. Comput. Aided Design"}
@STRING{IEEE_J_CAD = "{IEEE} Trans. Comput.-Aided Design Integr. Circuits Syst."}
@STRING{IEEE_J_BD = "{IEEE} Trans. Big Data"}
@STRING{IEEE_J_IFS = "{IEEE} Trans. Inf. Forensics Security"}
@STRING{IEEE_J_IT = "{IEEE} Trans. Inf. Theory"}
@STRING{IEEE_J_KDE = "{IEEE} Trans. Knowl. Data Eng."}
@STRING{IEEE_J_CAL = "{IEEE} Comput. Archit. Lett."}
@STRING{IEEE_J_ES = "{IEEE} Embedded Syst. Lett."}
@STRING{IEEE_J_IOT = "{IEEE} Internet Things J."}
@STRING{IEEE_J_XCDC = "{IEEE} J. Explor. Solid-State Computat. Devices Circuits"}
@STRING{IEEE_J_MMCT = "{IEEE} J. Multiscale and Multiphys. Comput. Techn."}
@STRING{IEEE_J_SUSC = "{IEEE} Sustain. Comput."}
@STRING{IEEE_J_CC = "{IEEE} Trans. on Cloud Comput."}
@STRING{IEEE_J_CSS = "{IEEE} Trans. Comput. Social Syst."}
@STRING{IEEE_J_C = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_CNS = "{IEEE} Trans. Control Netw. Syst."}
@STRING{IEEE_J_DSC = "{IEEE} Trans. Depend. Sec. Comput."}
@STRING{IEEE_J_ECOMP = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_ETC = "{IEEE} Trans. Emerg. Topics Comput."}
@STRING{IEEE_J_EVC = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ = "{IEEE} Trans. Fuzzy Syst."}
@STRING{IEEE_J_MC = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_MSCS = "{IEEE} Trans. Multi-Scale Comput. Syst."}
@STRING{IEEE_J_NET = "{IEEE/ACM} Trans. Netw."}
@STRING{IEEE_J_NSE = "{IEEE} Trans. Netw. Sci. Eng."}
@STRING{IEEE_J_NSM = "{IEEE} Trans. Netw. Service Manag."}
@STRING{IEEE_J_NN = "{IEEE} Trans. Neural Netw."}
@STRING{IEEE_J_NNLS = "{IEEE} Trans. Neural Netw. Learn. Syst."}
@STRING{IEEE_J_PDS = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SC = "{IEEE} Trans. Serv. Comput."}
@STRING{IEEE_J_SIPN = "{IEEE} Trans. Signal Inf. Process. Netw."}
@STRING{IEEE_J_SE = "{IEEE} Trans. Softw. Eng."}
@STRING{IEEE_J_JDT = "{IEEE/OSA} J. Display Technol."}
@STRING{IEEE_J_IP = "{IEEE} Trans. Image Process."}
@STRING{IEEE_J_MM = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG = "{IEEE} Trans. Vis. Comput. Graphics"}
@STRING{IEEE_J_JAS = "{IEEE/CAA} J. Autom. Sinica"}
@STRING{IEEE_J_JRA = "{IEEE} J. Robot. Autom."}
@STRING{IEEE_J_AFFC = "{IEEE} Trans. Affect. Comput."}
@STRING{IEEE_J_ASE = "{IEEE} Trans. Autom. Sci. Eng."}
@STRING{IEEE_J_AMD = "{IEEE} Trans. Auton. Mental Develop."}
@STRING{IEEE_J_CCN = "{IEEE} Trans. on Cogn. Commun. Netw."}
@STRING{IEEE_J_CDS = "{IEEE} Trans. Cogn. Develop. Syst."}
@STRING{IEEE_J_CIAIG = "{IEEE} Trans. Comput. Intell. {AI} in Games"}
@STRING{IEEE_J_CYB = "{IEEE} Trans. Cybern."}
@STRING{IEEE_J_H = "{IEEE} Trans. Haptics"}
@STRING{IEEE_J_HFE = "{IEEE} Trans. Hum. Factors Electron."}
@STRING{IEEE_J_HMS = "{IEEE} Trans. Human-Mach. Syst."}
@STRING{IEEE_J_MMS = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
@STRING{IEEE_J_RA = "{IEEE} Trans. Robot. Autom."}
@STRING{IEEE_J_RAL = "{IEEE} Robot. Autom. Lett."}
@STRING{IEEE_J_RO = "{IEEE} Trans. Robot."}
@STRING{IEEE_J_SMC = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
@STRING{IEEE_J_SMCS = "{IEEE} Trans. Syst., Man, Cybern., Syst."}
@STRING{IEEE_J_SSC = "{IEEE} Trans. Syst. Sci. Cybern."}
@STRING{IEEE_J_GRSL = "{IEEE} Geosci. Remote Sens. Lett."}
@STRING{IEEE_J_GE = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS = "{IEEE} Trans. Geosci. Remote Sens."}
@STRING{IEEE_J_OE = "{IEEE} J. Ocean. Eng."}
@STRING{IEEE_J_STARS = "{IEEE} J. Sel. Topics Appl. Earth Observ. Remote Sens."}
@STRING{IEEE_J_CJECE = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC = "Proc. {IEEE}"}
@STRING{IEEE_J_RITA = "{IEEE} Revista Iberoamericana de Technolog{\'{i}}as del Aprendizaje"}
@STRING{IEEE_J_EDU = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM = "{IEEE} Trans. Eng. Manag."}
@STRING{IEEE_J_EWS = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_LT = "{IEEE} Trans. Learn. Technol."}
@STRING{IEEE_J_PC = "{IEEE} Trans. Prof. Commun."}
@STRING{IEEE_J_AWPL = "{IEEE} Antennas Wireless Propag. Lett."}
@STRING{IEEE_J_MAGL = "{IEEE} Magn. Lett."}
@STRING{IEEE_J_MGWL = "{IEEE} Microw. Guided Wave Lett."}
@STRING{IEEE_J_MWCL = "{IEEE} Microw. Wireless Compon. Lett."}
@STRING{IEEE_J_RFIC = "{IEEE} {RFIC} J."}
@STRING{IEEE_J_RFID = "{IEEE} {RFID} J."}
@STRING{IEEE_J_AP = "{IEEE} Trans. Antennas Propag."}
@STRING{IEEE_J_EMC = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT = "{IEEE} Trans. Microw. Theory Techn."}
@STRING{IEEE_J_RFI = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TTHZ = "{IEEE} Trans. {THz} Sci. Technol."}
@STRING{IEEE_J_TJMJ = "{IEEE} Transl. J. Magn. Jpn."}
@STRING{IEEE_J_PHOT = "{IEEE} J. Photovolt."}
@STRING{IEEE_J_PEL = "{IEEE} Power Electron. Lett."}
@STRING{IEEE_J_PETS = "{IEEE} Power Energy Technol. Syst. J."}
@STRING{IEEE_J_ESTPE = "{IEEE} Trans. Emerg. Sel. Topics Power Electron."}
@STRING{IEEE_J_EC = "{IEEE} Trans. Energy Convers."}
@STRING{IEEE_J_PWRAS = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD = "{IEEE} Trans. Power Del."}
@STRING{IEEE_J_PWRE = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS = "{IEEE} Trans. Power Syst."}
@STRING{IEEE_J_SG = "{IEEE} Trans. Smart Grid"}
@STRING{IEEE_J_STE = "{IEEE} Trans. Sustain. Energy"}
@STRING{IEEE_J_PSE = "{IEEE} J. Product Safety Eng."}
@STRING{IEEE_J_APPIND = "{IEEE} Trans. Appl. Ind."}
@STRING{IEEE_J_BC = "{IEEE} Trans. Broadcast."}
@STRING{IEEE_J_BCTV = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE = "{IEEE} Trans. Consum. Electron."}
@STRING{IEEE_J_IE = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA = "{IEEE} Trans. Ind. Appl."}
@STRING{IEEE_J_IGA = "{IEEE} Trans. Ind. Gen. Appl."}
@STRING{IEEE_J_IINF = "{IEEE} Trans. Ind. Informat."}
@STRING{IEEE_J_IM = "{IEEE} Trans. Instrum. Meas."}
@STRING{IEEE_J_JEM = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI = "{IEEE} Trans. Dielectr. Electr. Insul."}
@STRING{IEEE_J_EI = "{IEEE} Trans. Electr. Insul."}
@STRING{IEEE_J_MEMS = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MEMSI = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MECH = "{IEEE/ASME} Trans. Mechatronics"}
@STRING{IEEE_J_BHI = "{IEEE} J. Biomed. Health Inform."}
@STRING{IEEE_J_TEHM = "{IEEE} J. Transl. Eng. Health Med."}
@STRING{IEEE_J_LS = "{IEEE} Life Sci. Lett."}
@STRING{IEEE_J_RBME = "{IEEE} Rev. Biomed. Eng."}
@STRING{IEEE_J_BCAS = "{IEEE} Trans. Biomed. Circuits Syst."}
@STRING{IEEE_J_BMELC = "{IEEE} Trans. Bio-Med. Electron."}
@STRING{IEEE_J_BME = "{IEEE} Trans. Biomed. Eng."}
@STRING{IEEE_J_B-ME = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_CBB = "{IEEE/ACM} Trans. Comput. Biol. Bioinformatics"}
@STRING{IEEE_J_ITBM = "{IEEE} Trans. Inf. Technol. Biomed."}
@STRING{IEEE_J_ME = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI = "{IEEE} Trans. Med. Imag."}
@STRING{IEEE_J_MBSC = "{IEEE} Trans. Mol. Biol. Multi-Scale Commun."}
@STRING{IEEE_J_NB = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE = "{IEEE} Trans. Neural Syst. Rehabil. Eng."}
@STRING{IEEE_J_RE = "{IEEE} Trans. Rehabil. Eng."}
@STRING{IEEE_J_JLT = "J. Lightw. Technol."}
@STRING{IEEE_J_OCN = "{IEEE} J. Opt. Commun. Netw."}
@STRING{IEEE_J_PJ = "{IEEE} Photon. J."}
@STRING{IEEE_J_PTL = "{IEEE} Photon. Technol. Lett."}
@STRING{IEEE_J_EDL = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_EDS = "{IEEE} J. Electron Devices Soc."}
@STRING{IEEE_J_JQE = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE = "{IEEE} J. Sel. Topics Quantum Electron."}
@STRING{IEEE_J_ENANO = "{IEEE} Nanotechnol. Express"}
@STRING{IEEE_J_ED = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS = "{IEEE} Trans. Plasma Sci."}
@STRING{IEEE_J_DMR = "{IEEE} Trans. Device Mater. Rel."}
@STRING{IEEE_J_R = "{IEEE} Trans. Rel."}
@STRING{IEEE_J_ESSL = "{IEEE/ECS} Electrochem. Solid-State Lett."}
@STRING{IEEE_J_JSSC = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC = "{IEEE} Trans. Appl. Supercond."}
@STRING{IEEE_J_SM = "{IEEE} Trans. Semicond. Manuf."}
@STRING{IEEE_J_SENSOR = "{IEEE} Sensors J."}
@STRING{IEEE_J_VLSI = "{IEEE} Trans. {VLSI} Syst."}
@STRING{IEEE_O_ACC = "{IEEE} Access"}
@STRING{IEEE_M_AES = "{IEEE} Aerosp. Electron. Syst. Mag."}
@STRING{IEEE_M_HIST = "{IEEE} Ann. Hist. Comput."}
@STRING{IEEE_M_AP = "{IEEE} Antennas Propag. Mag."}
@STRING{IEEE_M_ASSP = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CHINAC = "China Commun."}
@STRING{IEEE_M_CD = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC = "{IEEE} Commun. Soc. Mag."}
@STRING{IEEE_O_CSTO = "{IEEE} Commun. Surveys Tuts."}
@STRING{IEEE_M_CIM = "{IEEE} Comput. Intell. Mag."}
@STRING{IEEE_M_CSE = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C = "Computer"}
@STRING{IEEE_M_CAP = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS = "{IEEE} Control Syst. Mag."}
@STRING{IEEE_M_DT = "{IEEE} Des. Test"}
@STRING{IEEE_M_DTC = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_O_DSO = "{IEEE} Distrib. Syst. Online"}
@STRING{IEEE_M_EI = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_ETF = "{IEEE} Electrific. Mag."}
@STRING{IEEE_M_EMC = "{IEEE} Electromagn. Compat."}
@STRING{IEEE_M_ETR = "{IEEE} ElectroTechnol. Rev."}
@STRING{IEEE_M_EMR = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EMB = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EXP = "{IEEE} Expert"}
@STRING{IEEE_M_GRS = "{IEEE} Geosci. Remote Sens. Mag."}
@STRING{IEEE_M_IA = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IE = "{IEEE} Ind. Electron. Mag."}
@STRING{IEEE_M_IM = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_ITS = "{IEEE} Intell. Transp. Syst. Mag."}
@STRING{IEEE_M_IC = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO = "{IEEE} Micro"}
@STRING{IEEE_M_MW = "{IEEE} Microw. Mag."}
@STRING{IEEE_M_MM = "{IEEE} Multimedia"}
@STRING{IEEE_M_NANO = "{IEEE} Nanotechnol. Mag."}
@STRING{IEEE_M_NET = "{IEEE} Netw."}
@STRING{IEEE_M_PCOM = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_PVC = "{IEEE} Pervasive Comput."}
@STRING{IEEE_M_POT = "{IEEE} Potentials"}
@STRING{IEEE_M_PEL = "{IEEE} Power Electron. Mag."}
@STRING{IEEE_M_PE = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_PULSE = "{IEEE} Pulse"}
@STRING{IEEE_M_RA = "{IEEE} Robot. Autom. Mag."}
@STRING{IEEE_M_SAP = "{IEEE} Security Privacy"}
@STRING{IEEE_M_SP = "{IEEE} Signal Process. Mag."}
@STRING{IEEE_M_S = "{IEEE} Softw."}
@STRING{IEEE_M_SSC = "{IEEE} Solid-State Circuits Mag."}
@STRING{IEEE_M_SPECT = "{IEEE} Spectr."}
@STRING{IEEE_M_SMC = "{IEEE} Syst., Man, Cybern. Mag."}
@STRING{IEEE_M_TS = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_VT = "{IEEE} Veh. Technol. Mag."}
@STRING{IEEE_M_WC = "{IEEE} Wireless Commun."}
@STRING{IEEE_M_TODAY = "Today's Engineer"}


==> figures/Journal_array_agent_18.tex <==
\tikzstyle{arrayBlue}=[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round];
\tikzstyle{arrayOrange}=[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round];

%  ---------- PM - step 18 ----------

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.68217261904762	6.99217261904762\\
1.33782738095238	6.99217261904762\\
1.33782738095238	6.64782738095238\\
1.68217261904762	6.64782738095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.68217261904762	6.99217261904762\\
1.33782738095238	6.99217261904762\\
1.33782738095238	6.64782738095238\\
1.68217261904762	6.64782738095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.68217261904762	6.99217261904762\\
1.33782738095238	6.99217261904762\\
1.33782738095238	6.99217261904762\\
1.68217261904762	6.99217261904762\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.68217261904762	6.64782738095238\\
1.33782738095238	6.64782738095238\\
1.33782738095238	6.64782738095238\\
1.68217261904762	6.64782738095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.68217261904762	6.99217261904762\\
1.68217261904762	6.64782738095238\\
1.68217261904762	6.64782738095238\\
1.68217261904762	6.99217261904762\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.33782738095238	6.99217261904762\\
1.33782738095238	6.64782738095238\\
1.33782738095238	6.64782738095238\\
1.33782738095238	6.99217261904762\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.65136904761905	6.96136904761905\\
1.60672619047619	6.96136904761905\\
1.60672619047619	6.91672619047619\\
1.65136904761905	6.91672619047619\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.59184523809524	6.96136904761905\\
1.54720238095238	6.96136904761905\\
1.54720238095238	6.91672619047619\\
1.59184523809524	6.91672619047619\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.53232142857143	6.96136904761905\\
1.48767857142857	6.96136904761905\\
1.48767857142857	6.91672619047619\\
1.53232142857143	6.91672619047619\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.47279761904762	6.96136904761905\\
1.42815476190476	6.96136904761905\\
1.42815476190476	6.91672619047619\\
1.47279761904762	6.91672619047619\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.41327380952381	6.96136904761905\\
1.36863095238095	6.96136904761905\\
1.36863095238095	6.91672619047619\\
1.41327380952381	6.91672619047619\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.65136904761905	6.90184523809524\\
1.60672619047619	6.90184523809524\\
1.60672619047619	6.85720238095238\\
1.65136904761905	6.85720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.59184523809524	6.90184523809524\\
1.54720238095238	6.90184523809524\\
1.54720238095238	6.85720238095238\\
1.59184523809524	6.85720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.53232142857143	6.90184523809524\\
1.48767857142857	6.90184523809524\\
1.48767857142857	6.85720238095238\\
1.53232142857143	6.85720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.47279761904762	6.90184523809524\\
1.42815476190476	6.90184523809524\\
1.42815476190476	6.85720238095238\\
1.47279761904762	6.85720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.41327380952381	6.90184523809524\\
1.36863095238095	6.90184523809524\\
1.36863095238095	6.85720238095238\\
1.41327380952381	6.85720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.65136904761905	6.84232142857143\\
1.60672619047619	6.84232142857143\\
1.60672619047619	6.79767857142857\\
1.65136904761905	6.79767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.59184523809524	6.84232142857143\\
1.54720238095238	6.84232142857143\\
1.54720238095238	6.79767857142857\\
1.59184523809524	6.79767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.53232142857143	6.84232142857143\\
1.48767857142857	6.84232142857143\\
1.48767857142857	6.79767857142857\\
1.53232142857143	6.79767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.47279761904762	6.84232142857143\\
1.42815476190476	6.84232142857143\\
1.42815476190476	6.79767857142857\\
1.47279761904762	6.79767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.41327380952381	6.84232142857143\\
1.36863095238095	6.84232142857143\\
1.36863095238095	6.79767857142857\\
1.41327380952381	6.79767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.65136904761905	6.78279761904762\\
1.60672619047619	6.78279761904762\\
1.60672619047619	6.73815476190476\\
1.65136904761905	6.73815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.59184523809524	6.78279761904762\\
1.54720238095238	6.78279761904762\\
1.54720238095238	6.73815476190476\\
1.59184523809524	6.73815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.53232142857143	6.78279761904762\\
1.48767857142857	6.78279761904762\\
1.48767857142857	6.73815476190476\\
1.53232142857143	6.73815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.47279761904762	6.78279761904762\\
1.42815476190476	6.78279761904762\\
1.42815476190476	6.73815476190476\\
1.47279761904762	6.73815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.41327380952381	6.78279761904762\\
1.36863095238095	6.78279761904762\\
1.36863095238095	6.73815476190476\\
1.41327380952381	6.73815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.65136904761905	6.72327380952381\\
1.60672619047619	6.72327380952381\\
1.60672619047619	6.67863095238095\\
1.65136904761905	6.67863095238095\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.59184523809524	6.72327380952381\\
1.54720238095238	6.72327380952381\\
1.54720238095238	6.67863095238095\\
1.59184523809524	6.67863095238095\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.53232142857143	6.72327380952381\\
1.48767857142857	6.72327380952381\\
1.48767857142857	6.67863095238095\\
1.53232142857143	6.67863095238095\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.47279761904762	6.72327380952381\\
1.42815476190476	6.72327380952381\\
1.42815476190476	6.67863095238095\\
1.47279761904762	6.67863095238095\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
1.41327380952381	6.72327380952381\\
1.36863095238095	6.72327380952381\\
1.36863095238095	6.67863095238095\\
1.41327380952381	6.67863095238095\\
}--cycle;




















%\addplot [-stealth, color=mycolor2x, line width=0.301pt,line cap = round, line join = round,%
%{-Stealth[inset=0pt, scale=0.6, angle'=25]}
%]  table[row sep=crcr]{%
%1.2201	6.8101\\
%0.7701	6.8101\\
%};


\addplot [-stealth, color=mycolor1, line width=0.301pt,line cap = round, line join = round,%
{-Stealth[inset=0pt, scale=0.6, angle'=25]}
]  table[row sep=crcr]{%
1.5101	6.8201\\
1.0601	6.8201\\
};






==> figures/Journal_array_agent_28.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%


%  ---------- PM - step 28 ----------



\addplot[area legend, line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.33264880952381	6.92264880952381\\
1.10735119047619	6.92264880952381\\
1.10735119047619	6.69735119047619\\
1.33264880952381	6.69735119047619\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.33264880952381	6.92264880952381\\
1.10735119047619	6.92264880952381\\
1.10735119047619	6.69735119047619\\
1.33264880952381	6.69735119047619\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.33264880952381	6.92264880952381\\
1.10735119047619	6.92264880952381\\
1.10735119047619	6.92264880952381\\
1.33264880952381	6.92264880952381\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.33264880952381	6.69735119047619\\
1.10735119047619	6.69735119047619\\
1.10735119047619	6.69735119047619\\
1.33264880952381	6.69735119047619\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.33264880952381	6.92264880952381\\
1.33264880952381	6.69735119047619\\
1.33264880952381	6.69735119047619\\
1.33264880952381	6.92264880952381\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.10735119047619	6.92264880952381\\
1.10735119047619	6.69735119047619\\
1.10735119047619	6.69735119047619\\
1.10735119047619	6.92264880952381\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.18279761904762	6.89184523809524\\
1.13815476190476	6.89184523809524\\
1.13815476190476	6.84720238095238\\
1.18279761904762	6.84720238095238\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.18279761904762	6.83232142857143\\
1.13815476190476	6.83232142857143\\
1.13815476190476	6.78767857142857\\
1.18279761904762	6.78767857142857\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.18279761904762	6.77279761904762\\
1.13815476190476	6.77279761904762\\
1.13815476190476	6.72815476190476\\
1.18279761904762	6.72815476190476\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.24232142857143	6.89184523809524\\
1.19767857142857	6.89184523809524\\
1.19767857142857	6.84720238095238\\
1.24232142857143	6.84720238095238\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.24232142857143	6.83232142857143\\
1.19767857142857	6.83232142857143\\
1.19767857142857	6.78767857142857\\
1.24232142857143	6.78767857142857\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.24232142857143	6.77279761904762\\
1.19767857142857	6.77279761904762\\
1.19767857142857	6.72815476190476\\
1.24232142857143	6.72815476190476\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.30184523809524	6.89184523809524\\
1.25720238095238	6.89184523809524\\
1.25720238095238	6.84720238095238\\
1.30184523809524	6.84720238095238\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.30184523809524	6.83232142857143\\
1.25720238095238	6.83232142857143\\
1.25720238095238	6.78767857142857\\
1.30184523809524	6.78767857142857\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.30184523809524	6.77279761904762\\
1.25720238095238	6.77279761904762\\
1.25720238095238	6.72815476190476\\
1.30184523809524	6.72815476190476\\
}--cycle;


%\addplot [-stealth, color=mycolor2x, line width=0.301pt,line cap = round, line join = round,%
%{-Stealth[inset=0pt, scale=0.6, angle'=25]}
%]  table[row sep=crcr]{%
%1.2201	6.8101\\
%0.7701	6.8101\\
%};

\addplot [-stealth, color=mycolor2x, line width=0.301pt,line cap = round, line join = round,%
{-Stealth[inset=0pt, scale=0.6, angle'=25]}
]  table[row sep=crcr]{%
1.2201	6.8101\\
1.2201	6.3601\\
};









%  ---------- PM - step 28 ----------




\addplot[area legend, line width=0.151pt, draw=gray, fill=gray!50!white, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.80134707907626	0.676161894350224\\
1.99453810564978	0.56024707907626\\
2.11045292092374	0.753438105649776\\
1.91726189435022	0.86935292092374\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=gray, fill=gray!50!white, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.80134707907626	0.676161894350224\\
1.99453810564978	0.56024707907626\\
2.11045292092374	0.753438105649776\\
1.91726189435022	0.86935292092374\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=gray, fill=gray!50!white, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.80134707907626	0.676161894350224\\
1.99453810564978	0.56024707907626\\
1.99453810564978	0.56024707907626\\
1.80134707907626	0.676161894350224\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=gray, fill=gray!50!white, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.91726189435022	0.86935292092374\\
2.11045292092374	0.753438105649776\\
2.11045292092374	0.753438105649776\\
1.91726189435022	0.86935292092374\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=gray, fill=gray!50!white, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.80134707907626	0.676161894350224\\
1.91726189435022	0.86935292092374\\
1.91726189435022	0.86935292092374\\
1.80134707907626	0.676161894350224\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=gray, fill=gray!50!white, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.99453810564978	0.56024707907626\\
2.11045292092374	0.753438105649776\\
2.11045292092374	0.753438105649776\\
1.99453810564978	0.56024707907626\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.94569168311935	0.625477827982877\\
1.98397259987764	0.602509238430572\\
2.00694118942995	0.640790155188865\\
1.96866027267166	0.663758744741169\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.97631646918909	0.676519050327267\\
2.01459738594738	0.653550460774962\\
2.03756597549969	0.691831377533255\\
1.9992850587414	0.714799967085559\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
2.00694125525883	0.727560272671657\\
2.04522217201712	0.704591683119352\\
2.06819076156943	0.742872599877645\\
2.02990984481114	0.765841189429949\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.89465046077496	0.656102614052616\\
1.93293137753325	0.633134024500312\\
1.95589996708556	0.671414941258604\\
1.91761905032727	0.694383530810908\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.9252752468447	0.707143836397006\\
1.96355616360299	0.684175246844702\\
1.9865247531553	0.722456163602994\\
1.94824383639701	0.745424753155298\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.95590003291444	0.758185058741396\\
1.99418094967273	0.735216469189092\\
2.01714953922504	0.773497385947384\\
1.97886862246675	0.796465975499688\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.84360923843057	0.686727400122355\\
1.88189015518886	0.663758810570051\\
1.90485874474117	0.702039727328343\\
1.86657782798288	0.725008316880648\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.87423402450031	0.737768622466745\\
1.9125149412586	0.714800032914441\\
1.93548353081091	0.753080949672733\\
1.89720261405262	0.776049539225038\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.90485881057005	0.788809844811135\\
1.94313972732834	0.765841255258831\\
1.96610831688065	0.804122172017123\\
1.92782740012236	0.827090761569428\\
}--cycle;
\addplot [-stealth, color=gray!50!white, line width=0.301pt,line cap = round, line join = round,%
{-Stealth[inset=0pt, scale=0.6, angle'=25]}
]  table[row sep=crcr]{%
1.956	0.7149\\
2.34187164092359	0.483376617312771\\
};


==> figures/Journal_array_agent_334.tex <==

%  ---------- PM - step 334 ----------




\addplot[area legend, line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.80134707907626	0.676161894350224\\
1.99453810564978	0.56024707907626\\
2.11045292092374	0.753438105649776\\
1.91726189435022	0.86935292092374\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.80134707907626	0.676161894350224\\
1.99453810564978	0.56024707907626\\
2.11045292092374	0.753438105649776\\
1.91726189435022	0.86935292092374\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.80134707907626	0.676161894350224\\
1.99453810564978	0.56024707907626\\
1.99453810564978	0.56024707907626\\
1.80134707907626	0.676161894350224\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.91726189435022	0.86935292092374\\
2.11045292092374	0.753438105649776\\
2.11045292092374	0.753438105649776\\
1.91726189435022	0.86935292092374\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.80134707907626	0.676161894350224\\
1.91726189435022	0.86935292092374\\
1.91726189435022	0.86935292092374\\
1.80134707907626	0.676161894350224\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.99453810564978	0.56024707907626\\
2.11045292092374	0.753438105649776\\
2.11045292092374	0.753438105649776\\
1.99453810564978	0.56024707907626\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.94569168311935	0.625477827982877\\
1.98397259987764	0.602509238430572\\
2.00694118942995	0.640790155188865\\
1.96866027267166	0.663758744741169\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.97631646918909	0.676519050327267\\
2.01459738594738	0.653550460774962\\
2.03756597549969	0.691831377533255\\
1.9992850587414	0.714799967085559\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
2.00694125525883	0.727560272671657\\
2.04522217201712	0.704591683119352\\
2.06819076156943	0.742872599877645\\
2.02990984481114	0.765841189429949\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.89465046077496	0.656102614052616\\
1.93293137753325	0.633134024500312\\
1.95589996708556	0.671414941258604\\
1.91761905032727	0.694383530810908\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.9252752468447	0.707143836397006\\
1.96355616360299	0.684175246844702\\
1.9865247531553	0.722456163602994\\
1.94824383639701	0.745424753155298\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.95590003291444	0.758185058741396\\
1.99418094967273	0.735216469189092\\
2.01714953922504	0.773497385947384\\
1.97886862246675	0.796465975499688\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.84360923843057	0.686727400122355\\
1.88189015518886	0.663758810570051\\
1.90485874474117	0.702039727328343\\
1.86657782798288	0.725008316880648\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.87423402450031	0.737768622466745\\
1.9125149412586	0.714800032914441\\
1.93548353081091	0.753080949672733\\
1.89720261405262	0.776049539225038\\
}--cycle;

\addplot[area legend, line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round,forget plot]
table[row sep=crcr] {%
x	y\\
1.90485881057005	0.788809844811135\\
1.94313972732834	0.765841255258831\\
1.96610831688065	0.804122172017123\\
1.92782740012236	0.827090761569428\\
}--cycle;
\addplot [-stealth, color=mycolor2x, line width=0.301pt,line cap = round, line join = round,%
{-Stealth[inset=0pt, scale=0.6, angle'=25]}
]  table[row sep=crcr]{%
1.956	0.7149\\
2.34187164092359	0.483376617312771\\
};


==> figures/Journal_arrays_only.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%








%  ---------- PA1 ----------
\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.327827380952381	5.82782738095238\\
-0.327827380952381	6.17217261904762\\
-0.672172619047619	6.17217261904762\\
-0.672172619047619	5.82782738095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.327827380952381	5.82782738095238\\
-0.327827380952381	6.17217261904762\\
-0.672172619047619	6.17217261904762\\
-0.672172619047619	5.82782738095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.327827380952381	5.82782738095238\\
-0.327827380952381	6.17217261904762\\
-0.327827380952381	6.17217261904762\\
-0.327827380952381	5.82782738095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.672172619047619	5.82782738095238\\
-0.672172619047619	6.17217261904762\\
-0.672172619047619	6.17217261904762\\
-0.672172619047619	5.82782738095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.327827380952381	5.82782738095238\\
-0.672172619047619	5.82782738095238\\
-0.672172619047619	5.82782738095238\\
-0.327827380952381	5.82782738095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.327827380952381	6.17217261904762\\
-0.672172619047619	6.17217261904762\\
-0.672172619047619	6.17217261904762\\
-0.327827380952381	6.17217261904762\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.358630952380952	5.85863095238095\\
-0.358630952380952	5.90327380952381\\
-0.40327380952381	5.90327380952381\\
-0.40327380952381	5.85863095238095\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.358630952380952	5.91815476190476\\
-0.358630952380952	5.96279761904762\\
-0.40327380952381	5.96279761904762\\
-0.40327380952381	5.91815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.358630952380952	5.97767857142857\\
-0.358630952380952	6.02232142857143\\
-0.40327380952381	6.02232142857143\\
-0.40327380952381	5.97767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.358630952380952	6.03720238095238\\
-0.358630952380952	6.08184523809524\\
-0.40327380952381	6.08184523809524\\
-0.40327380952381	6.03720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.358630952380952	6.09672619047619\\
-0.358630952380952	6.14136904761905\\
-0.403273809523809	6.14136904761905\\
-0.403273809523809	6.09672619047619\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.418154761904762	5.85863095238095\\
-0.418154761904762	5.90327380952381\\
-0.462797619047619	5.90327380952381\\
-0.462797619047619	5.85863095238095\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.418154761904762	5.91815476190476\\
-0.418154761904762	5.96279761904762\\
-0.462797619047619	5.96279761904762\\
-0.462797619047619	5.91815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.418154761904762	5.97767857142857\\
-0.418154761904762	6.02232142857143\\
-0.462797619047619	6.02232142857143\\
-0.462797619047619	5.97767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.418154761904762	6.03720238095238\\
-0.418154761904762	6.08184523809524\\
-0.462797619047619	6.08184523809524\\
-0.462797619047619	6.03720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.418154761904762	6.09672619047619\\
-0.418154761904762	6.14136904761905\\
-0.462797619047619	6.14136904761905\\
-0.462797619047619	6.09672619047619\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.477678571428571	5.85863095238095\\
-0.477678571428571	5.90327380952381\\
-0.522321428571429	5.90327380952381\\
-0.522321428571429	5.85863095238095\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.477678571428571	5.91815476190476\\
-0.477678571428571	5.96279761904762\\
-0.522321428571429	5.96279761904762\\
-0.522321428571429	5.91815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.477678571428571	5.97767857142857\\
-0.477678571428571	6.02232142857143\\
-0.522321428571429	6.02232142857143\\
-0.522321428571429	5.97767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.477678571428571	6.03720238095238\\
-0.477678571428571	6.08184523809524\\
-0.522321428571429	6.08184523809524\\
-0.522321428571429	6.03720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.477678571428571	6.09672619047619\\
-0.477678571428571	6.14136904761905\\
-0.522321428571429	6.14136904761905\\
-0.522321428571429	6.09672619047619\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.537202380952381	5.85863095238095\\
-0.537202380952381	5.90327380952381\\
-0.581845238095238	5.90327380952381\\
-0.581845238095238	5.85863095238095\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.537202380952381	5.91815476190476\\
-0.537202380952381	5.96279761904762\\
-0.581845238095238	5.96279761904762\\
-0.581845238095238	5.91815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.537202380952381	5.97767857142857\\
-0.537202380952381	6.02232142857143\\
-0.581845238095238	6.02232142857143\\
-0.581845238095238	5.97767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.537202380952381	6.03720238095238\\
-0.537202380952381	6.08184523809524\\
-0.581845238095238	6.08184523809524\\
-0.581845238095238	6.03720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.537202380952381	6.09672619047619\\
-0.537202380952381	6.14136904761905\\
-0.581845238095238	6.14136904761905\\
-0.581845238095238	6.09672619047619\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.59672619047619	5.85863095238095\\
-0.59672619047619	5.90327380952381\\
-0.641369047619048	5.90327380952381\\
-0.641369047619048	5.85863095238095\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.59672619047619	5.91815476190476\\
-0.59672619047619	5.96279761904762\\
-0.641369047619048	5.96279761904762\\
-0.641369047619048	5.91815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.59672619047619	5.97767857142857\\
-0.59672619047619	6.02232142857143\\
-0.641369047619048	6.02232142857143\\
-0.641369047619048	5.97767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.59672619047619	6.03720238095238\\
-0.59672619047619	6.08184523809524\\
-0.641369047619048	6.08184523809524\\
-0.641369047619048	6.03720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
-0.59672619047619	6.09672619047619\\
-0.59672619047619	6.14136904761905\\
-0.641369047619048	6.14136904761905\\
-0.641369047619048	6.09672619047619\\
}--cycle;



\addplot [-stealth, color=mycolor2x, line width=0.301pt,line cap = round, line join = round,%
{-Stealth[inset=0pt, scale=0.6, angle'=25]}
]
  table[row sep=crcr]{%
-0.4999	6.0001\\
-0.4999	6.4501\\
};
















%  ---------- PA2 ----------

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.37217261904762	1.12782738095238\\
4.37217261904762	1.47217261904762\\
4.02782738095238	1.47217261904762\\
4.02782738095238	1.12782738095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.37217261904762	1.12782738095238\\
4.37217261904762	1.47217261904762\\
4.02782738095238	1.47217261904762\\
4.02782738095238	1.12782738095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.37217261904762	1.12782738095238\\
4.37217261904762	1.47217261904762\\
4.37217261904762	1.47217261904762\\
4.37217261904762	1.12782738095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.02782738095238	1.12782738095238\\
4.02782738095238	1.47217261904762\\
4.02782738095238	1.47217261904762\\
4.02782738095238	1.12782738095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.37217261904762	1.12782738095238\\
4.02782738095238	1.12782738095238\\
4.02782738095238	1.12782738095238\\
4.37217261904762	1.12782738095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor1, fill=mycolor2, fill opacity=0.3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.37217261904762	1.47217261904762\\
4.02782738095238	1.47217261904762\\
4.02782738095238	1.47217261904762\\
4.37217261904762	1.47217261904762\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.34136904761905	1.15863095238095\\
4.34136904761905	1.20327380952381\\
4.29672619047619	1.20327380952381\\
4.29672619047619	1.15863095238095\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.34136904761905	1.21815476190476\\
4.34136904761905	1.26279761904762\\
4.29672619047619	1.26279761904762\\
4.29672619047619	1.21815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.34136904761905	1.27767857142857\\
4.34136904761905	1.32232142857143\\
4.29672619047619	1.32232142857143\\
4.29672619047619	1.27767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.34136904761905	1.33720238095238\\
4.34136904761905	1.38184523809524\\
4.29672619047619	1.38184523809524\\
4.29672619047619	1.33720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.34136904761905	1.39672619047619\\
4.34136904761905	1.44136904761905\\
4.29672619047619	1.44136904761905\\
4.29672619047619	1.39672619047619\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.28184523809524	1.15863095238095\\
4.28184523809524	1.20327380952381\\
4.23720238095238	1.20327380952381\\
4.23720238095238	1.15863095238095\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.28184523809524	1.21815476190476\\
4.28184523809524	1.26279761904762\\
4.23720238095238	1.26279761904762\\
4.23720238095238	1.21815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.28184523809524	1.27767857142857\\
4.28184523809524	1.32232142857143\\
4.23720238095238	1.32232142857143\\
4.23720238095238	1.27767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.28184523809524	1.33720238095238\\
4.28184523809524	1.38184523809524\\
4.23720238095238	1.38184523809524\\
4.23720238095238	1.33720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.28184523809524	1.39672619047619\\
4.28184523809524	1.44136904761905\\
4.23720238095238	1.44136904761905\\
4.23720238095238	1.39672619047619\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.22232142857143	1.15863095238095\\
4.22232142857143	1.20327380952381\\
4.17767857142857	1.20327380952381\\
4.17767857142857	1.15863095238095\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.22232142857143	1.21815476190476\\
4.22232142857143	1.26279761904762\\
4.17767857142857	1.26279761904762\\
4.17767857142857	1.21815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.22232142857143	1.27767857142857\\
4.22232142857143	1.32232142857143\\
4.17767857142857	1.32232142857143\\
4.17767857142857	1.27767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.22232142857143	1.33720238095238\\
4.22232142857143	1.38184523809524\\
4.17767857142857	1.38184523809524\\
4.17767857142857	1.33720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.22232142857143	1.39672619047619\\
4.22232142857143	1.44136904761905\\
4.17767857142857	1.44136904761905\\
4.17767857142857	1.39672619047619\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.16279761904762	1.15863095238095\\
4.16279761904762	1.20327380952381\\
4.11815476190476	1.20327380952381\\
4.11815476190476	1.15863095238095\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.16279761904762	1.21815476190476\\
4.16279761904762	1.26279761904762\\
4.11815476190476	1.26279761904762\\
4.11815476190476	1.21815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.16279761904762	1.27767857142857\\
4.16279761904762	1.32232142857143\\
4.11815476190476	1.32232142857143\\
4.11815476190476	1.27767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.16279761904762	1.33720238095238\\
4.16279761904762	1.38184523809524\\
4.11815476190476	1.38184523809524\\
4.11815476190476	1.33720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.16279761904762	1.39672619047619\\
4.16279761904762	1.44136904761905\\
4.11815476190476	1.44136904761905\\
4.11815476190476	1.39672619047619\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.10327380952381	1.15863095238095\\
4.10327380952381	1.20327380952381\\
4.05863095238095	1.20327380952381\\
4.05863095238095	1.15863095238095\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.10327380952381	1.21815476190476\\
4.10327380952381	1.26279761904762\\
4.05863095238095	1.26279761904762\\
4.05863095238095	1.21815476190476\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.10327380952381	1.27767857142857\\
4.10327380952381	1.32232142857143\\
4.05863095238095	1.32232142857143\\
4.05863095238095	1.27767857142857\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.10327380952381	1.33720238095238\\
4.10327380952381	1.38184523809524\\
4.05863095238095	1.38184523809524\\
4.05863095238095	1.33720238095238\\
}--cycle;

\addplot[line width=0.151pt, draw=mycolor3, fill=white!50!mycolor3, line cap = round, line join = round]
table[row sep=crcr] {%
x	y\\
4.10327380952381	1.39672619047619\\
4.10327380952381	1.44136904761905\\
4.05863095238095	1.44136904761905\\
4.05863095238095	1.39672619047619\\
}--cycle;

\addplot [-stealth, color=mycolor2x, line width=0.301pt,line cap = round, line join = round,%
{-Stealth[inset=0pt, scale=0.6, angle'=25]}
]
  table[row sep=crcr]{%
4.2001	1.3001\\
4.2001	1.7501\\
};




















==> figures/MVA-5-subplots/MVA-5plot-s1.tex <==


\addplot [color=IEEEgreen, dashed, line width=\LWestimates]
  table[row sep=crcr]{%
1	490.818588220251\\
2	263.682972151982\\
3	238.176494232264\\
4	242.975273987295\\
5	89.7737843093552\\
6	83.1848559959014\\
7	81.3475796236502\\
8	57.8838564358713\\
9	57.90566340377\\
10	9.79748049870281\\
11	70.5701562385537\\
12	13.6137906375741\\
13	15.9069450464689\\
14	28.9231688119614\\
15	25.4087444752226\\
16	25.9795439350155\\
17	26.5016068052685\\
18	24.5501677965706\\
19	22.4359108747521\\
20	21.1761928333771\\
21	19.8187655923645\\
22	18.5410614124152\\
23	17.0415671919311\\
24	15.889474434115\\
25	15.078686472126\\
26	13.5618984389968\\
27	12.4828280225103\\
28	11.8993291776803\\
29	10.9690454999521\\
30	10.3238127721644\\
31	9.71455675593258\\
32	8.42349781650561\\
33	8.46006130843461\\
34	8.006139771324\\
35	7.61033504344111\\
36	7.44005457899478\\
37	6.80431697514945\\
38	6.4038885958798\\
39	6.30761734458878\\
40	6.31358600813808\\
41	6.5333621929981\\
42	5.57406163155376\\
43	5.78696952788232\\
44	5.98807935635246\\
45	6.07378928137408\\
46	6.37144041102429\\
47	6.18242058613637\\
48	5.91308189282641\\
49	5.36931940753907\\
50	4.86688497964783\\
51	5.46406921514374\\
52	5.09354284326135\\
53	5.03754065146783\\
54	4.42668141530171\\
55	4.47220710057187\\
56	4.57530365879238\\
57	4.08840616357097\\
58	4.36500979196392\\
59	4.74178355114269\\
60	4.41199309385014\\
61	3.94284292632187\\
62	3.80946963697789\\
63	3.99986503134951\\
64	4.16032897540887\\
65	4.12803529101606\\
66	4.04408825693215\\
67	4.38365326136501\\
68	4.46948714964197\\
69	4.59425606040581\\
70	4.5799612735042\\
71	4.33732748478134\\
72	3.58925594585742\\
73	4.16262106171202\\
74	4.02651218866391\\
75	4.61552306255327\\
76	4.58637351969599\\
77	4.44924243302036\\
78	4.89331151471496\\
79	4.51222644362178\\
80	4.94127561364279\\
81	4.61572151071648\\
82	4.82778126501132\\
83	4.78180279801564\\
84	4.81731034852058\\
85	5.22641152559403\\
86	4.87220036127061\\
87	5.05811277058978\\
88	4.971689281004\\
89	4.89262005939398\\
90	4.76590919439582\\
91	4.93852933077826\\
92	4.1686784357775\\
93	4.30282311334947\\
94	4.09180107871523\\
95	4.54282306683334\\
96	4.9432728567703\\
97	4.09989240222478\\
98	4.54814078343296\\
99	4.95146652595987\\
100	4.85117694223118\\
101	4.99194133283749\\
102	4.62521242119934\\
103	4.05399201409318\\
104	4.00219036893104\\
105	4.26736645307781\\
106	4.27332097241678\\
107	4.24205602827214\\
108	4.50654017347274\\
109	4.2579562668821\\
110	4.21672006810858\\
111	4.32549587491752\\
112	4.55595802122024\\
113	4.37885790369999\\
114	3.53101190000907\\
115	3.94955051693181\\
116	3.83730672256186\\
117	3.66044132762237\\
118	3.89254106455889\\
119	4.01358287625\\
120	3.48780502670894\\
121	3.22369065997183\\
122	2.90979927174979\\
123	2.98226103016233\\
124	2.69154316929815\\
125	2.04799415808272\\
126	1.93009759884616\\
127	1.91566616852844\\
128	1.83162018483755\\
129	1.73276186255949\\
130	1.69515280898433\\
131	1.67298569446109\\
132	1.57864546305918\\
133	1.50737507011822\\
134	1.6552143122457\\
135	1.60983373115357\\
136	1.64254312683471\\
137	1.7450156901548\\
138	1.55097591848125\\
139	1.78019543349538\\
140	1.44508746116368\\
141	1.61402925752679\\
142	1.47588027271836\\
143	1.66125698638247\\
144	1.69610064785028\\
145	1.49110053800947\\
146	1.60846438019142\\
147	1.41167488374693\\
148	1.49353355329031\\
149	1.39046162283534\\
150	1.53236002248004\\
151	1.301841390057\\
152	1.34511715398013\\
153	1.25678731933546\\
154	1.38632829829044\\
155	1.21203838487266\\
156	1.21913133926836\\
157	1.25522160044288\\
158	1.34506558157607\\
159	1.3340402066898\\
160	1.44516413199541\\
161	1.31732015478773\\
162	1.33925619327394\\
163	1.35514482951765\\
164	1.41829688896358\\
165	1.25811881738802\\
166	1.31532524888483\\
167	1.45487598538826\\
168	1.38750306770542\\
169	1.21437342009277\\
170	1.2972194412711\\
171	1.42952987874355\\
172	1.3186407250686\\
173	1.17217634825689\\
174	1.49189311641025\\
175	1.05642082002907\\
176	1.24679068737953\\
177	1.43710663455465\\
178	1.35148621625539\\
179	1.41145426447654\\
180	1.338228541443\\
181	1.20122297997931\\
182	1.42104729631168\\
183	1.20863511172287\\
184	1.29212357447206\\
185	1.25950411082841\\
186	1.5105558819833\\
187	1.06936578816471\\
188	1.29521863966724\\
189	1.31268531443769\\
190	1.25751969922366\\
191	1.35126769490924\\
192	1.3631388792631\\
193	1.47246601374869\\
194	1.30534913464958\\
195	1.35580243403181\\
196	1.2715553467275\\
197	1.51839532440769\\
198	1.48270287416854\\
199	1.24756533798593\\
200	1.56163612856378\\
201	1.30906658178152\\
202	1.37474164568539\\
203	1.46603133821296\\
204	1.23162849589851\\
205	1.29689126888526\\
206	1.41794783946995\\
207	1.58801902622268\\
208	1.80611515679115\\
209	1.52077671908326\\
210	1.91137180779656\\
211	1.82569923588858\\
212	1.76617949072501\\
213	1.78071980542644\\
214	2.13074099216627\\
215	1.87357875859627\\
216	1.76098597191319\\
217	1.90205652762173\\
218	2.16875297122848\\
219	2.18099642748393\\
220	2.11444690998161\\
221	2.08111610471485\\
222	2.1857938729075\\
223	2.62355498110016\\
224	2.5227974168491\\
225	2.64886777893485\\
226	2.64414942125164\\
227	2.34704744755126\\
228	2.61723331773029\\
229	2.40844883486255\\
230	2.71691372107982\\
231	2.56126883303616\\
232	2.43383069227321\\
233	2.30267056132917\\
234	2.24468557151083\\
235	2.49281763935931\\
236	2.73807266275889\\
237	2.79967623572126\\
238	2.9859396993486\\
239	2.76661803011636\\
240	2.59493255324619\\
241	2.87960225915991\\
242	3.1373086117478\\
243	2.78509132214168\\
244	2.94635723164492\\
245	3.10951115878995\\
246	3.15041676150101\\
247	3.14729355473581\\
248	2.96823409444718\\
249	3.25800277185687\\
250	3.30391470603637\\
251	3.25441207552113\\
252	3.44300911247231\\
253	3.81914439081732\\
254	3.52673976811358\\
255	3.514935006967\\
256	3.97134399812122\\
257	3.88060674111777\\
258	3.77442940397392\\
259	3.83704431107724\\
260	3.77924851392166\\
261	3.44775182306203\\
262	3.93550217489428\\
263	3.96987579646267\\
264	3.79142566858412\\
265	3.89455619948839\\
266	3.91071477192974\\
267	4.0994030989266\\
268	4.59574562515107\\
269	4.29739708211353\\
270	4.49134317668345\\
271	4.45522253970829\\
272	4.81512986371746\\
273	5.02704533992095\\
274	4.86751517914847\\
275	5.04519500899453\\
276	4.75191902463906\\
277	4.82514349581243\\
278	4.67623377641958\\
279	4.9054677927109\\
280	4.44349177211118\\
281	4.67936484861231\\
282	4.57433495738196\\
283	4.73981019834126\\
284	4.85496829802419\\
285	5.05092265176057\\
286	3.52737568686423\\
287	3.1038995020966\\
288	2.47061336327439\\
289	2.26223797636485\\
290	2.47120288392444\\
291	2.04200208427879\\
292	2.38706023525815\\
293	2.08468469127625\\
294	1.97037452192227\\
295	2.29840186699444\\
296	2.10030771733753\\
297	2.66195687147188\\
298	2.25614102670991\\
299	2.11245281029964\\
300	2.3916110761043\\
301	2.36315555075507\\
302	2.39053585678585\\
303	2.2849496823386\\
304	2.29005264751514\\
305	2.52466809249223\\
306	2.80703064499029\\
};\label{pgf:rmseMVA}
\addlegendentry{\lblMVAest{1}}

\addplot [color=IEEEgreen, line width=\LWbound]
  table[row sep=crcr]{%
1	29.6639788785148\\
2	24.2403065658504\\
3	21.014633263461\\
4	18.8198104071077\\
5	17.2053451474288\\
6	15.955656264333\\
7	14.9531610302566\\
8	14.1269995300103\\
9	13.4320073620581\\
10	12.8377417034273\\
11	12.3228410546825\\
12	11.8718101380398\\
13	11.4730968089259\\
14	11.1178871435998\\
15	10.7993223039758\\
16	10.5119728674173\\
17	10.2514762366707\\
18	10.0142805069204\\
19	9.797459725688\\
20	9.59818782240513\\
21	9.41417364569685\\
22	9.24361004132248\\
23	9.08498922775108\\
24	8.93702778985228\\
25	8.79863343347665\\
26	8.66885008517179\\
27	8.54684354667435\\
28	8.43188467206701\\
29	8.32339950743979\\
30	8.22077307777521\\
31	8.1234887825645\\
32	8.03110148268816\\
33	7.94322129719879\\
34	7.85950255092467\\
35	7.77913072757682\\
36	7.70186022647705\\
37	7.62751545322477\\
38	7.55592860879711\\
39	7.48694980025944\\
40	7.42043331260614\\
41	7.35624256860388\\
42	7.29424970139757\\
43	7.23433484608455\\
44	7.17638553724726\\
45	7.12029613412947\\
46	7.06596729815561\\
47	7.01330551776466\\
48	6.96222267786876\\
49	6.91263566957804\\
50	6.86446603607183\\
51	6.81763965076403\\
52	6.76435838301437\\
53	6.71482425193313\\
54	6.66756491431781\\
55	6.62195564994362\\
56	6.57953261847355\\
57	6.53822400521932\\
58	6.49788435472876\\
59	6.45843389082656\\
60	6.41981753306521\\
61	6.38198812410987\\
62	6.34514444075567\\
63	6.30888103806186\\
64	6.2732128548109\\
65	6.2381498632918\\
66	6.20367593309759\\
67	6.16976577955779\\
68	6.13639166933129\\
69	6.10352597589407\\
70	6.07114211666836\\
71	6.03921480100152\\
72	6.00772004388858\\
73	5.97663510656591\\
74	5.94593842228665\\
75	5.91560952547269\\
76	5.8856289879601\\
77	5.85465957538149\\
78	5.82476441777599\\
79	5.79533564629507\\
80	5.76630735882026\\
81	5.73760688516851\\
82	5.70918729109885\\
83	5.68102549491334\\
84	5.65310553599715\\
85	5.62541331146833\\
86	5.59793558518553\\
87	5.57065992997107\\
88	5.54357471841916\\
89	5.51666906586643\\
90	5.48993275754679\\
91	5.46335618272596\\
92	5.43693028175638\\
93	5.41064650461118\\
94	5.38490843636935\\
95	5.35969694522432\\
96	5.33500109037853\\
97	5.31082137284052\\
98	5.28716833573138\\
99	5.26406076038445\\
100	5.24152432266762\\
101	5.21959047886673\\
102	5.19829552625554\\
103	5.17630374953402\\
104	5.15536355046738\\
105	2.92582586631437\\
106	2.38293049831102\\
107	2.14837122658946\\
108	2.02993782522856\\
109	1.96535135972418\\
110	1.92790124224822\\
111	1.90462422771635\\
112	1.88885496825073\\
113	1.87707671603159\\
114	1.86690378616008\\
115	1.85759063842742\\
116	1.84865470637189\\
117	1.83987223302925\\
118	1.8312326829495\\
119	1.8227371359068\\
120	1.43613464080868\\
121	1.34914365101261\\
122	1.32258017447939\\
123	1.31052648500896\\
124	1.30365691733595\\
125	1.16927582893194\\
126	1.12906392163757\\
127	1.11733170795562\\
128	1.10936944741244\\
129	1.1020518247162\\
130	1.09492209787514\\
131	1.08791412415689\\
132	1.08101835901452\\
133	1.07423357043966\\
134	1.06875974316155\\
135	1.06357378624105\\
136	1.05843153431304\\
137	1.05350849856559\\
138	1.04878909086615\\
139	1.04427601323077\\
140	0.9920058825229\\
141	0.987836147477577\\
142	0.983024195424718\\
143	0.979296296049034\\
144	0.976351029077698\\
145	0.973868888593342\\
146	0.971720869389764\\
147	0.969864835731403\\
148	0.9682909727805\\
149	0.799432889552788\\
150	0.796248982368658\\
151	0.794888095140776\\
152	0.793820327933013\\
153	0.792958436275078\\
154	0.792123705951104\\
155	0.791304740516991\\
156	0.79049529411564\\
157	0.771189142353109\\
158	0.77027896075825\\
159	0.770337341484677\\
160	0.769835038273222\\
161	0.769192963358072\\
162	0.768516137557641\\
163	0.767822711291387\\
164	0.767123761657816\\
165	0.76642519443291\\
166	0.765730145402267\\
167	0.765040291538469\\
168	0.758773646422581\\
169	0.757618731243207\\
170	0.756745273938928\\
171	0.753348050444445\\
172	0.752142779062039\\
173	0.751228489474828\\
174	0.750470569273272\\
175	0.749690620439861\\
176	0.748768892062834\\
177	0.747948265281328\\
178	0.747151232153754\\
179	0.746363143198474\\
180	0.745581588671185\\
181	0.744935911839229\\
182	0.745109718507201\\
183	0.744514439159215\\
184	0.743775788643484\\
185	0.742465015349505\\
186	0.741659576670216\\
187	0.740725003063738\\
188	0.739578406092585\\
189	0.738667737104192\\
190	0.737959119505575\\
191	0.737308400405002\\
192	0.736679813027381\\
193	0.736060881754404\\
194	0.735448802665285\\
195	0.734842756124341\\
196	0.734242606341625\\
197	0.733648376718339\\
198	0.733060145775392\\
199	0.732478006536371\\
200	0.731902058345666\\
201	0.73133240439087\\
202	0.730769151839278\\
203	0.730212412286212\\
204	0.729871895785405\\
205	0.729508341690276\\
206	0.729117930516466\\
207	0.71732400905297\\
208	0.716751412010049\\
209	0.716234826989345\\
210	0.715763679005716\\
211	0.715277819303848\\
212	0.714611553137841\\
213	0.713883940619329\\
214	0.713220029531011\\
215	0.712610260401594\\
216	0.712022822450636\\
217	0.711452036164341\\
218	0.710891334071085\\
219	0.710338460136219\\
220	0.708968158969517\\
221	0.708283545656144\\
222	0.707675370198518\\
223	0.707097992820549\\
224	0.70654120655315\\
225	0.705998800665388\\
226	0.705465704431908\\
227	0.705115403510852\\
228	0.705029073862796\\
229	0.705217138700919\\
230	0.705680685634807\\
231	0.706418341737899\\
232	0.707426830345164\\
233	0.708700919950239\\
234	0.710233297552542\\
235	0.712014431194875\\
236	0.714032438144557\\
237	0.716272971001907\\
238	0.718608187614616\\
239	0.720981598639952\\
240	0.723386568748794\\
241	0.725822254458914\\
242	0.728288435255453\\
243	0.730784963123368\\
244	0.733311695359666\\
245	0.735868486207\\
246	0.738455186388718\\
247	0.741071643126791\\
248	0.743717700322255\\
249	0.746393198635797\\
250	0.749097975583715\\
251	0.751831865636556\\
252	0.754594700346417\\
253	0.757386308500016\\
254	0.777001567766213\\
255	0.78197599884403\\
256	0.785237838967377\\
257	0.753067675896357\\
258	0.754033472186934\\
259	0.756914661124674\\
260	0.759794798741723\\
261	0.762685671718416\\
262	0.765626172968411\\
263	0.768615684758866\\
264	0.771478434471199\\
265	0.774633695500664\\
266	0.777848646132956\\
267	0.781046756227729\\
268	0.784203439571266\\
269	0.787375148062132\\
270	0.790572193723407\\
271	0.79379716633619\\
272	0.797219431858503\\
273	0.800768172684826\\
274	0.804360106514087\\
275	0.807979444621142\\
276	0.811800391587069\\
277	0.815912151072072\\
278	0.819737521587515\\
279	0.823556596317241\\
280	0.827372681240354\\
281	0.831189330734395\\
282	0.835010528180131\\
283	0.838840959914725\\
284	0.842683928394679\\
285	0.846541660874786\\
286	0.852900380545554\\
287	0.857213226321875\\
288	0.861310805703639\\
289	0.938162538132815\\
290	0.976518015032948\\
291	0.994649270845101\\
292	1.00443651095565\\
293	1.01057108678831\\
294	1.02262957502389\\
295	1.02751315294987\\
296	1.03082109057691\\
297	1.03359547116505\\
298	1.03733606607788\\
299	1.0401806588828\\
300	1.04261830582442\\
301	1.044853881113\\
302	1.04698115566999\\
303	1.0490453419502\\
304	1.05107133643232\\
305	1.05307432698287\\
306	1.05805812742425\\
};\label{pgf:MEB}
\addlegendentry{\lblMVAmeb{1}}


\addplot[area legend, draw=none, fill=IEEEgreen, fill opacity=0.1]
table[row sep=crcr] {%
x	y\\
1	500\\
2	500\\
3	500\\
4	500\\
5	500\\
6	500\\
7	500\\
8	500\\
9	500\\
10500\\
11	500\\
12	223.119870577401\\
13	192.792368125918\\
14	180.005362859279\\
15	114.294239133851\\
16	112.930850528952\\
17	177.391966932797\\
18	165.481837236414\\
19	102.66012685528\\
20	101.757206122727\\
21	99.8978815357654\\
22	98.8554482355557\\
23	81.8788624598998\\
24	73.0267492010196\\
25	69.9974431793715\\
26	66.5819051494843\\
27	54.7115428415827\\
28	49.3192282178623\\
29	45.3170621880242\\
30	44.1420942862558\\
31	41.4158606325189\\
32	38.6650600257154\\
33	37.9220518932707\\
34	33.0559742685672\\
35	33.0375518488758\\
36	31.1402401262679\\
37	29.9949175906377\\
38	28.897796831845\\
39	26.5186095227977\\
40	22.8376843298197\\
41	21.3206060932211\\
42	20.107608559949\\
43	18.694079653015\\
44	15.1611224650314\\
45	14.6438324542079\\
46	13.178949039378\\
47	12.3125278363952\\
48	12.1233221600965\\
49	13.0194861445862\\
50	10.9652937713347\\
51	10.1831450383526\\
52	11.1877167487238\\
53	10.3072320107151\\
54	9.32134115090837\\
55	10.4801939666916\\
56	8.8769037920774\\
57	10.4144474053363\\
58	8.68721210583745\\
59	8.9800567698146\\
60	8.08544441026324\\
61	7.91572465089981\\
62	8.31528742820679\\
63	7.89006782344787\\
64	7.66252757825892\\
65	7.73203463451798\\
66	7.54264154868022\\
67	8.80941017153845\\
68	9.51646453406646\\
69	8.60230324399962\\
70	7.98269183346464\\
71	7.43103381841442\\
72	6.31478638659775\\
73	8.20327302671631\\
74	7.85040446226683\\
75	8.74546293263586\\
76	9.05382882987407\\
77	7.40389345329127\\
78	8.56163047111908\\
79	8.58588529717279\\
80	8.67823785247488\\
81	9.19182340782607\\
82	8.69250107412494\\
83	8.22318128441739\\
84	9.50177377002806\\
85	9.84662941141455\\
86	8.90497161949643\\
87	9.64218082739388\\
88	8.51967287727996\\
89	7.98210426020937\\
90	8.5980542096796\\
91	8.50430905750176\\
92	7.82694202413101\\
93	8.2836335904499\\
94	9.62694492181683\\
95	8.41408050423916\\
96	8.69178933104378\\
97	8.32875305997193\\
98	9.05405502556563\\
99	8.50650287634624\\
100	8.95489646204561\\
101	8.59623612845343\\
102	8.52111460098504\\
103	7.9366703228127\\
104	7.56872684891127\\
105	7.79187176056693\\
106	7.44214950160355\\
107	7.72293720274439\\
108	7.4935244586633\\
109	7.89716703906497\\
110	7.07791165100911\\
111	6.84616391048613\\
112	8.35015240062198\\
113	8.20294252294603\\
114	6.82185549987919\\
115	7.15607584583743\\
116	6.62032601254701\\
117	6.16206660221199\\
118	6.37156662197252\\
119	6.64709369201576\\
120	6.15615387039674\\
121	5.5359770535969\\
122	5.1124426015144\\
123	5.45273965710943\\
124	4.4952577781489\\
125	3.46708528231078\\
126	3.27184031173309\\
127	3.02060129521877\\
128	3.09643246013136\\
129	2.77011277489578\\
130	3.04749212721288\\
131	2.87269920877479\\
132	2.50870889532247\\
133	2.51517964477515\\
134	2.81834696920086\\
135	2.77822957901235\\
136	2.66834178360392\\
137	2.81698084188819\\
138	2.65782187462389\\
139	2.86477724368419\\
140	2.48881708435985\\
141	2.85474320205006\\
142	2.64622636438018\\
143	2.68647827627062\\
144	2.94169098670389\\
145	2.51740945732976\\
146	2.72803901619463\\
147	2.4709766018423\\
148	2.36382481566183\\
149	2.57321319398378\\
150	2.7472031109415\\
151	2.70965848128844\\
152	2.38349287535355\\
153	2.24966523509034\\
154	2.42930546965102\\
155	2.08489383906582\\
156	2.00307037924232\\
157	2.29103476404146\\
158	2.88324021142239\\
159	2.58096875536738\\
160	2.51669483180158\\
161	2.53429963262011\\
162	2.50908114692268\\
163	2.55771619013396\\
164	2.67648234989545\\
165	2.39293004022171\\
166	2.68230251248394\\
167	2.73085005410519\\
168	2.50285512308484\\
169	2.19531153466787\\
170	2.09246694780779\\
171	2.58680492919073\\
172	2.47577848848772\\
173	2.19011953767083\\
174	2.46286082300886\\
175	2.06823499361034\\
176	2.20972613316974\\
177	2.53349652043531\\
178	2.58475519005947\\
179	2.25176631995919\\
180	2.32758357103233\\
181	2.07432747269013\\
182	2.34752415978896\\
183	2.08826485177721\\
184	2.21397618687423\\
185	2.14900653095533\\
186	2.31159406844523\\
187	2.04709486782173\\
188	2.3547929113628\\
189	2.30060867701706\\
190	2.26994548858423\\
191	2.13274443204536\\
192	2.40101125810537\\
193	2.47118405894158\\
194	2.41582816971614\\
195	2.38681319290202\\
196	2.07677536354882\\
197	2.53842610865761\\
198	2.51373282878405\\
199	2.48387785985783\\
200	2.73064652393534\\
201	2.25897629064045\\
202	2.53603626040302\\
203	2.33139713140268\\
204	2.18948403016323\\
205	2.13540121293502\\
206	2.43580017804289\\
207	2.69289070798444\\
208	3.22505438019949\\
209	2.69418316739737\\
210	3.10348222265871\\
211	3.25486955378648\\
212	3.10169207469934\\
213	3.26090797446314\\
214	3.33370257432897\\
215	3.16968163483629\\
216	3.46257892980307\\
217	3.38539073155654\\
218	3.28761137708049\\
219	3.34981560350415\\
220	3.67369781425707\\
221	3.73689042916793\\
222	3.96569794183709\\
223	4.22928860337932\\
224	4.33880781811721\\
225	3.97680615375348\\
226	4.37729840258546\\
227	4.57838371869488\\
228	4.37172901207358\\
229	3.94939611561492\\
230	4.35648751852853\\
231	4.62545516986402\\
232	4.29561650245125\\
233	4.15582520127254\\
234	4.30922370374929\\
235	4.54140624636997\\
236	4.42298167501559\\
237	4.91585890701929\\
238	4.75867486429898\\
239	4.54195230100855\\
240	4.47606894362067\\
241	4.81394844709126\\
242	4.87423643940268\\
243	4.87323248820078\\
244	4.97169656928292\\
245	5.2130728121519\\
246	5.42684496197894\\
247	5.43840905575278\\
248	5.02491381343423\\
249	5.59699175896015\\
250	5.4347209299528\\
251	4.98595650339763\\
252	5.26856560578709\\
253	6.03206924463048\\
254	6.71874568779597\\
255	7.13599102825654\\
256	6.39393654631834\\
257	6.01589665788415\\
258	5.91501403284587\\
259	6.1864498577679\\
260	5.86386652669312\\
261	5.47391017905674\\
262	6.19338091841392\\
263	6.42486355329587\\
264	6.53798116316014\\
265	6.61677227064243\\
266	6.39406393301595\\
267	6.14632678658613\\
268	7.30957705410444\\
269	8.00606477558027\\
270	7.22589540283455\\
271	7.19577609883992\\
272	7.38905993477356\\
273	8.27426669068839\\
274	7.72681121565654\\
275	7.34463487976931\\
276	7.72219117451055\\
277	7.32058872214406\\
278	7.44345735594761\\
279	7.63644315680543\\
280	8.23437068010537\\
281	7.94896396374618\\
282	7.29238711578999\\
283	8.43114357669492\\
284	8.43342363885691\\
285	8.61392228961752\\
286	6.61847260383392\\
287	5.04784592671376\\
288	4.47478492559095\\
289	4.35694685305714\\
290	4.23572230916171\\
291	3.94714063354639\\
292	4.08339330539737\\
293	3.6545504498148\\
294	3.77590319544399\\
295	3.81313216243853\\
296	3.72628118374003\\
297	4.2895810608849\\
298	3.82574525285742\\
299	3.46212103977384\\
300	4.41119352799238\\
301	4.02502299637557\\
302	4.39260100238087\\
303	3.88318080369555\\
304	3.90979533713207\\
305	4.15276309772766\\
306	4.68116198800078\\
306	0.692959404021881\\
305	0.448795637445326\\
304	0.466379261819949\\
303	0.573422062371488\\
302	0.545980473537595\\
301	0.460910172195877\\
300	0.40950346573923\\
299	0.39473631453736\\
298	0.52487007678011\\
297	0.709746782187208\\
296	0.536937275950252\\
295	0.455090424214858\\
294	0.432113188715138\\
293	0.509389996368185\\
292	0.462726365548474\\
291	0.48853668171541\\
290	0.437957510319414\\
289	0.46732154580083\\
288	0.414040604305952\\
287	0.517825048127455\\
286	0.490230637406966\\
285	1.3681488079705\\
284	1.44511777900029\\
283	1.76998227969437\\
282	1.4112944856409\\
281	1.56075932213506\\
280	1.30045803978562\\
279	1.50572015491838\\
278	1.77930972264218\\
277	1.44010701322981\\
276	1.80377549819569\\
275	1.47585203318633\\
274	1.77158825065008\\
273	1.63324052454709\\
272	1.77961234934611\\
271	1.64030274549696\\
270	1.46538869162841\\
269	1.58270753650433\\
268	1.1246291340639\\
267	1.21799782772149\\
266	1.25453838337879\\
265	1.13121839573225\\
264	1.0217998965615\\
263	1.08705014049456\\
262	0.963998047602693\\
261	0.696795312917658\\
260	0.995304169515773\\
259	1.03608092712677\\
258	0.82285217320598\\
257	0.998830667241714\\
256	1.37301135788109\\
255	0.845204127016232\\
254	0.901893943844007\\
253	1.09342151429748\\
252	0.985176982565976\\
251	0.83338937217701\\
250	0.663607994669459\\
249	0.828072879368571\\
248	0.745854888901289\\
247	1.00293097756149\\
246	0.74684773112625\\
245	0.838246959394368\\
244	0.630999367091389\\
243	0.655305367448479\\
242	0.587143010547573\\
241	0.579760628188047\\
240	0.796180859892037\\
239	0.452303081853449\\
238	0.564925114647011\\
237	0.448805610532366\\
236	0.529627145021219\\
235	0.432769590943782\\
234	0.617470952873507\\
233	0.490895119063558\\
232	0.748512349746056\\
231	0.470753874199172\\
230	0.526876824679523\\
229	0.456021757552907\\
228	0.667510977808034\\
227	0.392936020732046\\
226	0.455422388890883\\
225	0.555051344753677\\
224	0.599467124659363\\
223	0.491432347147295\\
222	0.465376482232813\\
221	0.533343867815753\\
220	0.393895083934763\\
219	0.592963115053445\\
218	0.476176661632946\\
217	0.384887475692448\\
216	0.400120100656757\\
215	0.409577034501714\\
214	0.501180355369148\\
213	0.312466326393899\\
212	0.399376423778874\\
211	0.602609960846516\\
210	0.347305552910617\\
209	0.400698478304346\\
208	0.563500673653575\\
207	0.381627371354319\\
206	0.447220561751046\\
205	0.389244558379235\\
204	0.233626316294802\\
203	0.339539295457072\\
202	0.2690396371957\\
201	0.418502605715186\\
200	0.325967604208677\\
199	0.342375419090218\\
198	0.351594593031568\\
197	0.495247919849468\\
196	0.338899831561286\\
195	0.433501388830099\\
194	0.404056910388429\\
193	0.431201780412536\\
192	0.366277436976833\\
191	0.422208747029228\\
190	0.33200004128028\\
189	0.273068412080602\\
188	0.343119048721881\\
187	0.280398572009739\\
186	0.372174817169273\\
185	0.322445936304738\\
184	0.30151885325353\\
183	0.307098568137788\\
182	0.294654518239507\\
181	0.287629326766405\\
180	0.225544866471003\\
179	0.398436085863432\\
178	0.288113513621819\\
177	0.279148560357773\\
176	0.268077248414912\\
175	0.26027416486061\\
174	0.280099840931902\\
173	0.257610210586922\\
172	0.317511457915962\\
171	0.456819440834979\\
170	0.428594797948401\\
169	0.249862032402144\\
168	0.270938826799404\\
167	0.379358044583733\\
166	0.291004112052279\\
165	0.312590819380776\\
164	0.349584835929517\\
163	0.407203343007596\\
162	0.426851608543086\\
161	0.281713618644763\\
160	0.340894723654928\\
159	0.42402818008835\\
158	0.291085247236951\\
157	0.330256384083856\\
156	0.350581939648592\\
155	0.396146207879165\\
154	0.309700839876736\\
153	0.303912093413723\\
152	0.358796623886173\\
151	0.230798633188246\\
150	0.366851629402281\\
149	0.384129659708916\\
148	0.461980768252676\\
147	0.512579141305679\\
146	0.411073527149934\\
145	0.435444636887456\\
144	0.492344183898328\\
143	0.57776265476658\\
142	0.444377831922098\\
141	0.511635415665147\\
140	0.571957123474806\\
139	0.541098812628404\\
138	0.576448263497972\\
137	0.631953866755199\\
136	0.355507817441131\\
135	0.59087476228214\\
134	0.47267734920948\\
133	0.514122638455741\\
132	0.44986045951836\\
131	0.621048538548705\\
130	0.639289383372971\\
129	0.669440297022713\\
128	0.607237541937629\\
127	0.740230463059018\\
126	0.67525788228327\\
125	0.634430203847476\\
124	0.744327917361598\\
123	0.94005064560964\\
122	1.14780455167786\\
121	1.14947223580012\\
120	0.979120711460696\\
119	1.14250091673948\\
118	1.09058982838838\\
117	1.34057399747433\\
116	1.38164480291615\\
115	1.25385712980955\\
114	1.37151754594398\\
113	1.60738784889007\\
112	1.39815967762486\\
111	1.56269229584194\\
110	1.19479171240175\\
109	1.36574873457129\\
108	1.5259111616264\\
107	0.991893045544285\\
106	1.12445018660802\\
105	1.23906896050799\\
104	1.26087599606161\\
103	1.16263107441058\\
102	1.49934825463544\\
101	0.96964541174842\\
100	1.10023759043974\\
99	0.947808854052498\\
98	1.53074061992416\\
97	1.13082873780354\\
96	1.5113088699627\\
95	1.23524648968409\\
94	1.13320309878749\\
93	0.940285147315219\\
92	1.36996492160661\\
91	1.06194884204908\\
90	1.3410227781363\\
89	1.09610691319679\\
88	1.17379862861932\\
87	1.37509212235298\\
86	1.29864630716098\\
85	1.33956393505531\\
84	0.833684446252689\\
83	1.00381241427724\\
82	1.02313671366764\\
81	1.27193423084606\\
80	1.4696665338909\\
79	1.16646394199539\\
78	1.03674017179101\\
77	1.31999003382776\\
76	0.749444078021239\\
75	1.1914345892585\\
74	1.01492352619467\\
73	1.0928823028447\\
72	0.919655286188278\\
71	0.89796404316381\\
70	0.895169931446845\\
69	0.999372731253908\\
68	1.03678641326625\\
67	0.699468907715631\\
66	0.867878543488219\\
65	1.14745744734528\\
64	0.801304166104869\\
63	1.10192297967026\\
62	1.30867443980152\\
61	0.657445007155203\\
60	0.963280299455036\\
59	1.32981830356736\\
58	0.796131967127224\\
57	1.01826579797546\\
56	1.45827405419587\\
55	1.16939699857928\\
54	0.91722171830402\\
53	1.37214627217489\\
52	1.15200572032531\\
51	0.730647348535081\\
50	1.49643256859438\\
49	1.22297512365388\\
48	1.29519470545091\\
47	1.64910328758101\\
46	1.45490714418421\\
45	1.50117463396877\\
44	1.2260124724517\\
43	1.32809934906975\\
42	1.39385830304293\\
41	0.980034021108913\\
40	1.31162937537651\\
39	1.15065066159641\\
38	1.29787994420099\\
37	1.49401818172617\\
36	1.79559045357084\\
35	1.31332991651946\\
34	1.47612213167584\\
33	2.09730509962836\\
32	1.90966107009551\\
31	1.85321142815215\\
30	2.28491045916375\\
29	1.88475039901032\\
28	2.22010246762461\\
27	2.21851647753729\\
26	2.06071558502438\\
25	1.77388311401175\\
24	2.28000178136023\\
23	2.09004830520274\\
22	2.80558674566635\\
21	2.89641930801789\\
20	4.0172953314399\\
19	3.71568985064167\\
18	3.02731226988334\\
17	0\\
16	0\\
15	0\\
14	0\\
13	0\\
12	0\\
11	0\\
10	0\\
9	0\\
8	0\\
7	0\\
6	0\\
5	0\\
4	0\\
3	0\\
2	0\\
1	367.329335817291\\
}--cycle;\label{pgf:sigmaMVA}
\addlegendentry{\lblMVAuncertainty{1}}


==> figures/MVA-5-subplots/MVA-5plot-s2.tex <==
\addplot [color=mycolor2, dashed, line width=\LWestimates]
  table[row sep=crcr]{%
1	79.3677956914618\\
2	14.085950261264\\
3	12.622030365884\\
4	10.6963361352222\\
5	9.71970570036316\\
6	9.33540515339634\\
7	8.5657647845598\\
8	7.88639235364319\\
9	7.64665381758637\\
10	7.11092382034246\\
11	7.2743997085548\\
12	6.8854307703479\\
13	6.52396681929679\\
14	6.41767480498623\\
15	6.72394720313521\\
16	6.67936117963891\\
17	6.62034603571912\\
18	6.8883466562649\\
19	6.70819764517888\\
20	6.45223412797815\\
21	6.4680456984754\\
22	6.63596396477271\\
23	6.68598525873481\\
24	6.17074185267748\\
25	6.1101542630686\\
26	6.16330237960221\\
27	6.03294119489981\\
28	6.20101897500002\\
29	6.68418825848826\\
30	6.7731874777562\\
31	6.55985916957492\\
32	7.05859592991005\\
33	6.84467379037112\\
34	6.94868218121216\\
35	6.68264002913792\\
36	6.57630511331329\\
37	6.49858833557376\\
38	6.19025616415687\\
39	6.13026578178521\\
40	5.59672593385462\\
41	4.86876296661352\\
42	5.10288224609698\\
43	4.8356145727075\\
44	4.94758731738336\\
45	4.61345273869893\\
46	4.64702799085584\\
47	4.79066682894385\\
48	4.43191500793952\\
49	4.58206147266085\\
50	4.27079987148742\\
51	4.60879293880035\\
52	4.44572897792634\\
53	4.73661402678511\\
54	5.32688959192024\\
55	4.96881546099336\\
56	4.91438569901981\\
57	4.68897938730571\\
58	4.7612927895892\\
59	4.74789126341094\\
60	4.49461074470146\\
61	4.44603772353103\\
62	5.07929446830411\\
63	5.2151012491019\\
64	5.27944973851484\\
65	5.15580416012812\\
66	5.50417537105746\\
67	5.81009117814468\\
68	5.53147878410692\\
69	5.88478936754869\\
70	5.88013223615827\\
71	5.8465806968248\\
72	6.112078976194\\
73	6.1213999858142\\
74	6.25530934595162\\
75	5.80235724997754\\
76	5.4012958110923\\
77	5.79944396006615\\
78	5.02827630328018\\
79	5.3730262855622\\
80	5.02323145118943\\
81	4.75205219093553\\
82	4.44075608209618\\
83	4.26012919664297\\
84	4.1385558485074\\
85	3.94663950211041\\
86	3.87088189375678\\
87	3.7929721829544\\
88	3.98867014438145\\
89	3.64998870072831\\
90	3.78340441852054\\
91	3.46559802332909\\
92	3.19862669706174\\
93	3.43034155829453\\
94	3.53227976870904\\
95	3.50724960320967\\
96	3.39942735908393\\
97	3.32296824836541\\
98	3.23377062717813\\
99	3.37675339727963\\
100	3.43322684536955\\
101	3.77322252061783\\
102	3.33887671488941\\
103	3.60352754214818\\
104	3.59680191416616\\
105	3.87475589779215\\
106	3.73675955539388\\
107	3.8904408304025\\
108	3.90478065289007\\
109	3.83249896087603\\
110	3.70594499525704\\
111	3.36856418505878\\
112	3.49687765802131\\
113	3.43534261926122\\
114	3.36054393601014\\
115	3.50470201857458\\
116	3.59418629910616\\
117	3.57440777523127\\
118	3.17729940140154\\
119	3.61079416427416\\
120	3.42838866264517\\
121	3.73535811939043\\
122	3.76168904627956\\
123	3.90824803949708\\
124	3.75652799383963\\
125	3.63611750205722\\
126	3.34875468099198\\
127	3.61484918197694\\
128	3.25001444639406\\
129	2.98738764036086\\
130	3.07331611748197\\
131	2.87883712831187\\
132	2.77583310781265\\
133	3.0541542003116\\
134	3.00264612026402\\
135	2.91570518786764\\
136	3.10230874476564\\
137	3.29983275426681\\
138	3.00822623117126\\
139	3.37860420980323\\
140	3.0517959987393\\
141	3.10665816203555\\
142	2.83040119007488\\
143	2.70994984180307\\
144	2.7811581528881\\
145	2.96873648632947\\
146	2.92466438601462\\
147	2.70288924090262\\
148	2.62642607605475\\
149	2.75768141764002\\
150	2.71652587107359\\
151	3.09100237710221\\
152	3.00649528610654\\
153	3.02273767019007\\
154	3.05230643400358\\
155	3.05196120471206\\
156	2.84324224538127\\
157	2.63978102386301\\
158	2.84874879114008\\
159	2.71184127855152\\
160	2.8959575611228\\
161	2.67857918767056\\
162	2.64811646088914\\
163	3.00095742003207\\
164	2.94617214759957\\
165	2.86135064323862\\
166	3.17173445581734\\
167	2.99278600018929\\
168	2.79309501770408\\
169	2.66723981240555\\
170	2.78838315042657\\
171	2.62133064293436\\
172	2.28614385516957\\
173	2.36036010579609\\
174	2.37490904083169\\
175	2.13217694255271\\
176	2.49139072896993\\
177	2.41906713997561\\
178	2.1693361852687\\
179	2.13920717824392\\
180	1.87745186424726\\
181	2.14615771234104\\
182	2.45088572538814\\
183	2.66109852783915\\
184	2.5225904165325\\
185	3.39649563862631\\
186	3.93861985741946\\
187	4.50701571310261\\
188	4.63105174674709\\
189	5.07532983778584\\
190	5.53659323051241\\
191	6.06687794112321\\
192	6.31695714902157\\
193	6.38572102736126\\
194	6.41594959149136\\
195	6.36569239279358\\
196	6.45254334658312\\
197	6.80453851503341\\
198	6.46682247549914\\
199	6.91384460348693\\
200	6.95801080850443\\
201	7.01373617071906\\
202	7.384154004338\\
203	6.87996672341307\\
204	7.66936914345461\\
205	7.63388343665935\\
206	7.7832476226576\\
207	8.40048503076246\\
208	8.48026190588416\\
209	7.48770683020834\\
210	6.75220244883213\\
211	7.01729498631184\\
212	6.27472835064069\\
213	5.58416817849254\\
214	5.45648069886888\\
215	5.06656913393956\\
216	4.86109671587011\\
217	4.58690032837803\\
218	5.07682680030994\\
219	4.71055590251769\\
220	4.2468700153878\\
221	4.37291246422844\\
222	4.44248855312556\\
223	4.50974564806987\\
224	4.40093693006871\\
225	3.91739323692994\\
226	4.44040373891606\\
227	4.2896788416604\\
228	4.06993054429994\\
229	4.56203234505905\\
230	4.42863497302921\\
231	4.46079731430559\\
232	4.46763848625744\\
233	4.72353709635472\\
234	4.48542594412439\\
235	4.67177541940533\\
236	4.5124977163416\\
237	4.30062869068656\\
238	5.07160128487092\\
239	4.9422387008726\\
240	4.95395984833691\\
241	4.93040395857664\\
242	5.27631457646728\\
243	5.46610949432708\\
244	5.50817494903251\\
245	5.22242696506923\\
246	5.23007911736389\\
247	5.68606778260555\\
248	5.88127029947496\\
249	6.10827052861271\\
250	6.1021736880146\\
251	6.34239753087146\\
252	5.86496755547959\\
253	5.7685656728344\\
254	5.11254012519199\\
255	5.42111669080948\\
256	5.58794763249801\\
257	6.12818689719867\\
258	6.07714860008084\\
259	6.42364164636333\\
260	6.63825422954832\\
261	6.93155711628742\\
262	6.6947065731816\\
263	6.73363417880316\\
264	7.04228877644808\\
265	7.12386379669998\\
266	7.14630863199439\\
267	7.05364105970089\\
268	7.55995753960974\\
269	7.54164427161813\\
270	7.57194522147966\\
271	7.83059675023437\\
272	7.59560324699898\\
273	7.74812843369075\\
274	7.90581333704438\\
275	8.17902998442262\\
276	6.42430650050577\\
277	4.69825941961655\\
278	3.90230678072027\\
279	3.37801039594868\\
280	3.22953626418935\\
281	3.18585564338649\\
282	3.31846530193113\\
283	3.02481704612689\\
284	2.82364054718684\\
285	2.91331594034001\\
286	3.03602330744349\\
287	2.90109730492543\\
288	2.37636975318704\\
289	2.10719583684714\\
290	2.8325352233996\\
291	2.8003480611773\\
292	2.47000139548482\\
293	2.46173779530237\\
294	2.47918068095444\\
295	2.74331014456179\\
296	2.68842968712697\\
297	2.6161261392389\\
298	2.34601366499226\\
299	2.3565165250242\\
300	2.91672805221704\\
301	2.51136239149787\\
302	2.81582729403619\\
303	2.47198311702809\\
304	2.53386903223779\\
305	2.59591760538315\\
306	2.60803069763799\\
};
\addlegendentry{\lblMVAest{2}}

\addplot [color=mycolor2, line width=\LWbound]
  table[row sep=crcr]{%
1	2.01065953258301\\
2	1.75724679059\\
3	1.64389770209273\\
4	1.58845222521026\\
5	1.559563689349\\
6	1.54332726517962\\
7	1.53904871573154\\
8	1.54231636925787\\
9	1.54825161754708\\
10	1.55393762188831\\
11	1.55810435874468\\
12	1.56050793731483\\
13	1.56130898271741\\
14	1.56080307617097\\
15	1.55928908641341\\
16	1.55702317173671\\
17	1.55420813294\\
18	1.55099789667427\\
19	1.54750638225254\\
20	1.54395767139617\\
21	1.5403473594527\\
22	1.5366514523939\\
23	1.53286642131107\\
24	1.52900215829827\\
25	1.52512549482106\\
26	1.52124262893004\\
27	1.51735209677517\\
28	1.51345921542075\\
29	1.53293068436379\\
30	1.54546399319378\\
31	1.55310422351858\\
32	1.55675240286607\\
33	1.55748031139371\\
34	1.55624231873341\\
35	1.55342391418139\\
36	1.54967909231564\\
37	1.54532800867132\\
38	1.54024421408121\\
39	1.53642377538672\\
40	1.53313050472176\\
41	1.53004404760753\\
42	1.52701038287341\\
43	1.52395537433734\\
44	1.52084268664763\\
45	1.51765475397361\\
46	1.51438354124775\\
47	1.51102600123749\\
48	1.50758177867795\\
49	1.50405203111652\\
50	1.50043881673904\\
51	1.49674477472404\\
52	1.47993276445905\\
53	1.4690687020256\\
54	1.46137326599009\\
55	1.45539953628817\\
56	1.45374708699892\\
57	1.45089268468253\\
58	1.44776527087813\\
59	1.44440042562008\\
60	1.44083664995228\\
61	1.43711380061914\\
62	1.66114989332771\\
63	1.83251390393891\\
64	1.96298198410139\\
65	2.06096665648867\\
66	2.13457583043749\\
67	2.1902246485278\\
68	2.23280590258079\\
69	2.26594908309842\\
70	2.29230566935773\\
71	2.31379212888044\\
72	2.33178501282855\\
73	2.34726928216289\\
74	2.36094835905286\\
75	2.37332424696307\\
76	2.38475525908461\\
77	1.95533771315848\\
78	1.79502121831416\\
79	1.72281441186175\\
80	1.68883076211006\\
81	1.67311921773573\\
82	1.6664048496415\\
83	1.66421966697548\\
84	1.66434622942727\\
85	1.66566640114283\\
86	1.66760954619216\\
87	1.66988161395317\\
88	1.67232974021719\\
89	1.67487375878724\\
90	1.67747122004599\\
91	1.68009937988508\\
92	1.68274585725004\\
93	1.685403756368\\
94	1.68770509527541\\
95	1.68983181364031\\
96	1.69180151831996\\
97	1.69360399969007\\
98	1.69522902264482\\
99	1.69666591676207\\
100	1.6979049533882\\
101	1.6989376661047\\
102	1.69975759267984\\
103	1.69472283284068\\
104	1.69243290390277\\
105	1.69055785252778\\
106	1.68966808122203\\
107	1.68891908906393\\
108	1.68811690660731\\
109	1.68718967738188\\
110	1.68611062712911\\
111	1.68487345202335\\
112	1.68348067063045\\
113	1.68193927475422\\
114	1.68247711777706\\
115	1.68104263991601\\
116	1.67944033258991\\
117	1.67763818900768\\
118	1.67568443595576\\
119	1.67363784385311\\
120	1.669718944925\\
121	1.66724591327107\\
122	1.65300148290889\\
123	1.6488061090262\\
124	1.64814523902154\\
125	1.64710976182832\\
126	1.64594171246148\\
127	1.64483695123373\\
128	1.64351757637638\\
129	1.64200998845338\\
130	1.64037593796644\\
131	1.6386626389945\\
132	1.63690179684789\\
133	1.63511433404322\\
134	1.63348630282443\\
135	1.63206045514249\\
136	1.63065185835193\\
137	1.6294482148573\\
138	1.6284700753804\\
139	1.62771512805352\\
140	1.61873215850296\\
141	1.61594089265449\\
142	1.61482353254244\\
143	1.61459442932202\\
144	1.61486778905324\\
145	1.61545981151287\\
146	1.61627868751642\\
147	1.61727637627512\\
148	1.61842522562165\\
149	1.61646478375952\\
150	1.61692333339143\\
151	1.61789659958307\\
152	1.61913276931031\\
153	1.62054149328112\\
154	1.62235319861603\\
155	1.62429885831472\\
156	1.62627835785333\\
157	1.54762407203434\\
158	1.51833881716403\\
159	1.51537144302192\\
160	1.51623469521651\\
161	1.51765895397357\\
162	1.51923365276877\\
163	1.52078782379173\\
164	1.52229286519332\\
165	1.52375227412137\\
166	1.52517355399032\\
167	1.526562890662\\
168	1.47628375152275\\
169	1.46937727617083\\
170	1.46789828780729\\
171	1.23315415380715\\
172	1.18118782901704\\
173	1.16748186042211\\
174	1.18085813058489\\
175	1.18450518334236\\
176	1.18591013043747\\
177	1.18705829231467\\
178	1.18816988881128\\
179	1.18929665304969\\
180	1.1904565805483\\
181	1.20656922328403\\
182	1.30510413902481\\
183	1.34355699550472\\
184	1.36077024751029\\
185	1.36119306483577\\
186	1.36583341297229\\
187	1.50592271901181\\
188	1.59094983894774\\
189	1.63823021076931\\
190	1.66481397622541\\
191	1.68033582185503\\
192	1.69002083775292\\
193	1.69664315365751\\
194	1.70166329456707\\
195	1.70584605634235\\
196	1.70959132000865\\
197	1.71310801946581\\
198	1.71650535476786\\
199	1.71984042686177\\
200	1.72314311492038\\
201	1.72642906595557\\
202	1.72970648236466\\
203	1.73297967098436\\
204	1.94852111669613\\
205	2.12116432780372\\
206	2.26118606156063\\
207	2.37093820094658\\
208	2.46022960479822\\
209	2.54186416179025\\
210	2.60857044481319\\
211	2.66322174205591\\
212	2.36050235577085\\
213	2.20915906651159\\
214	2.12579816739481\\
215	2.07920002031332\\
216	2.05387606963169\\
217	2.04130190556009\\
218	2.03652254938473\\
219	2.03657501351108\\
220	1.673011168176\\
221	1.54813130084834\\
222	1.49946862423193\\
223	1.48126104207554\\
224	1.47591434895428\\
225	1.47614099687839\\
226	1.47882348553932\\
227	1.48250635268413\\
228	1.48659453159196\\
229	1.49080390897961\\
230	1.49498596260868\\
231	1.49905285527585\\
232	1.50294456893999\\
233	1.50661447340541\\
234	1.51002304381423\\
235	1.5131351953488\\
236	1.51591923693434\\
237	1.51834655578644\\
238	1.52068660797219\\
239	1.52300429797605\\
240	1.5253286605498\\
241	1.52767317474022\\
242	1.53004418555292\\
243	1.53244473088984\\
244	1.53487632949278\\
245	1.53733980055715\\
246	1.53983564521237\\
247	1.54236422258165\\
248	1.5449258317418\\
249	1.54752074980119\\
250	1.55014924972236\\
251	1.55281160870717\\
252	1.55550811219724\\
253	1.5582390558198\\
254	1.56112117602177\\
255	1.56400818768269\\
256	1.56690428669715\\
257	1.56950140675055\\
258	1.57232886915843\\
259	1.57526863908873\\
260	1.57826939157077\\
261	1.58131405461439\\
262	1.58439702512613\\
263	1.58751762624945\\
264	1.50474798322176\\
265	1.4846487436684\\
266	1.48330016995188\\
267	1.4871059952699\\
268	1.49193914036074\\
269	1.49663552614657\\
270	1.50097795300931\\
271	1.50501798308016\\
272	1.5088704960515\\
273	1.51262420663055\\
274	1.51633895783824\\
275	1.52005516413217\\
276	1.53126780816023\\
277	1.56284677518063\\
278	1.58134719007371\\
279	1.59300429922423\\
280	1.6012301269679\\
281	1.60776926802547\\
282	1.61349162310746\\
283	1.61883156030981\\
284	1.62400743961704\\
285	1.62913043598613\\
286	1.63566656278664\\
287	1.64156801142306\\
288	1.64715030451777\\
289	1.66736201054933\\
290	1.68590767586163\\
291	1.70112653188321\\
292	1.71290858129956\\
293	1.72234696003985\\
294	1.73431485011341\\
295	1.74563709394311\\
296	1.75561865734593\\
297	1.76440276011541\\
298	1.78043111241039\\
299	1.79739299167448\\
300	1.81315329144765\\
301	1.82687258180259\\
302	1.83856122392891\\
303	1.84856443908105\\
304	1.85729428280738\\
305	1.86511687823429\\
306	2.02120519592218\\
};
\addlegendentry{\lblMVAmeb{2}}


\addplot[area legend, draw=none, fill=mycolor2, fill opacity=0.1]
table[row sep=crcr] {%
x	y\\
1	200.891604267966\\
2	41.2503551191357\\
3	49.265713028603\\
4	45.8607945483113\\
5	43.5436595818258\\
6	38.9578956835843\\
7	35.0518597977636\\
8	30.8346410266958\\
9	27.5852661794331\\
10	22.5782939668552\\
11	19.157810077207\\
12	16.7225540913786\\
13	15.1665015960298\\
14	14.5928151983554\\
15	16.5099882354157\\
16	14.0492975177032\\
17	13.8405404990398\\
18	13.5560937767522\\
19	15.0087506025716\\
20	12.1520753013163\\
21	12.845347979767\\
22	11.7907604563247\\
23	10.5746370789827\\
24	11.7066419878353\\
25	11.3142417674507\\
26	12.3351440773821\\
27	12.3223765621757\\
28	11.4497102447781\\
29	11.049948189239\\
30	11.4099956024261\\
31	11.7931610478078\\
32	12.1090350553721\\
33	11.455524715113\\
34	11.2928818886426\\
35	12.0352127337855\\
36	10.8914456616776\\
37	10.8867201715583\\
38	10.8264567550409\\
39	10.7638359565559\\
40	9.27060892365932\\
41	9.42279976465093\\
42	9.27105115780017\\
43	8.36411971470752\\
44	8.5735124212057\\
45	7.58818809447815\\
46	7.40585032949165\\
47	7.63820218871713\\
48	7.28394012970661\\
49	8.02275112234955\\
50	7.4734073936012\\
51	7.89300935292094\\
52	7.87658039193955\\
53	8.04509485137071\\
54	8.92781589537574\\
55	8.81562524826453\\
56	8.63720147328659\\
57	8.79863546809072\\
58	9.36989243227516\\
59	9.41763869858877\\
60	8.64825829083476\\
61	8.70298401156568\\
62	9.23122522087756\\
63	9.35945866659095\\
64	9.21228558130151\\
65	8.97928855739847\\
66	9.86300190721963\\
67	9.44178741424858\\
68	10.264493670775\\
69	10.4964120245549\\
70	10.2019407677693\\
71	9.75649519086477\\
72	10.8206854912987\\
73	9.83772868965247\\
74	9.97190374975859\\
75	10.5768118748413\\
76	8.99164389057774\\
77	9.13908301177452\\
78	8.54916457345908\\
79	8.42796913249865\\
80	7.83798165494546\\
81	8.00209948873692\\
82	7.31791182223998\\
83	6.83656025331527\\
84	7.25020912505305\\
85	6.38692780294459\\
86	6.97640480036257\\
87	6.5217920555833\\
88	6.9059352755541\\
89	5.77590156044024\\
90	6.47764327060183\\
91	6.57172137194441\\
92	6.94309748279486\\
93	5.86448334036411\\
94	6.04455909421899\\
95	6.81894522122092\\
96	6.85098090770522\\
97	5.9119720437147\\
98	6.51750401934438\\
99	6.35601732286711\\
100	6.03879521583835\\
101	6.69947820521844\\
102	5.40970887271935\\
103	5.71503293719351\\
104	6.38441898843357\\
105	6.81331492493261\\
106	6.10696274832258\\
107	6.79350845484724\\
108	6.64775720902279\\
109	6.09748450146595\\
110	5.9149854572448\\
111	6.41445915149415\\
112	6.62740000277372\\
113	6.61544519750223\\
114	6.41670408436757\\
115	5.73255307988526\\
116	6.75552510485803\\
117	6.89341951996805\\
118	6.64478731239357\\
119	6.51513561073596\\
120	6.17564681415318\\
121	6.17589784690615\\
122	7.36095455950557\\
123	7.06171578441317\\
124	5.96195879925857\\
125	6.01425270564606\\
126	5.3162458705949\\
127	6.00095017851553\\
128	5.5349475074559\\
129	5.44848283819354\\
130	5.23540721870013\\
131	5.36361677683426\\
132	5.52487429293319\\
133	5.14906873684618\\
134	5.34450950819059\\
135	4.81884240443563\\
136	4.94859442670886\\
137	5.33895753147796\\
138	4.92346909729834\\
139	4.88974480548253\\
140	5.1607359417212\\
141	4.69124251597193\\
142	4.53329203255803\\
143	4.9211827505833\\
144	4.79248971648978\\
145	5.24726708465572\\
146	4.81873756961008\\
147	4.53545987265882\\
148	5.64747118087287\\
149	5.10770639387176\\
150	4.53916514801566\\
151	4.84517085837618\\
152	4.80904433610666\\
153	5.47101538343174\\
154	5.19418833561785\\
155	4.81569743324689\\
156	4.43881436268956\\
157	4.8064513746891\\
158	4.58585256259697\\
159	5.01355344257613\\
160	4.80724384004805\\
161	4.59085655469075\\
162	4.22189412442393\\
163	5.80793379502121\\
164	5.12426588932649\\
165	4.88763346327214\\
166	5.41920696159412\\
167	5.13455794210074\\
168	4.89563283455809\\
169	5.04826593810835\\
170	4.99524036803798\\
171	4.29837919116987\\
172	4.01498097676625\\
173	4.12858809210951\\
174	4.25225942823059\\
175	3.50899741200371\\
176	3.68061670127014\\
177	3.94834081900048\\
178	3.52597984455346\\
179	3.73125418944972\\
180	3.3198514576089\\
181	4.14893975236039\\
182	3.8106776188878\\
183	4.38807527398287\\
184	4.09745344065008\\
185	5.74002836021711\\
186	5.71027249508737\\
187	6.76076518245813\\
188	7.08006026859421\\
189	7.80548842922798\\
190	8.2755469137404\\
191	8.88176033789836\\
192	9.06895019825361\\
193	9.16302889021251\\
194	9.44432527479881\\
195	10.1973744925554\\
196	11.1673943174011\\
197	11.3429405528835\\
198	11.1711433493822\\
199	11.0952463003505\\
200	11.0602843096357\\
201	10.9834592153346\\
202	11.3845778198021\\
203	10.7427881722822\\
204	12.645086588893\\
205	13.2860912965196\\
206	12.4190759017955\\
207	12.4131589315187\\
208	13.4187732643655\\
209	11.1493573441729\\
210	11.4658634592649\\
211	10.8443032704728\\
212	10.3465610827555\\
213	9.14810657955791\\
214	9.43180716474248\\
215	8.36538431544482\\
216	8.10035791487925\\
217	8.5377740440102\\
218	8.88772591491919\\
219	7.83743463310745\\
220	6.97599084693914\\
221	6.75046053118496\\
222	6.90299232936753\\
223	6.99845482127391\\
224	6.14579823366402\\
225	6.21104781415076\\
226	7.11288331706204\\
227	7.16394387579515\\
228	6.18856466229297\\
229	6.78907880245922\\
230	7.67753210636414\\
231	7.47613337496652\\
232	7.79190521936901\\
233	8.15068284017283\\
234	8.62635847093016\\
235	7.95987551415576\\
236	8.20960056696999\\
237	8.11955047715966\\
238	7.94819171430752\\
239	8.08799594416739\\
240	7.92289131138194\\
241	7.72976599338246\\
242	8.36920473671373\\
243	8.61001543596498\\
244	8.73659755281909\\
245	8.36094721792844\\
246	8.62238028918986\\
247	8.48469520942638\\
248	9.02903943970504\\
249	9.17487125786456\\
250	9.79376932476201\\
251	9.36962512026266\\
252	9.10372059559685\\
253	8.35285292763354\\
254	8.54998275067363\\
255	8.76598401416959\\
256	9.01334447522913\\
257	9.23875847362073\\
258	9.15120395950071\\
259	9.87866489560997\\
260	9.78501663009235\\
261	10.927799328472\\
262	10.4683026402603\\
263	10.1465086417728\\
264	10.4075800286249\\
265	10.2972295842137\\
266	11.516803928872\\
267	12.2879251971345\\
268	11.9669147383709\\
269	12.6212595541933\\
270	12.1615319303833\\
271	12.1867349908473\\
272	11.9394057210467\\
273	12.3067451620091\\
274	12.2754520223601\\
275	12.567457657568\\
276	10.7024589923811\\
277	7.92835768245387\\
278	6.49791230319012\\
279	5.56170308453166\\
280	5.186148753304\\
281	5.03008996819421\\
282	5.17687072219237\\
283	5.15035318079776\\
284	4.67574162977858\\
285	4.69922141681803\\
286	4.9537608995116\\
287	4.36513734123569\\
288	4.92806179513882\\
289	4.11088639506766\\
290	4.54070207363253\\
291	4.50183759184327\\
292	4.37768888410314\\
293	4.19230703343686\\
294	5.17657245515403\\
295	5.20601611183724\\
296	4.41927207222434\\
297	5.07255220158112\\
298	4.46369239477098\\
299	4.69627914439165\\
300	4.60435646300446\\
301	4.69403482794328\\
302	4.49149410256868\\
303	4.33847468294108\\
304	4.44605586837992\\
305	5.15046271987272\\
306	4.27548056700241\\
306	0.770488611519348\\
305	0.751677601263516\\
304	0.588771837819709\\
303	0.757813696230969\\
302	0.711816204400881\\
301	0.637447029133897\\
300	0.624548988632287\\
299	0.563944337614803\\
298	0.697088476069774\\
297	0.75738249057484\\
296	0.578346976034719\\
295	0.674794426888245\\
294	0.572770062069586\\
293	0.566581766904105\\
292	0.62778404734375\\
291	0.653081472875926\\
290	0.500737876489739\\
289	0.69260038202166\\
288	0.403361511870104\\
287	0.832306019747225\\
286	0.728036114319797\\
285	0.715362889767273\\
284	0.615566819565099\\
283	0.757798755953339\\
282	0.846992691107677\\
281	0.851033968723918\\
280	0.77566082156808\\
279	0.599648879119232\\
278	0.906907093123961\\
277	1.10785317040307\\
276	1.64195388318499\\
275	2.44999347681257\\
274	2.23863944050458\\
273	1.71927963215069\\
272	1.84013658669776\\
271	2.16326122555697\\
270	2.33037052431453\\
269	2.28449838685091\\
268	1.97233945530897\\
267	1.75966959430324\\
266	1.78254244687062\\
265	1.96285447966996\\
264	1.45808700656121\\
263	2.03126870689582\\
262	1.6438249463622\\
261	1.57519553621467\\
260	1.85637791909061\\
259	1.69744852970948\\
258	1.97702657210822\\
257	2.37068811775358\\
256	2.0682014072591\\
255	1.44371587239652\\
254	1.42111472671748\\
253	1.89513322242636\\
252	1.74601807286499\\
251	1.82832609222049\\
250	1.90388317237614\\
249	1.70032389436925\\
248	1.93581775597429\\
247	1.56787824485292\\
246	1.69453888504063\\
245	1.93921434818446\\
244	2.05594802676742\\
243	1.82145262634779\\
242	1.26784562393489\\
241	1.91069638517838\\
240	1.62943276853468\\
239	1.41126757913419\\
238	1.20656622446592\\
237	1.20253860369005\\
236	1.42589850334617\\
235	1.4110082320904\\
234	1.44606083402419\\
233	1.10302514787608\\
232	1.22562715157603\\
231	1.31792475267594\\
230	1.31503280800937\\
229	1.29160020506278\\
228	1.59378181433925\\
227	1.17364969653544\\
226	1.36924565048223\\
225	1.44656344070758\\
224	1.49266958864058\\
223	1.12583061916618\\
222	1.12521877705541\\
221	1.27209128960204\\
220	1.67609479625953\\
219	1.09991303014574\\
218	0.970638928249745\\
217	1.14935985561472\\
216	1.2768480619069\\
215	1.36838463488214\\
214	1.50276703416797\\
213	1.7509782369874\\
212	1.68280035803015\\
211	1.85210847218755\\
210	1.82181600584591\\
209	2.01772819924522\\
208	3.22993347661293\\
207	2.99992134385455\\
206	2.17995095230439\\
205	2.15270305871067\\
204	2.53457843257829\\
203	2.90884970131204\\
202	2.10798978528209\\
201	2.37219213178054\\
200	1.88001550245285\\
199	1.73085690640045\\
198	2.16161297837134\\
197	2.4012263964113\\
196	2.00077050422184\\
195	1.84553329160558\\
194	1.8076792244674\\
193	2.03233877395415\\
192	1.95749819620638\\
191	1.88609595269595\\
190	2.0124380832793\\
189	1.27834669720223\\
188	1.51197690308565\\
187	1.19263426649903\\
186	1.34926515560302\\
185	0.855680669410025\\
184	0.575312999164141\\
183	0.794356040467426\\
182	0.585950246858576\\
181	0.77956761840799\\
180	0.548982593559581\\
179	0.647777019267671\\
178	0.583126650904468\\
177	0.704247112570423\\
176	0.820163182274298\\
175	0.556905681100975\\
174	0.707470109393675\\
173	0.59082940808868\\
172	0.814445468117632\\
171	0.513785051394032\\
170	0.959913367418458\\
169	0.88814433849481\\
168	1.10824909853351\\
167	0.751045960779399\\
166	0.746360937210995\\
165	0.628910388984176\\
164	0.81371631002116\\
163	0.673766682711785\\
162	0.744911707262104\\
161	0.797220168653469\\
160	0.795894791321178\\
159	0.741943558187961\\
158	0.759997987774655\\
157	0.755833398845146\\
156	0.776228768938519\\
155	0.702726714958257\\
154	0.891835221819421\\
153	0.601590457138032\\
152	0.91408102852846\\
151	0.970475175070299\\
150	0.794967532372797\\
149	0.902009773340987\\
148	1.00416005353396\\
147	0.764119812281821\\
146	0.809762448837274\\
145	0.689618301162427\\
144	0.618293389954029\\
143	0.86698851242018\\
142	0.473314546644423\\
141	0.762135990567047\\
140	0.850955740510836\\
139	0.790743996971057\\
138	1.0353151533882\\
137	0.741927624806649\\
136	0.814456824646356\\
135	0.733351743394159\\
134	0.724832149782865\\
133	0.585825131853876\\
132	0.70968837782344\\
131	0.931603916195415\\
130	1.01584498931757\\
129	0.97023085391154\\
128	0.93329245003882\\
127	0.839890863802914\\
126	1.03635943287011\\
125	1.14420301023228\\
124	1.07281705395687\\
123	0.845107794822991\\
122	0.869771365335141\\
121	1.10186936383741\\
120	0.729264332370821\\
119	0.784404104232143\\
118	0.997473867951904\\
117	0.984060408238826\\
116	1.10758336400927\\
115	1.0415234599724\\
114	0.831068066882673\\
113	0.945507102075145\\
112	0.614312244620897\\
111	0.768486965873082\\
110	1.00664973648018\\
109	0.904947179478244\\
108	0.939099769011756\\
107	0.660566671357989\\
106	1.02586100855687\\
105	0.909629512881617\\
104	0.845442030911909\\
103	0.824098604761316\\
102	0.820077267615487\\
101	0.81130974295904\\
100	0.895808096778947\\
99	0.773955755411271\\
98	0.628945502417319\\
97	0.766460764139813\\
96	0.815824935954925\\
95	0.86583520615579\\
94	0.898999529922672\\
93	0.744262499812055\\
92	0.829643977434072\\
91	0.97932214568902\\
90	1.14510194727574\\
89	0.780861730199955\\
88	0.833121246489402\\
87	0.968589546284067\\
86	0.778592290375068\\
85	1.11018410154717\\
84	0.96491006917647\\
83	1.18275542657674\\
82	1.15066203885602\\
81	1.24163364544854\\
80	1.53232077124375\\
79	1.89020030668069\\
78	1.15000830555418\\
77	1.57863833319861\\
76	1.50309613294684\\
75	1.72726119749145\\
74	1.60982990692823\\
73	1.65674676811431\\
72	1.38726870048042\\
71	1.44515792298284\\
70	1.2137416955617\\
69	1.40587760036086\\
68	1.15775184514232\\
67	1.1983968367616\\
66	1.10131884637873\\
65	1.18199138944251\\
64	1.09123395072994\\
63	0.933503113382779\\
62	1.25265948423038\\
61	0.812645518974946\\
60	0.97653001276664\\
59	1.030687365906\\
58	0.932611058663868\\
57	1.11319182457116\\
56	1.17102896794755\\
55	1.00240311195139\\
54	0.975502597414279\\
53	1.45248519599582\\
52	1.0311559035163\\
51	0.94688096308494\\
50	0.818711960266413\\
49	1.04923037705283\\
48	1.05933335335827\\
47	1.15661270380487\\
46	1.40266508077145\\
45	1.16355225441659\\
44	1.19099951991422\\
43	1.12429516961459\\
42	1.39891328858958\\
41	1.0430540677129\\
40	1.12621886062906\\
39	0.901933014735316\\
38	1.22957524885921\\
37	1.22701967991223\\
36	1.46407815608654\\
35	1.13413162992888\\
34	1.3291328218648\\
33	1.70129830425582\\
32	1.64632923612906\\
31	1.56818447342742\\
30	2.2147633158041\\
29	1.97893775332738\\
28	1.86640400694465\\
27	1.46376761153199\\
26	1.46404297042385\\
25	1.75351737905336\\
24	1.50060825478926\\
23	1.16534066145387\\
22	1.12447937346032\\
21	1.76526698868214\\
20	1.88142909542963\\
19	1.19995805515276\\
18	1.17026279142613\\
17	0.872182794080811\\
16	1.08619748264513\\
15	1.6824635048036\\
14	1.9179849868172\\
13	1.53457029943573\\
12	1.37592038922396\\
11	1.49395505919536\\
10	1.48835550486024\\
9	1.56174753637129\\
8	1.78267816776345\\
7	1.77710853205231\\
6	1.91804662766592\\
5	1.98307343665021\\
4	2.0545665822083\\
3	2.60288556346081\\
2	2.99582115538639\\
1	13.2677248180713\\
}--cycle;
\addlegendentry{\lblMVAuncertainty{2}}


==> figures/MVA-5-subplots/MVA-5plot-s3.tex <==
\addplot [color=IEEEblue, dashed, line width=\LWestimates]
  table[row sep=crcr]{%
1	39.0612032105767\\
2	27.5683051596618\\
3	28.4520185210869\\
4	24.6941974961441\\
5	24.3823820781378\\
6	24.7742416152732\\
7	26.8643091730127\\
8	23.7451392705875\\
9	24.3732370954985\\
10	24.2773952081768\\
11	24.1636958698249\\
12	25.090987269315\\
13	25.9001854964034\\
14	25.0821780586664\\
15	24.821646639089\\
16	24.1674218691706\\
17	24.5772263804647\\
18	24.4799650988314\\
19	24.1671278178649\\
20	24.1122438295704\\
21	24.2255207466655\\
22	24.0354100880249\\
23	23.8876216230318\\
24	24.0587743573922\\
25	23.9712379304218\\
26	23.9136490635826\\
27	23.5256410232926\\
28	22.701046144732\\
29	23.4866676060819\\
30	23.1484641057508\\
31	22.3574089144985\\
32	22.5366631974432\\
33	22.8444294090444\\
34	22.8398077342559\\
35	22.1105614157091\\
36	22.1924032558978\\
37	22.1966290876125\\
38	22.0196473298608\\
39	21.3498932097297\\
40	21.0420677063602\\
41	20.8983650146476\\
42	21.0554870668032\\
43	20.8661278294366\\
44	20.3289822053088\\
45	20.4239702197241\\
46	20.281664032811\\
47	21.72995882227\\
48	21.4137801611782\\
49	21.2852833022755\\
50	21.5595151262261\\
51	21.5623732695278\\
52	21.6946973860428\\
53	21.7224801112891\\
54	21.7905852400185\\
55	21.8083503851959\\
56	21.7892091681385\\
57	21.7005314121129\\
58	21.601192381569\\
59	21.7105844381828\\
60	21.7657214219149\\
61	22.1478014868879\\
62	22.4010259273026\\
63	22.3264208981887\\
64	22.2782292940322\\
65	22.4843523165984\\
66	22.227390714638\\
67	22.102620004171\\
68	21.7183804421725\\
69	21.962135455992\\
70	21.0133649203316\\
71	21.0788475938491\\
72	20.9386418198023\\
73	21.1681122988693\\
74	21.0977618163895\\
75	21.2940295726944\\
76	20.9806279050127\\
77	20.9044653329415\\
78	20.6137307706901\\
79	20.8313210496416\\
80	20.985319833285\\
81	21.1527539933315\\
82	21.1267082000254\\
83	20.9718975634782\\
84	20.7481827477597\\
85	20.4188065007665\\
86	20.6816274826375\\
87	20.3176003227974\\
88	20.2765882769025\\
89	20.1687462411366\\
90	20.0925824424615\\
91	20.0037440729422\\
92	20.3870456327233\\
93	20.4195289769029\\
94	20.5341737644589\\
95	20.6043234560737\\
96	20.469418462194\\
97	20.5274971224367\\
98	20.5424319249421\\
99	21.1748691883508\\
100	20.8034765236322\\
101	20.7449904126915\\
102	20.9962897546105\\
103	20.9816136084625\\
104	20.7969139022816\\
105	21.1544546033393\\
106	21.0060078752897\\
107	20.8756063846642\\
108	20.8304895191275\\
109	20.7848091225084\\
110	20.7341079283495\\
111	20.6454885324\\
112	20.6867388714803\\
113	20.9064373959189\\
114	20.7392519384583\\
115	21.2680842015328\\
116	21.4117282537387\\
117	21.2807312963655\\
118	21.4802479632185\\
119	21.0022210847275\\
120	21.302686725007\\
121	21.0918588870932\\
122	20.0674087653329\\
123	18.8473314008399\\
124	17.6211354377216\\
125	16.2755406714161\\
126	15.6692303235103\\
127	14.1321709501406\\
128	12.9384536454096\\
129	11.9841762364631\\
130	11.1434332585426\\
131	10.0758007339358\\
132	9.28924777934463\\
133	8.19317259491476\\
134	7.06624193104055\\
135	6.63872624785484\\
136	6.08060633840228\\
137	5.71475832868382\\
138	5.14798555063152\\
139	4.90520841846866\\
140	4.26184167531296\\
141	4.40094499869485\\
142	4.28897503646446\\
143	4.05589926317572\\
144	3.81556622253017\\
145	3.81550187509008\\
146	3.43390241683666\\
147	3.84841792055957\\
148	3.46311228481908\\
149	3.97204097017609\\
150	3.57661169889689\\
151	3.61956005537532\\
152	3.59620289798097\\
153	3.68067144150737\\
154	3.04783229694374\\
155	3.54764414002486\\
156	3.6181072762441\\
157	3.48319092519451\\
158	3.17802009757165\\
159	3.23223887799687\\
160	3.08135798221431\\
161	3.19029737270913\\
162	3.17056800785583\\
163	3.47442833238293\\
164	2.9182655606175\\
165	3.0743360445919\\
166	2.92699597443793\\
167	3.31925893573757\\
168	3.04895389050057\\
169	2.88058272746801\\
170	2.6807501289545\\
171	3.30972875110217\\
172	3.13838108570546\\
173	2.92477647998593\\
174	3.26188034192147\\
175	3.05484440418553\\
176	2.92457677032728\\
177	2.3844109035975\\
178	3.23308728450304\\
179	3.17579968320224\\
180	3.18607691041909\\
181	2.99320307429702\\
182	3.12031036133284\\
183	3.60933783995442\\
184	3.65530408325099\\
185	3.5176217141737\\
186	3.2932383243706\\
187	3.37788074377647\\
188	3.16870374060869\\
189	3.24534420816525\\
190	2.79167781761891\\
191	3.28120431877002\\
192	3.25555770030389\\
193	2.9037814228609\\
194	3.07440179445189\\
195	3.1534282372823\\
196	2.52751354452876\\
197	2.86294008385966\\
198	3.11816446716638\\
199	3.10604672073904\\
200	2.90584363673938\\
201	3.1894285225049\\
202	3.16929265201981\\
203	3.31634690495563\\
204	3.47849808570884\\
205	3.29992500835271\\
206	3.48767630443756\\
207	3.55745876869217\\
208	3.94623440567484\\
209	4.21226647548417\\
210	4.3308091556317\\
211	3.8826862961831\\
212	3.44118595574424\\
213	3.73835603478707\\
214	3.82311603078672\\
215	4.15511222282969\\
216	4.25437778245306\\
217	3.39485444562389\\
218	3.85179706455331\\
219	3.93096876908445\\
220	4.06394560315444\\
221	4.33751385472217\\
222	4.04798806625519\\
223	4.16886236375473\\
224	4.65626810800896\\
225	4.26863071762491\\
226	3.93133282401338\\
227	4.08521456873869\\
228	3.71181378183562\\
229	3.97895816420044\\
230	3.73209416277322\\
231	4.27550384686402\\
232	4.31021276868333\\
233	4.55067670011604\\
234	4.31649158344683\\
235	3.94436036513325\\
236	3.96312059596174\\
237	4.10749405417032\\
238	4.5350145843943\\
239	4.36030863968907\\
240	4.28002799325516\\
241	4.09514184850831\\
242	4.43872567942187\\
243	4.15951938610268\\
244	3.54521860195143\\
245	4.0193796810898\\
246	4.13355106328101\\
247	4.3171503604725\\
248	4.58600604570068\\
249	4.49306926627611\\
250	4.26293951837928\\
251	4.11201646461555\\
252	3.74024037370106\\
253	4.02816051430678\\
254	3.86767997155946\\
255	4.65809831662556\\
256	4.09623807717675\\
257	4.13580138344337\\
258	4.70092460162957\\
259	4.1556195450385\\
260	4.08206899169218\\
261	3.91298628179126\\
262	3.80948846117408\\
263	4.59249325803086\\
264	4.5873996678282\\
265	4.58315060942658\\
266	4.59181128621414\\
267	4.14188004740068\\
268	4.14297021748935\\
269	4.25625606980001\\
270	4.84315266324723\\
271	4.24625026165552\\
272	3.76485415480686\\
273	4.3672591002659\\
274	4.6570887640979\\
275	4.70032192827548\\
276	5.07221120986676\\
277	5.46945626523496\\
278	5.51492643965504\\
279	5.38623812301127\\
280	5.16480235521471\\
281	5.48996058134327\\
282	5.40323263512811\\
283	5.89289268383278\\
284	5.79348877250669\\
285	5.72210945806131\\
286	6.20182189609691\\
287	5.74510545699112\\
288	5.66027841550645\\
289	5.25020666198912\\
290	5.56803040660638\\
291	5.27860091230466\\
292	5.00779188860315\\
293	4.72099563651488\\
294	4.71440965144831\\
295	4.47180497411079\\
296	4.90535745633833\\
297	4.9298354560248\\
298	5.10815691537445\\
299	4.95609547289878\\
300	5.05017590326975\\
301	4.92835107728355\\
302	5.37705827477043\\
303	5.07756072846204\\
304	5.30241989831764\\
305	5.57111615948742\\
306	5.98023132447881\\
};
\addlegendentry{\lblMVAest{3}}

\addplot [color=IEEEblue, line width=\LWbound]
  table[row sep=crcr]{%
1	2.48892040610815\\
2	2.25873389469024\\
3	2.13626160518158\\
4	2.06788153574396\\
5	2.02887281513673\\
6	2.00652024919158\\
7	2.00363310613061\\
8	2.00892414512592\\
9	2.01562569173566\\
10	2.02180246682564\\
11	2.0272211709652\\
12	2.03174529954425\\
13	2.0353655300023\\
14	2.03814634311902\\
15	2.04019118260123\\
16	2.04161786626798\\
17	2.04254101739524\\
18	2.04306323509101\\
19	2.04327137848018\\
20	2.04271274835654\\
21	2.04150213315793\\
22	2.0397328473134\\
23	2.03747035564156\\
24	2.03476517186425\\
25	2.03174472243787\\
26	2.02841681940193\\
27	2.02478039812192\\
28	2.02084714785637\\
29	2.03368879880803\\
30	2.04836472586234\\
31	2.06136363749449\\
32	2.07182034203307\\
33	2.07958898866855\\
34	2.08473116127201\\
35	2.08643802162993\\
36	2.0853980041552\\
37	2.08216719140408\\
38	2.08394692504039\\
39	2.08372073854257\\
40	2.08209752103737\\
41	2.07947739105661\\
42	2.07613685824552\\
43	2.07226809127115\\
44	2.0680091605261\\
45	2.06346096947915\\
46	2.05869845061682\\
47	2.05377796114436\\
48	2.04874234763063\\
49	2.04362448997799\\
50	2.03844983060999\\
51	2.03323820878085\\
52	2.02029906412606\\
53	2.01261443990008\\
54	2.00639454217438\\
55	2.00104647077736\\
56	2.00046517418504\\
57	1.99993413041651\\
58	1.99899613285703\\
59	1.99751588973195\\
60	1.99549581458295\\
61	1.99299510486964\\
62	2.00448970325057\\
63	2.00854886699326\\
64	2.00955900200869\\
65	2.00917724589188\\
66	2.00777207166767\\
67	2.00563648912947\\
68	2.00294996564354\\
69	1.99984541831304\\
70	1.99642264448573\\
71	1.99275989702078\\
72	1.98891897277095\\
73	1.98494899211495\\
74	1.98088897003588\\
75	1.97676986154309\\
76	1.97261618289751\\
77	1.95711260554744\\
78	1.93145234141746\\
79	1.91568439747197\\
80	1.9051047045967\\
81	1.89695848180373\\
82	1.89021228512398\\
83	1.88446665324642\\
84	1.87947279644736\\
85	1.8750507134311\\
86	1.87106493904432\\
87	1.86741328379569\\
88	1.86401930113641\\
89	1.86082634434795\\
90	1.85779284366643\\
91	1.85488855762412\\
92	1.85209165219819\\
93	1.84938645972671\\
94	1.84702088853244\\
95	1.8448608216457\\
96	1.8428697914385\\
97	1.84102755635946\\
98	1.83932721447109\\
99	1.83776779813959\\
100	1.8363508639704\\
101	1.83507907304984\\
102	1.8339570979177\\
103	1.82208057677665\\
104	1.81392659204685\\
105	1.80592074603796\\
106	1.80135224735596\\
107	1.79841649411079\\
108	1.79653959691206\\
109	1.79540224073599\\
110	1.79480543935445\\
111	1.7946186990445\\
112	1.79475333533546\\
113	1.79514751618256\\
114	1.80530729436851\\
115	1.81490686967822\\
116	1.82159500184501\\
117	1.82636762777698\\
118	1.83012627598558\\
119	1.83327920792033\\
120	1.83514815883974\\
121	1.83740904014513\\
122	1.84548658924956\\
123	1.857012024685\\
124	1.90343008585073\\
125	1.93319992861646\\
126	1.94994151817355\\
127	1.96432032867884\\
128	1.9743197650979\\
129	1.98130073288091\\
130	1.98630319076359\\
131	1.99002526473643\\
132	1.99292585499341\\
133	1.99530291616941\\
134	1.99731784569888\\
135	1.9990029906095\\
136	2.00507580763972\\
137	2.01101674882874\\
138	2.01680739727457\\
139	2.02247701794908\\
140	2.02718543705358\\
141	2.03226794346541\\
142	2.03737664688612\\
143	2.04242706937127\\
144	2.04737068468928\\
145	2.05216173068715\\
146	2.05675650178075\\
147	2.06111301635018\\
148	2.06519144978595\\
149	2.06843533925114\\
150	2.07153636956791\\
151	2.07436986695866\\
152	2.07686549968588\\
153	2.07898024429561\\
154	2.08081680068359\\
155	2.0824353116793\\
156	2.08390737304993\\
157	2.08507985646821\\
158	2.08628113287153\\
159	2.09197313869123\\
160	2.09723575641949\\
161	2.10170757218796\\
162	2.10535056468294\\
163	2.10827045546681\\
164	2.11061220677785\\
165	2.112513495857\\
166	2.11408850075854\\
167	2.11542591415669\\
168	2.11218439689022\\
169	2.11064298327195\\
170	2.10984554663076\\
171	2.1062922473715\\
172	2.10501687785218\\
173	2.10460611180117\\
174	2.10590455232207\\
175	2.10719532049611\\
176	2.10632346591495\\
177	2.10600130920703\\
178	2.10605959363084\\
179	2.1063897099367\\
180	2.10691294716107\\
181	2.10794990835273\\
182	2.12210010497192\\
183	2.1347705707771\\
184	2.14482129019368\\
185	2.1507680981803\\
186	2.15612888981926\\
187	2.16733481829786\\
188	2.17506859538306\\
189	2.18035986448033\\
190	2.18403176340924\\
191	2.18661180591108\\
192	2.18848768305738\\
193	2.18991188427261\\
194	2.19104725284417\\
195	2.19199703079718\\
196	2.19282675252737\\
197	2.1935780978813\\
198	2.1942777322598\\
199	2.19494283203156\\
200	2.19558455452552\\
201	2.19621021788717\\
202	2.19682467793214\\
203	2.19743120177404\\
204	2.20073876958624\\
205	2.20499707585778\\
206	2.20988891713815\\
207	2.21481557418862\\
208	2.22007089798868\\
209	2.40151421256874\\
210	2.5617115817534\\
211	2.70412042316556\\
212	2.83119642418436\\
213	2.94495659162155\\
214	3.04686555889805\\
215	3.13831441842845\\
216	3.22053943645212\\
217	3.29463039808802\\
218	3.36154903293515\\
219	3.42214426420538\\
220	3.47412189417427\\
221	3.52235483663097\\
222	3.56659271127518\\
223	3.60717865526923\\
224	3.64451037353215\\
225	3.67896668397802\\
226	3.71088961948493\\
227	3.74032296402015\\
228	3.76723160434684\\
229	3.79155810621431\\
230	3.81323561930722\\
231	3.8321942756493\\
232	3.8483668283882\\
233	3.86169387144365\\
234	3.87212863941845\\
235	3.87964134569603\\
236	3.88422298859566\\
237	3.88588853801678\\
238	3.88495510177533\\
239	3.88173393632206\\
240	3.87651362023909\\
241	3.86955745604033\\
242	3.86110439401764\\
243	3.85137027768935\\
244	3.84054920758476\\
245	3.8288149737454\\
246	3.81632252250826\\
247	3.80320942609701\\
248	3.78959732923522\\
249	3.77559335219254\\
250	3.7612914347122\\
251	3.74677360968096\\
252	3.73211119917884\\
253	3.71736592868104\\
254	3.72860496666491\\
255	3.73688546858911\\
256	3.7426904161438\\
257	3.74611541984737\\
258	3.7478259603832\\
259	3.74791405614714\\
260	3.74659558545992\\
261	3.74407353355568\\
262	3.74052731031214\\
263	3.73611433323029\\
264	3.60439307352075\\
265	3.57858799654955\\
266	3.5454476043833\\
267	3.5168700462973\\
268	3.49347906697424\\
269	3.47424082650972\\
270	3.45822063158418\\
271	3.4447297283294\\
272	3.43326501864714\\
273	3.42344394572194\\
274	3.41496924161078\\
275	3.40760630404612\\
276	3.40278353609579\\
277	3.40120145860976\\
278	3.39874830695869\\
279	3.39625521119186\\
280	3.39392181692706\\
281	3.3917542591182\\
282	3.38972396261289\\
283	3.38780301267327\\
284	3.38597014836978\\
285	3.38421009877315\\
286	3.38263595457069\\
287	3.38111044058078\\
288	3.37962210092815\\
289	3.37866281440299\\
290	3.37753986936044\\
291	3.37629728349403\\
292	3.37501084672033\\
293	3.37372053894134\\
294	3.4118425875507\\
295	3.42937674550081\\
296	3.43997893053635\\
297	3.44783537443842\\
298	3.58979092084882\\
299	3.72461509488636\\
300	3.85339895076937\\
301	3.97753085634513\\
302	4.09780213187294\\
303	4.21465316933881\\
304	4.32835492249871\\
305	4.4391049796307\\
306	4.55920204544094\\
};
\addlegendentry{\lblMVAmeb{3}}


\addplot[area legend, draw=none, fill=IEEEblue, fill opacity=0.1]
table[row sep=crcr] {%
x	y\\
1	282.09430521305\\
2	51.5930293330129\\
3	51.8527996064243\\
4	51.3469712295272\\
5	50.3920212030226\\
6	49.8081764014277\\
7	49.2035346209006\\
8	47.0902222463759\\
9	46.486013858044\\
10	47.847801722253\\
11	46.074885207075\\
12	46.7136696722405\\
13	44.7998095154384\\
14	43.6813570608341\\
15	42.1822207227006\\
16	42.321441252236\\
17	42.0885842599348\\
18	41.8750440403233\\
19	41.7811295026608\\
20	42.1386194314218\\
21	43.1396961593315\\
22	41.9221746576365\\
23	41.0924853228699\\
24	40.9234342677835\\
25	40.9696753595142\\
26	41.6068041770238\\
27	40.1376328103777\\
28	39.0995326115654\\
29	41.9087611938883\\
30	40.4321308584269\\
31	39.1716031450662\\
32	39.6443768028246\\
33	38.5176015203097\\
34	38.8987597213867\\
35	38.8403681206802\\
36	38.3268793106817\\
37	37.2016815113993\\
38	36.9176133545128\\
39	35.2421674396495\\
40	34.5180537015268\\
41	34.4609310943448\\
42	34.698458054034\\
43	34.5421063692607\\
44	34.770220756572\\
45	35.2650151368987\\
46	36.0586366379308\\
47	35.1160759055088\\
48	34.2127128038687\\
49	34.9900169857711\\
50	35.4939910343513\\
51	34.2815412527457\\
52	35.526214360733\\
53	35.5238145521028\\
54	36.1756402632998\\
55	35.5496245783363\\
56	36.4531185564097\\
57	35.5607785465169\\
58	32.6902758029206\\
59	33.6579514757436\\
60	34.0133957223521\\
61	35.2595722386984\\
62	35.847953217332\\
63	34.9795372042884\\
64	36.0615175913741\\
65	36.697541670051\\
66	36.2006165638651\\
67	36.4860984863927\\
68	36.0838597610374\\
69	35.7106495824681\\
70	35.7955252625102\\
71	37.1231733683962\\
72	35.6455615325224\\
73	36.4683102083252\\
74	36.6588356769325\\
75	36.3300616270928\\
76	35.9468962228734\\
77	35.2909432016672\\
78	34.5222595698891\\
79	36.6631636502514\\
80	34.9010278206078\\
81	36.8687205341928\\
82	36.769630936974\\
83	37.0355339241242\\
84	35.8263835135153\\
85	36.0129034034487\\
86	36.587706128807\\
87	36.5985248072732\\
88	35.7132694757033\\
89	35.2526764150036\\
90	35.9356767189941\\
91	35.6013576931632\\
92	36.2072416877742\\
93	35.8591257924203\\
94	34.6049896729914\\
95	34.3644388605306\\
96	35.4535114651836\\
97	35.3531160145816\\
98	35.4803988105547\\
99	36.1236541992417\\
100	35.8857450569309\\
101	34.9946505658701\\
102	36.4155496286006\\
103	37.3601921879766\\
104	36.4536854830488\\
105	34.9925313303243\\
106	35.3631441144569\\
107	34.043609474018\\
108	34.3993095317839\\
109	34.2904929181599\\
110	34.1597333449061\\
111	34.922350723096\\
112	35.046331380028\\
113	34.7714555171269\\
114	34.8905077516626\\
115	35.9540832819627\\
116	36.476592555378\\
117	35.1157077678115\\
118	35.0672735044334\\
119	35.4136894119634\\
120	35.9123069607888\\
121	35.3397483231189\\
122	33.7630128156066\\
123	32.5018507597241\\
124	29.7590303433973\\
125	27.7480054169943\\
126	28.7442418795588\\
127	25.6268315855255\\
128	24.0803890062545\\
129	22.4439105989313\\
130	19.9563010073428\\
131	19.2040642711839\\
132	16.867638636227\\
133	16.6735796064228\\
134	15.2704848016615\\
135	14.1291595605596\\
136	12.2693302611473\\
137	11.2948579443342\\
138	9.25877317837249\\
139	8.66843658097177\\
140	8.74994010440479\\
141	8.26727523922055\\
142	7.31852761494618\\
143	7.50830163568527\\
144	6.41890347952524\\
145	6.80776165299779\\
146	6.3603814685074\\
147	6.91784397117524\\
148	6.01802722936661\\
149	6.66561453229376\\
150	6.16766896247358\\
151	6.11016101533566\\
152	6.30733833115341\\
153	5.77554622629049\\
154	5.58803909634184\\
155	6.04051064033065\\
156	6.40779262857016\\
157	6.25857750047362\\
158	6.30280157962752\\
159	6.31554363679214\\
160	5.34453018432022\\
161	5.90251248280879\\
162	5.02199952483945\\
163	5.631153940972\\
164	5.39925860594624\\
165	5.14462807010283\\
166	5.43863794464454\\
167	5.94306175488083\\
168	5.52147795719378\\
169	4.92062854022275\\
170	5.62417626427144\\
171	5.42865653673132\\
172	5.22872891948173\\
173	5.06986015798272\\
174	5.14096579409332\\
175	5.29348359524796\\
176	5.77865514088979\\
177	5.7832847551598\\
178	5.38725858902345\\
179	5.35250459634254\\
180	5.19596261117675\\
181	5.93955501660372\\
182	6.70642896734407\\
183	6.37267406427211\\
184	6.38061229037045\\
185	6.30897034094525\\
186	5.8274378380976\\
187	5.61364603795504\\
188	5.74837608934393\\
189	5.74846497628351\\
190	5.90135396460323\\
191	5.50697061078596\\
192	5.26469929847916\\
193	5.23769608506198\\
194	5.00737603847602\\
195	5.15379512267274\\
196	5.17065369523527\\
197	4.87425177395868\\
198	5.09173097559254\\
199	5.80916592426774\\
200	5.20658452620126\\
201	5.04154083061685\\
202	5.5530780700573\\
203	5.73002744048656\\
204	5.71276367162425\\
205	5.96738182805728\\
206	5.33607069346337\\
207	5.7256674830821\\
208	6.69977010545945\\
209	6.55882168465893\\
210	7.09374682316311\\
211	6.05466699039718\\
212	6.21907134834127\\
213	6.33785203418023\\
214	6.5763756035745\\
215	7.12532979047324\\
216	6.81534831692917\\
217	6.6276909606412\\
218	6.49791231960907\\
219	6.25563933156334\\
220	6.59869718838629\\
221	7.29485866693148\\
222	7.11153681479149\\
223	6.63500976545599\\
224	7.67951556739586\\
225	7.21778825238335\\
226	6.8582770972497\\
227	7.00630292988893\\
228	6.99141574802491\\
229	7.08475743657352\\
230	7.50312040521947\\
231	7.66279066783143\\
232	7.80788421564692\\
233	7.01522612227948\\
234	7.52868546329757\\
235	6.87581040472492\\
236	6.80955681948575\\
237	7.10060896911186\\
238	7.30335261553421\\
239	6.96958771200453\\
240	8.08918739461466\\
241	8.11712370591681\\
242	8.04207655079662\\
243	6.75398834983955\\
244	8.11793173176365\\
245	7.47951848492587\\
246	7.08576133640623\\
247	7.84975067114431\\
248	7.93882446062241\\
249	7.44835679909262\\
250	7.1808915108833\\
251	6.95936479194743\\
252	6.54060910992692\\
253	6.58595263916939\\
254	6.44052551856796\\
255	7.72843333587759\\
256	7.26465096519747\\
257	8.21555231797556\\
258	7.88029308956251\\
259	7.90256898493333\\
260	6.4194823809039\\
261	7.47577145699527\\
262	6.45989044985487\\
263	7.53614418318431\\
264	8.59301186096423\\
265	8.39072536680983\\
266	7.54219620495887\\
267	7.67466987200242\\
268	7.1655680353697\\
269	7.31403614256332\\
270	8.50445176444995\\
271	7.13478694294976\\
272	7.21759148878035\\
273	7.51949599493532\\
274	8.65263048925546\\
275	7.63410530149921\\
276	8.26793278348071\\
277	9.05528024388214\\
278	9.44427620351309\\
279	9.05790695822339\\
280	9.97944446782661\\
281	9.39813390931642\\
282	9.43606407022391\\
283	10.0394403719151\\
284	9.29452398806013\\
285	10.5280910432955\\
286	10.7214270985611\\
287	9.68370290937427\\
288	8.88878753963402\\
289	9.1778313239103\\
290	10.0008928929744\\
291	8.87351617277145\\
292	8.64202176938802\\
293	8.08607724992079\\
294	8.03530383465067\\
295	8.44024979086722\\
296	8.14273771767598\\
297	9.09933073373331\\
298	8.81985749982174\\
299	9.50382264180012\\
300	9.31770683454557\\
301	9.43884914827553\\
302	9.27823513883173\\
303	8.6427094534484\\
304	8.77441075255828\\
305	9.55101218700299\\
306	10.0413214202883\\
306	1.61176397061291\\
305	1.26691885697955\\
304	0.97118980080843\\
303	1.35352996159279\\
302	1.06068273522418\\
301	0.986793971290453\\
300	0.646425416598582\\
299	1.01672967967644\\
298	0.890511491565875\\
297	0.997113178443985\\
296	1.04746662911918\\
295	0.926629163076732\\
294	1.19525386654846\\
293	0.991990305849307\\
292	1.19682257250498\\
291	1.20437081013496\\
290	1.15016075756874\\
289	1.17194565028001\\
288	1.42587873953944\\
287	0.883389192312852\\
286	1.32006885600237\\
285	1.65883892066037\\
284	1.75514177745523\\
283	1.12406719246355\\
282	1.28090627887168\\
281	1.15159972514166\\
280	1.3680240894084\\
279	1.3595935060046\\
278	1.30352870047599\\
277	1.54958685653014\\
276	1.25068285856459\\
275	1.11922777941594\\
274	1.03761008381453\\
273	0.806719033896731\\
272	0.935674072952775\\
271	1.21682803553177\\
270	1.36354352586026\\
269	1.23893302443147\\
268	0.859742521630859\\
267	0.869469861450112\\
266	1.26788189519957\\
265	1.47206234036419\\
264	1.01779394383885\\
263	1.03757210110844\\
262	0.969797930373811\\
261	1.123837297907\\
260	0.747864130734199\\
259	1.1144304528042\\
258	1.31456918041008\\
257	0.989061272741253\\
256	1.1524295489251\\
255	0.987733396269498\\
254	0.779577694424035\\
253	1.10647198002783\\
252	1.13959132683789\\
251	1.12565048681663\\
250	1.16004356193774\\
249	0.90597283277816\\
248	0.933998858815176\\
247	0.910505493915094\\
246	0.724027239373917\\
245	1.01228103205632\\
244	0.787205697547789\\
243	0.748140129133603\\
242	1.03802142608895\\
241	0.751876921318532\\
240	0.817740742943225\\
239	0.491838005091051\\
238	0.855173800530737\\
237	0.762524135939881\\
236	0.88293734782616\\
235	1.06094425065561\\
234	1.08352141257808\\
233	0.848433865407322\\
232	1.47686893197121\\
231	1.0913711109099\\
230	0.889569023117355\\
229	1.11811920505153\\
228	0.888733153367846\\
227	1.03860446591055\\
226	0.767949652908684\\
225	0.841107302601518\\
224	0.791437916634313\\
223	1.02929741742184\\
222	0.721991294661407\\
221	0.851955475357928\\
220	0.499433519191946\\
219	0.997349637332918\\
218	0.75600890530437\\
217	0.842319428060904\\
216	0.912607770980484\\
215	0.778139812243609\\
214	1.05709886776874\\
213	0.739077099844965\\
212	0.686661718895223\\
211	1.00587934827699\\
210	0.820090333707574\\
209	0.591264531965127\\
208	0.922131164571211\\
207	0.725196932700403\\
206	0.799464783465842\\
205	0.92158347989633\\
204	0.944835523291565\\
203	0.909470851911644\\
202	0.790122081481022\\
201	0.899487968378218\\
200	0.82246964093987\\
199	0.684257154981803\\
198	0.592595320965897\\
197	0.551660950748331\\
196	0.827240780055458\\
195	0.495499014156371\\
194	0.792063665917679\\
193	0.723785634844337\\
192	0.91593910126856\\
191	0.54271594937067\\
190	0.666066708855094\\
189	0.613144105877057\\
188	0.865916424821164\\
187	0.754440063946518\\
186	0.722340360400002\\
185	0.611429041302188\\
184	0.581963795776302\\
183	0.767153628342216\\
182	0.869459973329432\\
181	0.876375843658079\\
180	0.546616477180934\\
179	0.670662779196959\\
178	0.648755323671008\\
177	0.704011793567242\\
176	0.582420421013597\\
175	0.641333354426479\\
174	0.853763044984273\\
173	0.876534168451777\\
172	0.603713174308695\\
171	0.579757950250613\\
170	0.65508586820927\\
169	0.699115623428232\\
168	0.714531349800456\\
167	0.780984315904649\\
166	0.747604396387598\\
165	0.620492696413603\\
164	0.850490004422229\\
163	0.811531167262056\\
162	0.664142823930732\\
161	0.858523306190909\\
160	0.876203446830019\\
159	0.499851360017347\\
158	0.902743784978821\\
157	0.917761288861202\\
156	0.928732042911635\\
155	0.880620959433185\\
154	0.648894905457521\\
153	0.837411355897089\\
152	0.712105405101697\\
151	0.900844787334358\\
150	0.899664512755046\\
149	0.668293134110206\\
148	0.913272644283024\\
147	0.472267129463309\\
146	0.692739839513762\\
145	0.830840350832594\\
144	1.48241872876351\\
143	1.24117745671206\\
142	1.27215084694634\\
141	0.997217523138185\\
140	1.31799859806542\\
139	1.14845719343345\\
138	0.933978337422529\\
137	1.35843482558366\\
136	1.50955814285759\\
135	2.03288406676389\\
134	1.87894130815077\\
133	1.90661491879099\\
132	1.65949742967665\\
131	1.19957329249054\\
130	1.75654640545813\\
129	1.79112514673328\\
128	1.57140952570799\\
127	1.19326934663497\\
126	1.66222380362889\\
125	2.53911300018011\\
124	3.4994342197581\\
123	4.23886599290501\\
122	4.64805150615136\\
121	5.0767650092265\\
120	4.71711886857826\\
119	4.4077986808013\\
118	5.28295735094337\\
117	4.65144046843125\\
116	5.04670207510474\\
115	4.98028163823417\\
114	5.29276860354595\\
113	5.07543483284046\\
112	5.36348905294434\\
111	5.30092107287389\\
110	5.54848683313886\\
109	6.2289787551291\\
108	6.04301130998632\\
107	5.57371520504412\\
106	5.03216669435831\\
105	5.48699785782478\\
104	5.1005331231595\\
103	4.30102256742174\\
102	4.70758168532325\\
101	4.767979806094\\
100	4.36017324298124\\
99	3.97965755233111\\
98	4.0377646082622\\
97	4.47090994377108\\
96	5.12260258262423\\
95	4.94391709284034\\
94	4.03558784855732\\
93	4.55376889584787\\
92	5.36369520078062\\
91	3.86749567625137\\
90	4.347169213799\\
89	4.5235521151141\\
88	4.55329248706904\\
87	4.55277189760359\\
86	4.59416830778788\\
85	4.54293851655938\\
84	5.23603760466309\\
83	5.64290429976352\\
82	4.89308313147412\\
81	5.17300298412422\\
80	4.75078792831362\\
79	3.94926335092258\\
78	5.04952067442968\\
77	4.55226506809989\\
76	3.61206769211636\\
75	3.18939785239595\\
74	4.06534837822586\\
73	4.23457905895434\\
72	3.7823963385164\\
71	4.38008406603059\\
70	4.55125551575836\\
69	4.59170246101693\\
68	4.60123629000206\\
67	3.93669178575774\\
66	4.09150187932668\\
65	3.97123052028166\\
64	4.53560503457695\\
63	4.6133805119163\\
62	5.07802728889037\\
61	5.16149777662214\\
60	5.05681529592036\\
59	4.94030213742619\\
58	4.38162521652918\\
57	5.03790884262732\\
56	3.75000890332573\\
55	3.77692348898982\\
54	4.42984032328093\\
53	3.23223600590574\\
52	4.70930969101189\\
51	4.21474809469067\\
50	4.03095289170485\\
49	3.74442467267887\\
48	3.67788730779603\\
47	3.69445592890295\\
46	4.10033930064206\\
45	3.8189436333445\\
44	4.28714593971314\\
43	3.82505468249846\\
42	3.18923099150283\\
41	3.35886751666877\\
40	4.11586572628011\\
39	4.47398605990343\\
38	4.56545959047364\\
37	4.53988718944997\\
36	4.62555669693976\\
35	4.54971898749202\\
34	4.63269395937067\\
33	4.4231028344155\\
32	5.27363999675846\\
31	4.9046493230152\\
30	4.84574581777574\\
29	4.97261309506406\\
28	5.71266171064614\\
27	5.45048751548303\\
26	5.72143148758499\\
25	6.24187703501731\\
24	6.24675642971466\\
23	5.8888649111743\\
22	5.58914422441533\\
21	5.72522311396479\\
20	5.83409395335891\\
19	5.62331807072841\\
18	5.72659110452119\\
17	5.60070014391223\\
16	6.28895276549015\\
15	5.65082144518713\\
14	5.67251040631793\\
13	4.68317660089986\\
12	5.12312871541274\\
11	4.80647381590912\\
10	4.75277515833493\\
9	6.20475482289382\\
8	5.71899082001777\\
7	5.71597384938086\\
6	4.92088613726532\\
5	6.1649739500342\\
4	4.36817084988671\\
3	5.27530808058818\\
2	5.70767062128974\\
1	5.68000338224855\\
}--cycle;
\addlegendentry{\lblMVAuncertainty{3}}


==> figures/MVA-5-subplots/MVA-5plot-s4.tex <==
\addplot [color=mycolor4, dashed, line width=\LWestimates]
  table[row sep=crcr]{%
1	375.15233052377\\
2	34.7961453907851\\
3	38.4387785620306\\
4	36.9768691190408\\
5	35.3223545641508\\
6	33.5561673971212\\
7	30.0084611762796\\
8	28.0694227762007\\
9	23.9751324507587\\
10	21.0493277062122\\
11	19.9820692625682\\
12	16.3643596451223\\
13	14.6432337323908\\
14	13.3692253447944\\
15	12.0152650174717\\
16	10.3472212896668\\
17	8.78458957800749\\
18	7.81251584286699\\
19	7.65599478367122\\
20	6.7588302395773\\
21	6.55098149521158\\
22	6.18486163692764\\
23	5.63862145803563\\
24	5.56479913840187\\
25	5.25705936554976\\
26	5.28015257904291\\
27	5.15732324657504\\
28	5.37958236658611\\
29	4.94570720810941\\
30	4.95028938653953\\
31	4.53592312121541\\
32	4.46259115236862\\
33	4.31778343633734\\
34	4.9346542386216\\
35	4.81293507521787\\
36	4.56487283119889\\
37	4.37780912465976\\
38	4.79022724248587\\
39	4.27429969751562\\
40	4.5303300041317\\
41	4.37041459380312\\
42	4.20465820021085\\
43	3.99310213639624\\
44	3.99947054419503\\
45	3.81632932926818\\
46	3.65514827633516\\
47	3.85210062156967\\
48	3.47596092770676\\
49	3.55028452573877\\
50	3.71495972785695\\
51	4.07419049326562\\
52	3.60267262853546\\
53	3.48033305996244\\
54	3.7342903361521\\
55	3.48034655693689\\
56	3.75287773879199\\
57	3.30633632555433\\
58	3.26708282736357\\
59	3.87399449321662\\
60	3.9067540246236\\
61	4.39508620280621\\
62	4.15104497723542\\
63	3.99615493658356\\
64	3.74619288574503\\
65	3.61354176984853\\
66	3.68788966048918\\
67	3.47411816036388\\
68	3.69215778792447\\
69	4.13780354301169\\
70	3.45509688997207\\
71	4.06635121870758\\
72	3.83989351961718\\
73	3.58271028797656\\
74	4.11843446463946\\
75	4.13336447899035\\
76	3.9957154766406\\
77	3.96709407562265\\
78	3.81994575726498\\
79	3.80863526117726\\
80	3.79947506864579\\
81	3.73807058936736\\
82	3.41075704224194\\
83	3.32603826426386\\
84	3.807561677457\\
85	3.38385919150451\\
86	3.50386154414701\\
87	4.27990787665521\\
88	3.99984771490908\\
89	3.89704624006277\\
90	3.64946632977367\\
91	3.33002414979529\\
92	3.20943907162878\\
93	3.29244274466178\\
94	3.26153288813754\\
95	3.26059449876374\\
96	3.0734870653697\\
97	3.20249058954307\\
98	3.38593747830402\\
99	3.1169572631753\\
100	2.91972167791595\\
101	3.03315065697455\\
102	3.04245949250704\\
103	3.09346116257598\\
104	3.40312092993913\\
105	3.06407639921868\\
106	3.04779312157502\\
107	3.10460736453831\\
108	3.16638740568859\\
109	3.26360620997577\\
110	3.07765190494305\\
111	2.94636706244935\\
112	3.33857282304026\\
113	3.32653446485921\\
114	3.16261902422558\\
115	3.30630872731094\\
116	3.33109582821041\\
117	3.39771378865743\\
118	3.33356335202025\\
119	3.6012702013355\\
120	3.70179016129699\\
121	4.03243667308293\\
122	4.35601261889479\\
123	4.40605359605263\\
124	4.28300896713292\\
125	4.27769656878303\\
126	4.26650951890851\\
127	4.30466364294654\\
128	4.54314545700824\\
129	4.15230436213619\\
130	4.20786843993332\\
131	4.09791775399882\\
132	4.00773576866039\\
133	3.61115488045678\\
134	3.38282259227207\\
135	3.34727661374503\\
136	3.35692739328874\\
137	3.34222927864963\\
138	3.69961715154685\\
139	3.69799291384743\\
140	3.8515163692498\\
141	3.62949099460595\\
142	3.89810412825975\\
143	4.10173812338683\\
144	4.16956853632561\\
145	3.95710934759154\\
146	4.28485640011051\\
147	4.16376534821129\\
148	4.58379476595383\\
149	4.50290520897368\\
150	4.41127904326749\\
151	4.44143703249699\\
152	4.1395910104138\\
153	4.38271820588698\\
154	4.47525359628416\\
155	4.37799415134125\\
156	4.14509854532678\\
157	4.15647681181519\\
158	4.49716071372478\\
159	4.63956818419428\\
160	4.25854327018666\\
161	3.9376194528748\\
162	4.331771603572\\
163	4.23372238922231\\
164	4.26532929004468\\
165	3.77430075359981\\
166	3.97806812961105\\
167	3.77167834684899\\
168	3.99439321000461\\
169	3.9955343755828\\
170	3.3325888531832\\
171	3.61337890744841\\
172	3.30407547128528\\
173	3.57957125229135\\
174	3.45051946188473\\
175	3.47599095680628\\
176	3.35160355297279\\
177	3.12367882948605\\
178	3.06664086386202\\
179	2.84983609069594\\
180	2.49781905360423\\
181	2.24789479579819\\
182	2.05135407015487\\
183	2.2726010417533\\
184	2.06930334009521\\
185	2.2738113267013\\
186	1.87704533038501\\
187	1.8111960153063\\
188	1.65556197832758\\
189	2.08843031873894\\
190	2.05444519393486\\
191	1.75862087109186\\
192	1.86204255875878\\
193	2.06818044203926\\
194	2.1112764622906\\
195	2.41202598228411\\
196	2.11013311512937\\
197	2.13924246203171\\
198	2.00468567032058\\
199	2.12766704455106\\
200	2.42356407822275\\
201	2.19558718330606\\
202	2.32736409033599\\
203	1.76590456269144\\
204	2.05798759844178\\
205	2.33775311449837\\
206	2.44127556211779\\
207	2.30084698759067\\
208	2.22985233163735\\
209	2.23289431322964\\
210	2.1469310905632\\
211	1.90776275462393\\
212	1.92634134539235\\
213	2.29255230143337\\
214	2.02572524795765\\
215	1.57162247188031\\
216	1.41047229922982\\
217	1.5063055449109\\
218	1.64203042345311\\
219	1.63851539266427\\
220	1.87604487718779\\
221	1.83999208955703\\
222	1.80029953748715\\
223	1.79888968153709\\
224	1.60487895841824\\
225	1.60548527523547\\
226	1.51134665749262\\
227	1.68973008099892\\
228	1.60935811642867\\
229	1.63834037793344\\
230	1.78265572502709\\
231	1.71822568814678\\
232	1.50380355595822\\
233	1.73178783894924\\
234	1.71802988715439\\
235	1.62035750790363\\
236	1.5723958957025\\
237	1.62717997362691\\
238	1.55064576551686\\
239	1.42730291347236\\
240	1.41659981982497\\
241	1.6545118407205\\
242	1.45664601461972\\
243	1.71715125973746\\
244	1.59679004112679\\
245	1.61332967719948\\
246	1.54902709137545\\
247	1.54211985221986\\
248	1.59540317494425\\
249	1.65122757425075\\
250	1.72270124162613\\
251	1.78959621814333\\
252	1.58836245600324\\
253	1.61381321594775\\
254	1.59464748752178\\
255	1.75049821604464\\
256	1.67703042306812\\
257	1.68234290034537\\
258	1.58576099451258\\
259	1.61668861053157\\
260	1.59419001044972\\
261	1.6291764448938\\
262	1.73044183837684\\
263	1.71427180739784\\
264	1.87048773971579\\
265	1.90962678566118\\
266	1.7688265735641\\
267	1.93043480003658\\
268	1.83828956623959\\
269	1.98739334331983\\
270	2.04495087007962\\
271	2.0110006430852\\
272	2.04215956584284\\
273	2.04615097796607\\
274	2.09278927887439\\
275	2.11813541306184\\
276	2.26973427029576\\
277	2.16136730352276\\
278	1.63015513286272\\
279	1.82735095236466\\
280	1.94072661918505\\
281	1.74236924679981\\
282	1.79075437605734\\
283	1.73324738072559\\
284	1.86649212379229\\
285	1.97861814512826\\
286	1.78048234439967\\
287	1.46684337225608\\
288	1.37190952700854\\
289	1.31998705579171\\
290	1.31664367991857\\
291	1.11067188541787\\
292	1.16501219659181\\
293	1.24213585929661\\
294	1.11289182489583\\
295	1.19160804357899\\
296	1.21559774927613\\
297	1.25182123442148\\
298	1.17442541071996\\
299	1.31599531028052\\
300	1.24123876891104\\
301	1.11183131276082\\
302	1.18493897124664\\
303	1.07882105165354\\
304	1.18983817782572\\
305	1.12685968406955\\
306	1.18936947123029\\
};
\addlegendentry{\lblMVAest{4}}

\addplot [color=mycolor4, line width=\LWbound]
  table[row sep=crcr]{%
1	3.69199888901641\\
2	3.07297827886573\\
3	2.73671444441153\\
4	2.5334121385822\\
5	2.40359629302825\\
6	2.31798558728476\\
7	2.26037680526283\\
8	2.22083783188783\\
9	2.19325972315252\\
10	2.1736846617621\\
11	2.15950381882744\\
12	2.14897952390308\\
13	2.14094403160759\\
14	2.13460826163392\\
15	2.12943649768613\\
16	2.1250635660184\\
17	2.12123951208844\\
18	2.11779245719623\\
19	2.11460355449832\\
20	2.11140983049684\\
21	2.10815521833985\\
22	2.10478665621523\\
23	2.10126699751828\\
24	2.09757500182331\\
25	2.09382160146922\\
26	2.08998716601468\\
27	2.08604090706366\\
28	2.08197038741142\\
29	2.07786598209388\\
30	2.07361015638221\\
31	2.06922951097166\\
32	2.06475329922208\\
33	2.060209289125\\
34	2.05562368727877\\
35	2.05052096448433\\
36	2.04512944622712\\
37	2.03956599663065\\
38	2.033856512032\\
39	2.02813966861457\\
40	2.02242805200385\\
41	2.01672732086495\\
42	2.01104047168735\\
43	2.00536911184992\\
44	1.99971419848691\\
45	1.9940763658954\\
46	1.98845609169352\\
47	1.98285377267273\\
48	1.97726975827453\\
49	1.9717043644316\\
50	1.96615787974546\\
51	1.96063056959387\\
52	1.81096910142506\\
53	1.73579243390137\\
54	1.69461979591572\\
55	1.67026536490585\\
56	1.75137744398938\\
57	1.80022644855639\\
58	1.82831290791667\\
59	1.84316404278106\\
60	1.84963354714232\\
61	1.85084234846644\\
62	1.85631988151566\\
63	1.85929270842977\\
64	1.85998553259914\\
65	1.85875755555053\\
66	1.85607353730746\\
67	1.85234273112431\\
68	1.84790015847148\\
69	1.84299956696929\\
70	1.83782491141511\\
71	1.83250448448826\\
72	1.82712511422698\\
73	1.82174387568013\\
74	1.81639714046675\\
75	1.81110717576499\\
76	1.80588680576644\\
77	1.79196227834542\\
78	1.77785937177105\\
79	1.76709716030229\\
80	1.75856197254898\\
81	1.7515527783912\\
82	1.74552719640922\\
83	1.74009878328374\\
84	1.73503728600585\\
85	1.73021046316222\\
86	1.72554243740614\\
87	1.72098765788946\\
88	1.71651673605409\\
89	1.71210911614752\\
90	1.70774936647497\\
91	1.70342529481548\\
92	1.6991269501066\\
93	1.69484605094282\\
94	1.69106499461262\\
95	1.6875489513651\\
96	1.6841813441923\\
97	1.68088576528461\\
98	1.67762875024548\\
99	1.67439899178978\\
100	1.67119774968239\\
101	1.66803337315941\\
102	1.66492202093635\\
103	1.56302534163603\\
104	1.51575088460378\\
105	1.48936757156393\\
106	1.47583822851293\\
107	1.46800918359182\\
108	1.46309364399488\\
109	1.45976607070543\\
110	1.45737237190394\\
111	1.45558542534378\\
112	1.45423998738816\\
113	1.4532521810062\\
114	1.45946681281065\\
115	1.46196939401765\\
116	1.46313914689691\\
117	1.46359846220669\\
118	1.46362972539861\\
119	1.46341555418757\\
120	1.46149283553828\\
121	1.46024699828056\\
122	1.46228317976605\\
123	1.46243282283423\\
124	1.46352484186086\\
125	1.44221389731104\\
126	1.42871462363013\\
127	1.42348478079697\\
128	1.4216733184618\\
129	1.4213157615431\\
130	1.42158792953031\\
131	1.42213065890873\\
132	1.4227842274185\\
133	1.42347668458552\\
134	1.42405851853493\\
135	1.42447164332483\\
136	1.42061095008492\\
137	1.41982612113556\\
138	1.42008778424387\\
139	1.42064996166673\\
140	1.41324756081051\\
141	1.41203491285942\\
142	1.41186996109744\\
143	1.41189647609411\\
144	1.41182926083433\\
145	1.41156236342436\\
146	1.41105561373858\\
147	1.41029455714596\\
148	1.40927623721766\\
149	1.39998759498041\\
150	1.39549420418912\\
151	1.39240907869925\\
152	1.38983254226272\\
153	1.38737799641605\\
154	1.38449372045968\\
155	1.38144008461202\\
156	1.37830380358405\\
157	1.36836642608309\\
158	1.36174878752356\\
159	1.44231355849425\\
160	1.48236321924142\\
161	1.50131440616898\\
162	1.50939162011856\\
163	1.51190535002674\\
164	1.51155840319224\\
165	1.50973057390283\\
166	1.5071256871118\\
167	1.50410459530338\\
168	1.3589139275083\\
169	1.30594848680057\\
170	1.2829517544052\\
171	1.26775892918543\\
172	1.25741708744311\\
173	1.2491167808001\\
174	1.24184914887234\\
175	1.23480223821174\\
176	1.18344689039678\\
177	1.16320760123513\\
178	1.1528293869147\\
179	1.14564493330366\\
180	1.13952289783385\\
181	1.14438550560503\\
182	1.14248700405622\\
183	1.13843148847028\\
184	1.13359954987763\\
185	1.12772381192584\\
186	1.12237542469687\\
187	1.1062539225209\\
188	1.10016988886088\\
189	1.09505044278136\\
190	1.09022722893082\\
191	1.08555846536742\\
192	1.08101440576042\\
193	1.07655754487956\\
194	1.07216038599644\\
195	1.06780407432976\\
196	1.06347766969432\\
197	1.0591751229253\\
198	1.0548932849716\\
199	1.05063056264671\\
200	1.04638617568889\\
201	1.04215975320148\\
202	1.03795112778385\\
203	1.03376023231579\\
204	1.03112270119028\\
205	1.02749442628941\\
206	1.02360092201277\\
207	1.01919178061193\\
208	1.01492291572964\\
209	1.01070429215863\\
210	1.00663910188909\\
211	1.00272283424918\\
212	0.974124590579493\\
213	0.967634693789746\\
214	0.963234128440926\\
215	0.958877430062893\\
216	0.954437355380392\\
217	0.949989571164824\\
218	0.945568655135349\\
219	0.941182544793051\\
220	0.932722774858674\\
221	0.927142352380002\\
222	0.922249371897603\\
223	0.91762982464786\\
224	0.913158270995898\\
225	0.90876709046326\\
226	0.904425846764373\\
227	0.900125197011137\\
228	0.895763372659917\\
229	0.891359138633732\\
230	0.886955765589546\\
231	0.882601353379705\\
232	0.878344143217615\\
233	0.874230852197642\\
234	0.870305728769395\\
235	0.866609855240254\\
236	0.863180611073702\\
237	0.860051274376834\\
238	0.856937207382852\\
239	0.8538743204769\\
240	0.850867986857446\\
241	0.847918449693038\\
242	0.845025170100999\\
243	0.84218749069594\\
244	0.839404737318187\\
245	0.836676228419264\\
246	0.834001277309688\\
247	0.83137919279732\\
248	0.828809280604143\\
249	0.826290844800283\\
250	0.8238231893203\\
251	0.821405619428956\\
252	0.819037443131792\\
253	0.816717972504894\\
254	0.814569370766713\\
255	0.812347165928072\\
256	0.810173289276815\\
257	0.807410693506027\\
258	0.805108094130418\\
259	0.802982626948338\\
260	0.800951863504535\\
261	0.798981720402049\\
262	0.797061137209481\\
263	0.795185060879527\\
264	0.793141450890885\\
265	0.795259674851807\\
266	0.794579606337678\\
267	0.793010883805013\\
268	0.791282651903523\\
269	0.789561175357935\\
270	0.787877137160656\\
271	0.786233906538764\\
272	0.784655421592734\\
273	0.783125991128215\\
274	0.781633337377785\\
275	0.780176309274667\\
276	0.779345763962866\\
277	0.796606091446377\\
278	0.796568267979533\\
279	0.795233788694235\\
280	0.793720898298417\\
281	0.792211096824233\\
282	0.790734748033261\\
283	0.789297136358807\\
284	0.787899082029809\\
285	0.786540546797139\\
286	0.787543333482952\\
287	0.786843959776166\\
288	0.785662592270602\\
289	0.803747541764905\\
290	0.806594524553837\\
291	0.805832657532431\\
292	0.804676646032571\\
293	0.803374461271571\\
294	0.802183397770375\\
295	0.801026982887613\\
296	0.799880625192821\\
297	0.79875317333472\\
298	0.806542416536477\\
299	0.806238571644675\\
300	0.805403179077519\\
301	0.804552898327938\\
302	0.803760178920984\\
303	0.803036398361197\\
304	0.802383534267539\\
305	0.801801429718723\\
306	0.802304290337931\\
};
\addlegendentry{\lblMVAmeb{4}}


\addplot[area legend, draw=none, fill=mycolor4, fill opacity=0.1]
table[row sep=crcr] {%
x	y\\
1	500\\
2	448.981906337476\\
3	349.270535079624\\
4	78.3532792719168\\
5	61.887673457467\\
6	59.6202127413214\\
7	59.454781173502\\
8	53.2549091573309\\
9	51.2495889645071\\
10	46.5332398642737\\
11	43.8735580268363\\
12	41.7198120129723\\
13	37.4523396530481\\
14	34.527998782811\\
15	32.2089616096912\\
16	23.1794922911177\\
17	21.7510748926239\\
18	18.0101437887343\\
19	16.0043361221442\\
20	17.2051871907084\\
21	14.3396205185083\\
22	14.0419318738144\\
23	13.1436990982919\\
24	12.1051954138257\\
25	10.6833526720772\\
26	11.5315791211189\\
27	10.2321039536253\\
28	10.2612547192708\\
29	10.2568835207699\\
30	8.09920650379411\\
31	8.38325750271561\\
32	8.97937523832956\\
33	8.04910211029187\\
34	8.67521420792287\\
35	8.93767975284402\\
36	8.76361119248786\\
37	8.31858998243869\\
38	9.22493569483636\\
39	7.44866868031238\\
40	8.25513765576004\\
41	7.59057366984693\\
42	7.42244818585235\\
43	7.71237706738039\\
44	7.10635764817748\\
45	6.51989956891377\\
46	5.8915206039597\\
47	6.0989555012714\\
48	6.12009263912858\\
49	6.21565336448598\\
50	6.21534841993507\\
51	6.90797639939087\\
52	7.01079451617076\\
53	6.87773285850982\\
54	7.03716489584367\\
55	6.53204208516057\\
56	6.41544868868939\\
57	6.78390822150257\\
58	7.43786208142891\\
59	7.27676162070823\\
60	7.17193639256017\\
61	7.35625420063488\\
62	6.7190646112615\\
63	6.43106309851154\\
64	6.10789781361404\\
65	6.64816905769127\\
66	6.81274296298934\\
67	6.23648745435857\\
68	6.72459832074323\\
69	7.02804853137758\\
70	6.88874614185039\\
71	7.84734432354158\\
72	8.04004163500218\\
73	6.79241988498692\\
74	7.65724121335648\\
75	6.95856359196188\\
76	6.80275198520967\\
77	7.40235812297333\\
78	6.76596458808598\\
79	6.88789652910423\\
80	6.79571403081709\\
81	6.34131012449697\\
82	6.83283824026663\\
83	6.13933543132007\\
84	7.22847865657909\\
85	6.77798933598833\\
86	6.64298786470318\\
87	7.17067704529899\\
88	6.62114936004877\\
89	7.14609334863538\\
90	6.60722705663297\\
91	6.28661856700693\\
92	5.86764348910742\\
93	5.73983893361356\\
94	5.2803254428374\\
95	5.54022343403004\\
96	5.5102468136777\\
97	5.62888626327232\\
98	5.61245956259565\\
99	5.20825884951964\\
100	4.62054045556964\\
101	5.21952648104415\\
102	5.48797101386043\\
103	5.43981150926527\\
104	5.55232061148525\\
105	5.80580268872512\\
106	4.65565893726177\\
107	5.40449696182057\\
108	5.02896308732509\\
109	5.08303621435762\\
110	5.03613338935202\\
111	5.13346753799642\\
112	5.62442204201728\\
113	5.1259585860973\\
114	5.42201636627763\\
115	5.67321840256374\\
116	5.99368110405974\\
117	5.72500512917972\\
118	5.43872876698294\\
119	6.18751857545229\\
120	6.50080537241355\\
121	6.79616376193926\\
122	6.286768852316\\
123	6.62020576602504\\
124	7.06254757168009\\
125	7.34242073830676\\
126	7.24451685220409\\
127	7.36318801357246\\
128	6.99698785278115\\
129	6.72615667419783\\
130	6.64900963166463\\
131	6.49875720152879\\
132	6.12612172303184\\
133	6.25461871104977\\
134	5.43168285435406\\
135	5.923526736682\\
136	6.42810955827313\\
137	5.69474361465018\\
138	5.77449503002342\\
139	6.63231489383171\\
140	7.11390863943423\\
141	6.65365399601504\\
142	7.28652241424215\\
143	8.03524140070267\\
144	7.30042056279357\\
145	7.64248918596849\\
146	7.70220630870639\\
147	7.47273476131417\\
148	7.33350591435248\\
149	7.45238952698132\\
150	7.55825324159933\\
151	7.21044202941104\\
152	7.35854058475813\\
153	7.29187775815201\\
154	7.47548354909788\\
155	7.35820476738875\\
156	6.80234069010013\\
157	7.06432348745167\\
158	7.50019593780116\\
159	7.24283721346095\\
160	7.59605663212382\\
161	7.30511856422612\\
162	7.72471137464677\\
163	7.82236075594751\\
164	8.53948805242603\\
165	7.57901906741354\\
166	8.09640157501737\\
167	6.91941660721868\\
168	7.48035794580982\\
169	7.69892991060145\\
170	6.61232652818632\\
171	6.25372330972031\\
172	6.92907570996683\\
173	7.15881348280256\\
174	5.92346820531289\\
175	5.98716525944053\\
176	6.06838282658441\\
177	5.56760735907652\\
178	5.4019981940842\\
179	5.37205732771949\\
180	4.90634297360021\\
181	4.25015548131437\\
182	4.17836275293384\\
183	4.18983314410544\\
184	3.67171405687009\\
185	4.05560440772547\\
186	3.34925415447071\\
187	3.13477134397894\\
188	2.91431765280844\\
189	3.20808429875091\\
190	3.82771301348202\\
191	2.82491548045416\\
192	3.03592987830336\\
193	3.6770173837171\\
194	3.60612824544986\\
195	4.16431026805448\\
196	3.64990057744277\\
197	3.3449340249341\\
198	3.12177226555869\\
199	3.55963891521552\\
200	4.04579412760925\\
201	3.6869519717097\\
202	4.49853117858378\\
203	3.14932154769013\\
204	3.69383182843206\\
205	4.036007560763\\
206	4.50052125686367\\
207	4.07942514825173\\
208	3.7838595945695\\
209	3.5898131103808\\
210	3.44051885294779\\
211	3.52322790354421\\
212	3.26254390279489\\
213	3.68544741989134\\
214	3.38039087823383\\
215	3.18959735576049\\
216	2.51162489794551\\
217	2.58899733255808\\
218	2.82352106437355\\
219	2.9802496124006\\
220	3.19983194906028\\
221	2.90972362913012\\
222	3.1266214311124\\
223	2.75626737303882\\
224	2.6117805175218\\
225	2.90443380656913\\
226	2.70214752170829\\
227	2.79107817983494\\
228	2.66847321030679\\
229	2.72695829384473\\
230	2.8344641015376\\
231	3.04892653945021\\
232	2.39069742546998\\
233	2.62789782511373\\
234	2.79023176390253\\
235	2.60378551362242\\
236	2.52335865608391\\
237	2.64834167143408\\
238	2.4783609728661\\
239	2.28337961373664\\
240	2.09541765944465\\
241	2.64008668800129\\
242	2.36991819138907\\
243	2.93584571429655\\
244	2.71346715953275\\
245	2.75513042172514\\
246	2.81365906932751\\
247	2.85185510851945\\
248	2.65303379104665\\
249	2.74423438429734\\
250	3.00519382728668\\
251	2.84370305434084\\
252	2.79035133981022\\
253	3.04419115386128\\
254	2.5493312564355\\
255	2.91307002749111\\
256	2.7478217088448\\
257	2.73121186133769\\
258	2.80780915990826\\
259	3.28057920823974\\
260	2.5873756484813\\
261	2.6965452540275\\
262	2.97201560212265\\
263	2.81320687545107\\
264	2.90345020143973\\
265	3.23761951993641\\
266	3.01736066793555\\
267	3.30729246613439\\
268	3.42495296174112\\
269	3.71385972300944\\
270	4.07193889932651\\
271	3.53993343387034\\
272	3.08159609911269\\
273	3.17279904842641\\
274	3.27809813988191\\
275	3.58483742342761\\
276	3.57571102291115\\
277	3.91409789472926\\
278	3.58493402460765\\
279	3.0611839419536\\
280	3.19226195805386\\
281	3.11729566566567\\
282	3.07636624920845\\
283	3.17124123025782\\
284	3.08388542027352\\
285	3.44297465435767\\
286	3.14781934503876\\
287	2.86679083878452\\
288	2.58058048010722\\
289	2.27733268141166\\
290	2.27068040961598\\
291	1.79496037428038\\
292	2.05674221044612\\
293	2.10297998016953\\
294	1.82895575726901\\
295	2.29149294730899\\
296	1.7867432887266\\
297	1.92319353845401\\
298	2.12148515813316\\
299	1.90570185407136\\
300	2.0311591905981\\
301	1.80617335928047\\
302	1.96040060904888\\
303	1.76973039510425\\
304	1.81767784905841\\
305	1.81186360728135\\
306	1.91001736755278\\
306	0.349808881357062\\
305	0.397813682309296\\
304	0.462917652231631\\
303	0.445522070957907\\
302	0.286727096506257\\
301	0.420935408457624\\
300	0.283789082073885\\
299	0.384423170635581\\
298	0.547845178460975\\
297	0.408140617068889\\
296	0.385179435043314\\
295	0.36612560939931\\
294	0.349263814217911\\
293	0.337829456595541\\
292	0.425121626010038\\
291	0.453428122366761\\
290	0.507733422765821\\
289	0.384190717840334\\
288	0.322792355631466\\
287	0.519569890463669\\
286	0.64296172077709\\
285	0.469487781860115\\
284	0.4374829402624\\
283	0.586570686105888\\
282	0.704873257628175\\
281	0.599867916456279\\
280	0.51131980872418\\
279	0.465347732397015\\
278	0.565873484449141\\
277	0.504966804298962\\
276	0.690153828881483\\
275	0.760735253238245\\
274	0.466448183533962\\
273	0.580519943988942\\
272	0.701359097817879\\
271	0.632607802424605\\
270	0.68895184086183\\
269	0.690883128281046\\
268	0.489639112443047\\
267	0.656781958381402\\
266	0.49746592274754\\
265	0.629677357683783\\
264	0.357816411720524\\
263	0.618025822818716\\
262	0.522387067438392\\
261	0.477632657029248\\
260	0.462270031054339\\
259	0.691232355767652\\
258	0.599441202868728\\
257	0.522141761631751\\
256	0.353316812985131\\
255	0.457773069122385\\
254	0.439690580137899\\
253	0.404009867998101\\
252	0.433312872120773\\
251	0.543260121389896\\
250	0.528122153034155\\
249	0.660891992072182\\
248	0.487580071193011\\
247	0.540386467522281\\
246	0.551777024227163\\
245	0.385209863557843\\
244	0.44478566640604\\
243	0.342249548859402\\
242	0.586244174828881\\
241	0.428259008063102\\
240	0.645334894896294\\
239	0.388346078528089\\
238	0.456121797308192\\
237	0.45979750101678\\
236	0.569928369075384\\
235	0.453016154470959\\
234	0.450961745334062\\
233	0.48115805357031\\
232	0.506849363661314\\
231	0.410853566384692\\
230	0.459744479986873\\
229	0.460391334785376\\
228	0.563227359236237\\
227	0.390119310681083\\
226	0.46152697305913\\
225	0.407027460951295\\
224	0.470505348930746\\
223	0.580947271007577\\
222	0.589231154858417\\
221	0.371985816924136\\
220	0.415210641278189\\
219	0.386662154999305\\
218	0.481401742404696\\
217	0.409517737410365\\
216	0.442162438607409\\
215	0.362398229975955\\
214	0.485124048849934\\
213	0.522249360985057\\
212	0.701169341921795\\
211	0.617551031507221\\
210	0.475597301919383\\
209	0.666350638720139\\
208	0.398363351957874\\
207	0.762937892877592\\
206	0.667838537911632\\
205	0.577679165236177\\
204	0.470007446649428\\
203	0.401455509006276\\
202	0.703109602555317\\
201	0.71675848015345\\
200	0.687533811298438\\
199	0.667664154250317\\
198	0.627149096793778\\
197	0.517757726428295\\
196	0.623928958930141\\
195	0.63985941865927\\
194	0.644639519232867\\
193	0.548507428159517\\
192	0.52479429566651\\
191	0.365837598290465\\
190	0.715742844058687\\
189	0.473163999431169\\
188	0.536577208533833\\
187	0.500043793267856\\
186	0.485493091415684\\
185	0.591384858664549\\
184	0.575328824066029\\
183	0.46752001223039\\
182	0.555814299428464\\
181	0.699034398175932\\
180	0.633158459255753\\
179	0.552448845480259\\
178	0.617100709779652\\
177	0.867370058245659\\
176	0.509339674528219\\
175	0.544563896537363\\
174	0.644297056957933\\
173	0.517091273746685\\
172	0.693525222787448\\
171	0.670902995790263\\
170	0.751764205003849\\
169	0.685001157928177\\
168	0.626014210293732\\
167	0.52038628822426\\
166	0.511188028013898\\
165	0.916731067434791\\
164	0.946079409679674\\
163	0.727774396337027\\
162	1.09289442769122\\
161	0.523902533704673\\
160	0.764539640108818\\
159	0.894374656634816\\
158	0.848553691048461\\
157	1.10203424966503\\
156	1.02934240559888\\
155	0.844099012982036\\
154	0.964361813588334\\
153	0.8352074822409\\
152	0.855384052442055\\
151	0.726363834375507\\
150	1.04301486616316\\
149	0.735956061669632\\
148	0.925792209610203\\
147	0.872426324573293\\
146	0.795125484870332\\
145	0.649514282194602\\
144	0.693881279562011\\
143	0.883206422040336\\
142	0.732222301308548\\
141	0.843741991684329\\
140	0.86536401972181\\
139	0.499264160395621\\
138	0.540340372962718\\
137	0.645145061796583\\
136	0.49587305604448\\
135	0.878190599049835\\
134	0.428774487095223\\
133	0.356527048226858\\
132	0.591110888924775\\
131	0.661460231290968\\
130	0.745262102818424\\
129	0.766862815573019\\
128	0.558431853089066\\
127	0.716405301952995\\
126	0.882833150135167\\
125	0.688054795876514\\
124	0.769623020159238\\
123	0.828856951574669\\
122	0.746303507269593\\
121	0.680306789165508\\
120	0.774785376346585\\
119	0.563217606716284\\
118	0.820902127730202\\
117	0.716580203018285\\
116	0.751713527558102\\
115	0.65472371121716\\
114	0.62120738967918\\
113	0.621358855950953\\
112	0.838723996410449\\
111	0.72895561883503\\
110	0.712079274590619\\
109	0.654688577439802\\
108	0.666371199065833\\
107	0.730746968110791\\
106	0.635121822448633\\
105	0.855457350770429\\
104	0.649004738901192\\
103	0.485882224865453\\
102	0.64494097577559\\
101	0.486724007936647\\
100	0.633455714608757\\
99	0.806011539339647\\
98	0.656524789343\\
97	0.777863639294216\\
96	0.627635078014086\\
95	0.719344467877647\\
94	0.665024617686201\\
93	0.76578120667295\\
92	0.860296558004049\\
91	0.653863948209535\\
90	0.644218200593417\\
89	0.834892967317743\\
88	0.640973606822157\\
87	0.739897851632222\\
86	0.938375840717595\\
85	0.819105659073992\\
84	0.673500601230991\\
83	1.03742239782708\\
82	0.728335806005288\\
81	0.810087390097712\\
80	0.867627109958075\\
79	0.964027329694762\\
78	1.02137993659527\\
77	0.677468818602609\\
76	0.752052414162837\\
75	0.702976614276561\\
74	0.646973110026791\\
73	0.611782218653082\\
72	0.807073200895766\\
71	0.553784942475039\\
70	0.918473929642695\\
69	0.917531000995552\\
68	0.627155600293908\\
67	0.733776700332959\\
66	0.659461045797541\\
65	0.777061644350059\\
64	0.651759555262315\\
63	0.806917591419951\\
62	0.604690946263572\\
61	0.665970209664082\\
60	1.00884523205909\\
59	0.562836675413533\\
58	0.851699205309324\\
57	0.48901758642933\\
56	0.594582376859964\\
55	0.670159085677585\\
54	0.695097344158746\\
53	0.618535527320136\\
52	0.811838260856723\\
51	0.624299051974209\\
50	0.496257849871754\\
49	0.625937978756493\\
48	0.41931104688163\\
47	0.511027818087889\\
46	0.965860390997935\\
45	0.656835933995588\\
44	0.515824880412063\\
43	0.806421637574713\\
42	0.588929819139667\\
41	0.995135284577265\\
40	0.675299047291813\\
39	0.716296609682014\\
38	0.689824192493016\\
37	1.20753960920619\\
36	1.06153879594595\\
35	1.04212339761671\\
34	1.00457273157484\\
33	0.973766776097912\\
32	0.685978033448791\\
31	0.7460844617882\\
30	0.671110681075517\\
29	1.12774903348612\\
28	1.14807502197289\\
27	0.893438212698202\\
26	0.838675742071086\\
25	1.09194114467689\\
24	1.52368105511013\\
23	1.02948939956193\\
22	0.969221440006744\\
21	0.730251900979203\\
20	0.826927055019283\\
19	1.30495397518143\\
18	1.37093742073922\\
17	1.40320673224683\\
16	1.66009550448616\\
15	1.70202348689401\\
14	1.78843727229254\\
13	1.84318228883417\\
12	2.41295946199178\\
11	1.84558416034111\\
10	2.19286475087309\\
9	2.51041921451201\\
8	2.57387484960019\\
7	2.52951768859112\\
6	3.07161610370284\\
5	3.37870796813076\\
4	2.43278985591592\\
3	3.45647538440758\\
2	0\\
1	39.178716084934\\
}--cycle;
\addlegendentry{\lblMVAuncertainty{4}}

==> figures/MVA-5-subplots/MVA-5plot-s5.tex <==
\addplot [color=mycolor5, dashed, line width=\LWestimates]
  table[row sep=crcr]{%
1	500\\
2	3.84289907442711\\
3	30.8088347702469\\
4	28.7262446080342\\
5	27.8842355241369\\
6	24.7667166259469\\
7	22.8779250020741\\
8	21.7513839911776\\
9	18.6129277018045\\
10	18.1243204452404\\
11	17.018980393202\\
12	16.1652781478886\\
13	15.30481963487\\
14	15.3252165472254\\
15	15.4603743855403\\
16	15.5849497692757\\
17	15.5082856608076\\
18	15.2381044470238\\
19	15.3070287820825\\
20	15.7833952155978\\
21	15.709237187235\\
22	15.5593923113724\\
23	15.2427471910189\\
24	15.4735497824965\\
25	15.5955190388704\\
26	15.2986607032771\\
27	15.3649872408634\\
28	15.6110378231325\\
29	16.0172628819609\\
30	16.6634005041636\\
31	17.2478016399358\\
32	17.7990851437142\\
33	18.3057071753068\\
34	18.8842035725156\\
35	19.4085011622424\\
36	20.6584069864603\\
37	21.0093640497855\\
38	20.5831234359291\\
39	20.7344496907867\\
40	21.5561726207102\\
41	22.1999008491404\\
42	21.6553753606304\\
43	21.8887830838923\\
44	21.9754865732542\\
45	21.9247842415727\\
46	21.8785575358747\\
47	21.6980396632261\\
48	21.7777287436283\\
49	21.925277498189\\
50	21.8997529646775\\
51	22.5108614999063\\
52	22.7147345664381\\
53	23.0342428496905\\
54	23.1569384222217\\
55	23.4096760256213\\
56	23.6386960483572\\
57	23.9721795117466\\
58	23.9169304814454\\
59	23.9124929201589\\
60	24.240354071506\\
61	24.250670308506\\
62	24.4657678357876\\
63	24.3854388434144\\
64	24.4094484681561\\
65	23.8508994583811\\
66	24.2775259833324\\
67	24.0177614348148\\
68	24.109231359832\\
69	24.3103750843298\\
70	24.5992842052218\\
71	24.4544062522517\\
72	24.3774539649962\\
73	24.7247142080269\\
74	25.0022692757713\\
75	25.2410717531666\\
76	24.4928120594646\\
77	24.0536809296198\\
78	19.4990746434444\\
79	17.2909794961746\\
80	15.6464774420355\\
81	14.0015775206971\\
82	12.9871195817177\\
83	11.6866367444207\\
84	11.305442680542\\
85	10.1462557082687\\
86	9.63551877149903\\
87	8.30455956973969\\
88	9.31286912170659\\
89	8.53244227221993\\
90	7.74377014719309\\
91	7.74372254053386\\
92	7.76678300014991\\
93	7.00268870769413\\
94	6.85254018710803\\
95	6.56511132059091\\
96	6.36540413941438\\
97	6.09920715420373\\
98	6.29275636415562\\
99	6.12172588203932\\
100	5.64330359110008\\
101	5.85345187826145\\
102	5.95716220431964\\
103	6.0748815986202\\
104	6.06193396267624\\
105	5.86792482582214\\
106	5.32735224410485\\
107	5.28591339826457\\
108	5.64501323556156\\
109	5.50257919183361\\
110	5.47320169825907\\
111	5.32619850346906\\
112	5.39846605829076\\
113	5.6829649706526\\
114	6.40697418445715\\
115	7.16850627957112\\
116	8.23406543876954\\
117	8.97017437975594\\
118	9.97141691896229\\
119	10.711445338139\\
120	11.4680345160837\\
121	12.3235814124488\\
122	11.7719357498185\\
123	11.0604448301414\\
124	10.4424914231461\\
125	9.72337362712783\\
126	9.55116756221615\\
127	9.36201345079802\\
128	9.1945638261336\\
129	8.93864045330074\\
130	8.65943981572723\\
131	8.43816945370317\\
132	8.22958741072856\\
133	7.85742681106753\\
134	7.95308470096726\\
135	7.97124407013755\\
136	7.69887752784836\\
137	7.53226956115743\\
138	7.50973502617576\\
139	7.51096745323887\\
140	13.9963527850343\\
141	12.9043777544443\\
142	12.1584035770273\\
143	11.5673961796024\\
144	10.6230082112461\\
145	10.0463618696837\\
146	9.98028412720944\\
147	9.73415225896451\\
148	8.99633790127589\\
149	8.43198160173857\\
150	8.28252385535053\\
151	8.15083074532316\\
152	7.65626378607276\\
153	7.54073555073903\\
154	7.4186256216933\\
155	7.46959996953381\\
156	7.07581727674215\\
157	7.0362061771633\\
158	7.23349710233972\\
159	7.12320320989603\\
160	7.63823916951713\\
161	7.29514381089048\\
162	7.25959748370429\\
163	6.94027493367049\\
164	6.48141468012838\\
165	6.78784585120924\\
166	6.43404120808929\\
167	5.50895469879537\\
168	5.1207337417761\\
169	5.69784534591889\\
170	5.41008159944703\\
171	4.88044900776436\\
172	5.27385177391725\\
173	4.77584987309101\\
174	5.11394842292721\\
175	4.74708045599203\\
176	4.8504929097622\\
177	4.78583928506634\\
178	4.98983257044343\\
179	4.78758236700059\\
180	4.33230461469884\\
181	4.628728548086\\
182	4.95358019853626\\
183	5.07331983175102\\
184	5.1297454082588\\
185	4.76502851540159\\
186	4.39726706049555\\
187	3.31862132329666\\
188	3.1057350839561\\
189	2.4140091558169\\
190	2.29234137540918\\
191	2.51354271283916\\
192	2.51956594568505\\
193	2.54723083543366\\
194	2.52756252717417\\
195	2.59569634725109\\
196	2.66513910784608\\
197	2.72355968754743\\
198	2.66368483961032\\
199	2.60961453577935\\
200	2.55528508675722\\
201	2.6663907518933\\
202	2.72095446891926\\
203	2.7222276181259\\
204	2.53367845488467\\
205	2.63431126568041\\
206	2.89080293514881\\
207	2.14912707502332\\
208	2.59104181078563\\
209	2.62508284271861\\
210	2.65019182279493\\
211	2.60540543334781\\
212	2.30381926581596\\
213	2.61999088845026\\
214	2.33356726260628\\
215	2.32254594505593\\
216	2.49928038701246\\
217	2.53065218967339\\
218	2.70335305469865\\
219	2.80798676570125\\
220	2.58954771615158\\
221	2.79407469542808\\
222	2.67277016137722\\
223	2.55169593082422\\
224	2.64875075568072\\
225	2.44012961134829\\
226	2.62941211494088\\
227	2.84241951718241\\
228	2.66846431962436\\
229	2.32863081754276\\
230	2.92302734185191\\
231	2.51063110470004\\
232	2.59295521179409\\
233	2.47076334387218\\
234	2.73333604237658\\
235	2.52147051065844\\
236	2.60342748498781\\
237	2.48087194033118\\
238	2.44980559947781\\
239	2.6954315735871\\
240	2.59601146128853\\
241	2.39805279479134\\
242	2.76545172905027\\
243	2.59811051398208\\
244	2.6200164360767\\
245	2.4466359429104\\
246	2.58727745358187\\
247	2.85142193748459\\
248	2.75370633663136\\
249	3.23215079123124\\
250	3.18916902372511\\
251	3.1711787942815\\
252	2.85830618524981\\
253	2.92168381469501\\
254	2.94531392940391\\
255	3.10063929092728\\
256	2.96245327146947\\
257	2.74341515114986\\
258	2.40781084326664\\
259	2.62485062726011\\
260	2.6038943129413\\
261	2.87363470678906\\
262	2.79542136236011\\
263	2.48620774367218\\
264	3.31245597257594\\
265	2.86477782907009\\
266	2.85940064286255\\
267	3.13407098946013\\
268	3.17323940421925\\
269	3.2766544441499\\
270	3.24942880341599\\
271	3.17873960575834\\
272	3.4137830707097\\
273	3.07329383076814\\
274	2.96026188198065\\
275	2.9701064794165\\
276	3.16001697978194\\
277	2.82689463437293\\
278	2.88789635171441\\
279	2.9015097781346\\
280	2.7466456842133\\
281	2.68773703302656\\
282	2.91527784800162\\
283	3.10711111789075\\
284	3.26998673356001\\
285	3.05917610772695\\
286	3.12751285755567\\
287	3.05482356872487\\
288	2.67587730320174\\
289	2.67738481146217\\
290	2.92057137265819\\
291	3.38448767492925\\
292	3.06519949607306\\
293	3.46542439202048\\
294	3.23127504894143\\
295	3.0360267825145\\
296	3.11548667064905\\
297	3.23217180537071\\
298	3.15184412255413\\
299	3.22904746761295\\
300	3.46367776840927\\
301	3.84660816743874\\
302	3.29048807608033\\
303	3.4486291198965\\
304	3.19608490479185\\
305	3.44502681920149\\
306	3.95792968689696\\
};
\addlegendentry{\lblMVAest{5}}

\addplot [color=mycolor5, line width=\LWbound]
  table[row sep=crcr]{%
1	2.25453003092278\\
2	1.98017567136455\\
3	1.8589987171145\\
4	1.79975777939349\\
5	1.76903006204124\\
6	1.7522463672537\\
7	1.96164361433947\\
8	2.10392152798275\\
9	2.20533494458266\\
10	2.27737425696422\\
11	2.32759815561211\\
12	2.36151966454723\\
13	2.38330005136396\\
14	2.39609956687545\\
15	2.40230700080375\\
16	2.40370990306174\\
17	2.40163325285329\\
18	2.39705050661993\\
19	2.39067160190374\\
20	2.38377509229785\\
21	2.37652612547241\\
22	2.36904357015983\\
23	2.36143274366859\\
24	2.35378323868037\\
25	2.34623924317941\\
26	2.33885833863091\\
27	2.33167855934956\\
28	2.32473966693411\\
29	2.44535002032853\\
30	2.5381912937106\\
31	2.61070252309965\\
32	2.66748419717922\\
33	2.71186047860528\\
34	2.74643380975401\\
35	2.77341230105324\\
36	2.79427058157641\\
37	2.81023405881522\\
38	2.82286579990931\\
39	2.83278044379482\\
40	2.84055539551884\\
41	2.8466413710994\\
42	2.85139228980809\\
43	2.85508677046717\\
44	2.85794471960199\\
45	2.86013966276701\\
46	2.86180824758518\\
47	2.86305777103237\\
48	2.86397221493636\\
49	2.86461709564961\\
50	2.8650433506258\\
51	2.86529043983159\\
52	2.85108359463952\\
53	2.84506838639522\\
54	2.84221774384799\\
55	2.84060683163214\\
56	2.84103813572083\\
57	2.84175722225668\\
58	2.84245369708142\\
59	2.8429953426346\\
60	2.84333310766603\\
61	2.84346209137448\\
62	2.86159885156556\\
63	2.87299046937001\\
64	2.87911090766261\\
65	2.88222482831062\\
66	2.88368683079334\\
67	2.88418876050418\\
68	2.88408579709575\\
69	2.88356318860908\\
70	2.88272317743626\\
71	2.88162673494837\\
72	2.88031373916234\\
73	2.8788126094612\\
74	2.87714497563257\\
75	2.8753279965559\\
76	2.87337557666573\\
77	2.86302547919135\\
78	2.44982729915948\\
79	2.31464962275328\\
80	2.24135938646097\\
81	2.19668692119412\\
82	2.16740390547598\\
83	2.14713342819556\\
84	2.13229706372681\\
85	2.12078492614904\\
86	2.11131471551437\\
87	2.10309371926924\\
88	2.09562611256676\\
89	2.08859910463267\\
90	2.08181406210001\\
91	2.07514419336915\\
92	2.06850825218758\\
93	2.06185404911029\\
94	2.05576071109047\\
95	2.04982802412032\\
96	2.04388909694253\\
97	2.0378490364891\\
98	2.03166626297843\\
99	2.02532991591578\\
100	2.01884861957583\\
101	2.01224449053668\\
102	2.00555139609341\\
103	1.98748581028224\\
104	1.97393606250512\\
105	1.96266115578189\\
106	1.95308174379987\\
107	1.94463122760277\\
108	1.93707085104266\\
109	1.9302430678712\\
110	1.92406218326452\\
111	1.91848257031198\\
112	1.91348734582086\\
113	1.90907743351733\\
114	2.15475102794434\\
115	2.29998011999902\\
116	2.39889205731739\\
117	2.46984408525261\\
118	2.52161525373786\\
119	2.55940110546175\\
120	2.58461302517026\\
121	2.60411773136028\\
122	2.58318474233824\\
123	2.59982597882373\\
124	2.78242346253993\\
125	2.95298602612859\\
126	3.10994873459529\\
127	3.25419267408825\\
128	3.38707094719548\\
129	3.50976899080654\\
130	3.62326869973643\\
131	3.72837954526427\\
132	3.82578237194644\\
133	3.91606378807324\\
134	3.99943376976803\\
135	4.0765632679803\\
136	4.14791381133799\\
137	4.21382001037434\\
138	4.27454235158194\\
139	4.33029259661994\\
140	4.17856376377366\\
141	4.18998708301033\\
142	4.2184042062949\\
143	4.24772116140291\\
144	4.27404069396604\\
145	4.29625244587454\\
146	4.31404609404485\\
147	4.32737045361847\\
148	4.33627113052933\\
149	4.31533574525819\\
150	4.3097003969495\\
151	4.30379613314174\\
152	4.29493103296545\\
153	4.28263837916977\\
154	4.26569099807474\\
155	4.24439843772294\\
156	4.21911161880495\\
157	4.18873333016974\\
158	4.15600302979604\\
159	4.12127835661122\\
160	4.08415881503927\\
161	4.04496573119806\\
162	4.0040466509455\\
163	3.96174114119656\\
164	3.91837257025301\\
165	3.87424337865979\\
166	3.82963224867991\\
167	3.78479251754168\\
168	3.7393633215794\\
169	3.69441315631687\\
170	3.64995288498092\\
171	3.60368855145038\\
172	3.55953319242192\\
173	3.51664491959607\\
174	3.64944812748776\\
175	3.77937595660425\\
176	3.90498608506262\\
177	4.02638059924642\\
178	4.14377927117351\\
179	4.25742365485472\\
180	4.36754249710484\\
181	4.47434917416251\\
182	4.57802610215541\\
183	4.67873540340833\\
184	4.77662318502806\\
185	3.44903723293224\\
186	2.97311467091694\\
187	2.04401580418467\\
188	1.81638701546189\\
189	1.73060504012945\\
190	1.6970189285426\\
191	1.68592198617927\\
192	1.68525259189951\\
193	1.68958553250701\\
194	1.69639721723288\\
195	1.70448231215601\\
196	1.71325605411259\\
197	1.72243017344621\\
198	1.73186030865523\\
199	1.74147269454912\\
200	1.7512285800303\\
201	1.76110674754447\\
202	1.77109484639548\\
203	1.7811850546146\\
204	1.79191460206248\\
205	1.80271960656061\\
206	1.81359202799633\\
207	1.71907085473611\\
208	1.68279477879695\\
209	1.66922255780854\\
210	1.66593962103148\\
211	1.66765546644304\\
212	1.67122179120032\\
213	1.6765286213261\\
214	1.68248837703695\\
215	1.68877056900157\\
216	1.69522224517157\\
217	1.7017648636567\\
218	1.7083592403664\\
219	1.71498482984428\\
220	1.72026801511506\\
221	1.72681468295898\\
222	1.73345858773989\\
223	1.74012728563091\\
224	1.74681168888205\\
225	1.75350781640001\\
226	1.76021342476321\\
227	1.76690165681765\\
228	1.77365207191461\\
229	1.78050061274317\\
230	1.78743878068415\\
231	1.79443287600661\\
232	1.80143578629186\\
233	1.8083936363179\\
234	1.81524961099292\\
235	1.82194625265735\\
236	1.82842692721056\\
237	1.83463682269233\\
238	1.84077288472271\\
239	1.84688541036243\\
240	1.85298901797442\\
241	1.85909035831517\\
242	1.86519237618262\\
243	1.87129599616251\\
244	1.87740100930275\\
245	1.88350656546507\\
246	1.88961145076597\\
247	1.8957142454708\\
248	1.90181341465215\\
249	1.90790736083566\\
250	1.91399445505839\\
251	1.92007305563687\\
252	1.92614151992658\\
253	1.93219821208551\\
254	1.93851240859065\\
255	1.9445849399412\\
256	1.95060425782328\\
257	1.815296826409\\
258	1.75661064445361\\
259	1.72954064586906\\
260	1.71780684936996\\
261	1.71386404585025\\
262	1.71396639899303\\
263	1.71619601536496\\
264	1.71905475503938\\
265	1.72373066667536\\
266	1.72819926337464\\
267	1.73273201914295\\
268	1.7373099257784\\
269	1.74191766210231\\
270	1.74654249567286\\
271	1.75117683898542\\
272	1.75598488712035\\
273	1.7609408385114\\
274	1.76597097945222\\
275	1.77104157931105\\
276	1.82456519648016\\
277	1.85637075874691\\
278	1.87827665454804\\
279	1.89448609553898\\
280	1.90733858642372\\
281	1.91820224405314\\
282	1.92788965606853\\
283	1.93688548972409\\
284	1.94548010980678\\
285	1.95384805718286\\
286	2.00924440101637\\
287	2.04076191785964\\
288	2.06312969523944\\
289	2.15003454384555\\
290	2.21326194854965\\
291	2.26261304266753\\
292	2.30117052571943\\
293	2.33125804324727\\
294	2.35552649204469\\
295	2.37431810333672\\
296	2.38933840161428\\
297	2.40160649407508\\
298	2.41353103444165\\
299	2.42341493267226\\
300	2.4318639173171\\
301	2.4392425426924\\
302	2.44582690108312\\
303	2.45181888360231\\
304	2.45736785349345\\
305	2.46258432481657\\
306	2.47114792671587\\
};
\addlegendentry{\lblMVAmeb{5}}


\addplot[area legend, draw=none, fill=mycolor5, fill opacity=0.1]
table[row sep=crcr] {%
x	y\\
1	500\\
2	461.194435097404\\
3	57.1620636247818\\
4	55.7449316974464\\
5	53.2139673450305\\
6	48.8336571194233\\
7	47.2650881125475\\
8	44.5367179877561\\
9	41.8479702225767\\
10	39.3439994217165\\
11	38.3570930594524\\
12	32.8182856266982\\
13	30.9335231813157\\
14	28.2389477707164\\
15	27.9565124319406\\
16	26.9806987680053\\
17	26.2800500978072\\
18	26.7617437095971\\
19	25.5380031620823\\
20	25.7453480737126\\
21	25.9496351587446\\
22	26.8546537443675\\
23	25.2667539278005\\
24	26.3582714378819\\
25	25.927652972268\\
26	26.0559852229477\\
27	26.2697879371714\\
28	25.549063633202\\
29	25.911884791834\\
30	27.4845580748665\\
31	28.2267189410735\\
32	28.2538566507373\\
33	29.1639951699356\\
34	31.2018012161177\\
35	31.6630274036579\\
36	33.2954103540869\\
37	33.6771035138455\\
38	33.3105737932847\\
39	34.453669849613\\
40	35.2550890789042\\
41	36.6400294659261\\
42	35.6937717427519\\
43	35.1705901903377\\
44	35.5954472132563\\
45	37.6014499230295\\
46	35.201613429318\\
47	35.6563450396803\\
48	35.7668094941965\\
49	35.0481852061286\\
50	35.949246352391\\
51	36.1646475336071\\
52	36.5149767007927\\
53	36.3616552329241\\
54	36.3873269063457\\
55	36.7793768521413\\
56	37.6111928116548\\
57	39.7496099122992\\
58	37.0669280848067\\
59	38.4622394213941\\
60	38.0107864090638\\
61	38.7066571807512\\
62	38.8573888272696\\
63	41.1170210725803\\
64	40.1220303311114\\
65	40.9311104644858\\
66	38.0855340812818\\
67	38.4370939711608\\
68	38.6960849861614\\
69	39.5274776989804\\
70	39.6180733298991\\
71	39.0566992375113\\
72	39.1731668444587\\
73	38.3240918164899\\
74	40.223640804362\\
75	42.7982575122623\\
76	41.2597827046842\\
77	40.7010562371773\\
78	32.4043358427834\\
79	32.2063418256756\\
80	27.736833730433\\
81	26.5930020610716\\
82	26.5152225475316\\
83	25.068390236417\\
84	23.8407831313561\\
85	19.6935130853529\\
86	20.1427054852873\\
87	18.3508506344242\\
88	18.8162482942643\\
89	16.7688522121077\\
90	14.7414144040154\\
91	14.0080687583485\\
92	13.3553999798066\\
93	12.6727777934969\\
94	12.6212037060063\\
95	12.0889233645129\\
96	10.6089811073543\\
97	10.4078587744757\\
98	10.4762368019346\\
99	10.2592567541786\\
100	10.7032715918269\\
101	11.4058793085538\\
102	10.3962527806916\\
103	9.73911987271727\\
104	9.77108571634283\\
105	9.45979095890475\\
106	9.80866295745634\\
107	9.2590763952974\\
108	9.27388725428733\\
109	9.05648019914327\\
110	9.50286886846614\\
111	8.85075424293314\\
112	9.11051282546087\\
113	9.52763871834551\\
114	10.4366162799966\\
115	11.7683238549497\\
116	13.0897858501509\\
117	13.806320863301\\
118	15.2801989680367\\
119	16.0272562318666\\
120	17.1956504037766\\
121	19.217986502174\\
122	18.1407178867066\\
123	16.9857195408562\\
124	17.9633120999856\\
125	17.9659488180784\\
126	16.8538686407419\\
127	16.7164495145233\\
128	17.9239780687335\\
129	17.1641213672537\\
130	16.678474457143\\
131	17.0430243418095\\
132	17.1635957818856\\
133	16.2685596746368\\
134	18.17526204966\\
135	19.7429289283815\\
136	16.2348855267297\\
137	15.3101343155099\\
138	16.0516521762266\\
139	15.9901936536593\\
140	24.3315465648402\\
141	37.5171979847826\\
142	38.7171965206378\\
143	30.1920885990359\\
144	30.7460602624792\\
145	29.9841643615728\\
146	28.2839407973283\\
147	27.9687035234911\\
148	35.1188046910555\\
149	27.4328384847417\\
150	26.2591066117348\\
151	21.6077378741008\\
152	18.4505967484781\\
153	18.310119493341\\
154	19.1038605838089\\
155	17.1016057951169\\
156	16.2997241589023\\
157	16.1345799797116\\
158	15.6987493817034\\
159	15.9409157454465\\
160	15.6054865109513\\
161	15.4859833093812\\
162	14.7622308492922\\
163	13.9958025812711\\
164	12.3961702004982\\
165	12.0505189025821\\
166	11.3529560416468\\
167	9.94528670129836\\
168	9.00241131773425\\
169	10.4381074318867\\
170	10.1192318904287\\
171	10.329601443608\\
172	10.1309511138263\\
173	8.74449056353885\\
174	10.3219071757855\\
175	8.28648487812194\\
176	10.1310255820584\\
177	9.53512095124246\\
178	8.64873662137074\\
179	10.4889991208048\\
180	8.7993792701188\\
181	9.08294843835038\\
182	8.68942416108796\\
183	8.64356990304191\\
184	10.4279485850889\\
185	8.978638955843\\
186	8.08150494481685\\
187	5.52130004429966\\
188	5.32782810512942\\
189	4.07756483565192\\
190	4.32976865802565\\
191	4.00038883061539\\
192	4.31551840650191\\
193	4.74835980717259\\
194	4.82086759818967\\
195	4.72733838772398\\
196	5.31204189798437\\
197	4.7643791612184\\
198	4.08918289441018\\
199	4.55604479979948\\
200	3.96863418598176\\
201	4.84165032613567\\
202	4.26860783103345\\
203	4.45810720761865\\
204	4.23493760822003\\
205	4.78895141391093\\
206	4.82637812477633\\
207	4.43676871466333\\
208	4.99320828487588\\
209	4.4192791412989\\
210	4.53682362201082\\
211	4.39385768032488\\
212	3.72251965450789\\
213	4.03604675175413\\
214	3.85992274319617\\
215	4.22062890061302\\
216	3.91170699794529\\
217	4.34093992136486\\
218	4.60378487312525\\
219	4.49420500661662\\
220	3.90578346737092\\
221	4.67739808638654\\
222	4.05987430602646\\
223	4.17011656417815\\
224	4.62841032663297\\
225	3.86082623891607\\
226	4.40374463810874\\
227	4.34289162286513\\
228	4.01182194552536\\
229	4.3166057972643\\
230	5.10418942959984\\
231	4.59368342421206\\
232	4.83378680607509\\
233	4.49213937229048\\
234	4.40594471550322\\
235	4.43160652254709\\
236	4.26283555547363\\
237	3.75844473427344\\
238	4.1464007073548\\
239	4.82366492521956\\
240	4.42422936091198\\
241	3.81849310653908\\
242	4.4601495037263\\
243	4.4369420595688\\
244	4.80174759931611\\
245	4.29811609951603\\
246	4.62223601472093\\
247	4.60836291134884\\
248	4.54592180580149\\
249	5.26411419475732\\
250	5.76531612268423\\
251	5.55582480687483\\
252	5.04157302850327\\
253	5.66045317439591\\
254	5.74874030302318\\
255	4.9653683187485\\
256	4.72458750440582\\
257	4.22647105409832\\
258	4.00858910469778\\
259	4.29992501824768\\
260	4.3703606383867\\
261	4.71634348281018\\
262	4.61550516834734\\
263	4.79542707020415\\
264	5.5429685601437\\
265	5.04847169119332\\
266	5.61885512567536\\
267	6.20076331970988\\
268	5.55259497095438\\
269	5.73365252733888\\
270	5.667299882094\\
271	5.12579787853661\\
272	5.27787242346726\\
273	4.89648763166236\\
274	5.36265706622288\\
275	4.82511883328043\\
276	5.19935967813027\\
277	4.64198883754996\\
278	4.88783042089297\\
279	5.34497592155213\\
280	4.29285565690465\\
281	4.1572579345017\\
282	4.47451885788903\\
283	4.90621488484699\\
284	5.66929053182551\\
285	5.30277298028864\\
286	5.64747632773955\\
287	5.35949352338031\\
288	5.00337542860036\\
289	5.1896097882067\\
290	6.20377549521924\\
291	5.72024836362656\\
292	6.14700875654849\\
293	5.69045634390483\\
294	6.23585710245907\\
295	5.83243318022365\\
296	5.08568439194579\\
297	5.53357766046055\\
298	5.24896662966743\\
299	5.18643679381378\\
300	5.92490833051271\\
301	6.99884788059982\\
302	5.98389426602151\\
303	6.05233048588247\\
304	6.40521704844069\\
305	6.84223031474508\\
306	6.40796415170547\\
306	0.899074489471856\\
305	0.970868198424225\\
304	0.848446574188669\\
303	0.634937524941591\\
302	0.672855546309278\\
301	0.902356536392372\\
300	0.699752150837246\\
299	0.682240231734835\\
298	0.764366740093844\\
297	1.01068203197759\\
296	0.809862156382142\\
295	1.11752026951013\\
294	0.6806525607783\\
293	1.02811047945151\\
292	0.845427168718653\\
291	0.644437508781744\\
290	0.868611004355159\\
289	0.537408774960923\\
288	0.629157674473201\\
287	0.858444419891827\\
286	0.895305713809787\\
285	1.01175701128686\\
284	0.811528453539665\\
283	0.657484063174361\\
282	0.91458188742985\\
281	0.766184314857902\\
280	0.839203886891864\\
279	0.764961036662925\\
278	0.998462471742007\\
277	0.907291825330858\\
276	0.807201270620335\\
275	1.12953811724241\\
274	1.0477571995597\\
273	1.12754116565808\\
272	0.724825643327256\\
271	0.827721169157609\\
270	0.869072624950408\\
269	0.867854871205148\\
268	0.967817840687805\\
267	0.628348722793242\\
266	0.734897712983947\\
265	0.754295827847032\\
264	0.957536047732015\\
263	0.783342444219821\\
262	0.840266168777349\\
261	0.90106074752992\\
260	0.804906406180833\\
259	0.627520205617395\\
258	0.979341040265247\\
257	0.732882098218779\\
256	0.792044633274902\\
255	0.988135900729493\\
254	0.817260020046857\\
253	0.759344026084062\\
252	0.73202813812683\\
251	0.923757331933189\\
250	0.974691732431162\\
249	0.971198281808759\\
248	0.916425522348576\\
247	0.753230022747337\\
246	0.760461395995895\\
245	0.688625595222654\\
244	0.638817238817908\\
243	0.740673159717487\\
242	0.772021510612163\\
241	0.770522308167763\\
240	0.739725871586665\\
239	0.860532269748671\\
238	0.870562765813892\\
237	0.737280777304161\\
236	0.701089869851702\\
235	0.709029323371056\\
234	0.949041755697082\\
233	0.681550588071806\\
232	1.0314669981397\\
231	0.601638481637857\\
230	0.782146320921031\\
229	0.706395254057377\\
228	0.880363300161232\\
227	0.823476497478978\\
226	0.64011055879168\\
225	0.824732574331753\\
224	0.7163616625589\\
223	0.740143505535706\\
222	0.96592823983064\\
221	1.13460361775493\\
220	0.745252118846746\\
219	0.856426534412398\\
218	0.683109864677576\\
217	0.765839236361454\\
216	0.860236007853381\\
215	0.761785622124202\\
214	0.843677602798551\\
213	1.01017916788712\\
212	0.553220580340661\\
211	0.648802810263454\\
210	0.673332887124572\\
209	0.758758018163244\\
208	0.8574215030768\\
207	0.832503030107045\\
206	0.864991293454523\\
205	0.94700357241218\\
204	0.763028077316111\\
203	0.923543397684395\\
202	0.836710751752056\\
201	0.884236651630955\\
200	0.875898794196271\\
199	0.963083667262005\\
198	0.692635983062819\\
197	0.710294288370097\\
196	0.792994430639317\\
195	0.825650830109162\\
194	0.697016693378371\\
193	0.641000376859878\\
192	0.65719869363141\\
191	0.739798524893423\\
190	0.874135654419626\\
189	0.832583522357281\\
188	0.815165473791638\\
187	0.912045158653902\\
186	1.1207482562293\\
185	1.19066939511496\\
184	1.02869839969671\\
183	0.906268661669735\\
182	0.861989660487906\\
181	1.0713853744289\\
180	0.990850369830322\\
179	1.02821105744474\\
178	1.22378927663756\\
177	1.10390225663501\\
176	0.844032290650045\\
175	1.08770304599463\\
174	1.26747674630298\\
173	1.25501280018871\\
172	1.3935965095739\\
171	1.08620327726282\\
170	1.1347623570381\\
169	0.936678302757237\\
168	1.07959004234183\\
167	1.01513312723233\\
166	1.15284308967008\\
165	0.873947418032991\\
164	0.824504044956786\\
163	0.974058272622491\\
162	1.34719908952954\\
161	0.898110148142623\\
160	1.34524883129097\\
159	1.90750600318094\\
158	1.07114429966214\\
157	0.863729672441255\\
156	1.11722613841409\\
155	1.00019026555158\\
154	1.15126538026159\\
153	1.83174098132586\\
152	1.64704124455888\\
151	1.43877594808873\\
150	1.74068875802191\\
149	1.52828257763468\\
148	1.32133303139828\\
147	1.86676753732965\\
146	2.00391723519297\\
145	1.03347825972974\\
144	1.82663186716198\\
143	1.41063997618843\\
142	1.05544021000897\\
141	1.55271867453623\\
140	1.46583700288237\\
139	0\\
138	0\\
137	0\\
136	0\\
135	0\\
134	0\\
133	0\\
132	0\\
131	0\\
130	0\\
129	0\\
128	0\\
127	0\\
126	0\\
125	0\\
124	3.7979114332302\\
123	3.87960179476478\\
122	4.45497596740949\\
121	4.36987106890164\\
120	4.65606158370432\\
119	3.5357060593758\\
118	2.75240140636768\\
117	2.98251959714356\\
116	2.66808227400377\\
115	2.1879735321378\\
114	1.79355450867631\\
113	1.25720607153798\\
112	1.20283319237928\\
111	1.10858443387138\\
110	1.49977986566794\\
109	1.71669187321031\\
108	1.80341406077464\\
107	1.86291857807177\\
106	2.07670018120052\\
105	2.11112187847696\\
104	2.00716565269214\\
103	0.98231270987125\\
102	1.65892331916306\\
101	2.10650316825747\\
100	2.03235113384204\\
99	2.42453505354283\\
98	1.78599266808304\\
97	2.23631507120695\\
96	2.03382349639198\\
95	1.93025498781644\\
94	2.36573947608895\\
93	1.82870418369984\\
92	2.27624995974424\\
91	2.6422660410292\\
90	2.42578905852025\\
89	2.28700163800522\\
88	2.17347778564289\\
87	2.51541449833075\\
86	2.70786234155837\\
85	2.82823131098942\\
84	2.85610491423512\\
83	2.8543548796135\\
82	3.09089852994019\\
81	4.10600948137952\\
80	3.6519928960888\\
79	4.67884137187822\\
78	5.12051883521911\\
77	6.43744084112951\\
76	6.75908023983159\\
75	5.42114279680186\\
74	5.09944034483951\\
73	6.09256739888683\\
72	5.55986840795034\\
71	5.98814947894452\\
70	5.84288094037184\\
69	6.0743557599464\\
68	5.60862130307437\\
67	6.17958073550687\\
66	5.37445872530706\\
65	5.99112262380984\\
64	5.73963083366173\\
63	4.93796146449603\\
62	4.44973581619326\\
61	4.34932181071744\\
60	4.6482177912105\\
59	4.4629637441724\\
58	4.64683087864006\\
57	4.16982395312346\\
56	3.50625386298651\\
55	3.8519160556382\\
54	4.08701378680818\\
53	4.25669408057778\\
52	4.4115363178369\\
51	4.05048121086369\\
50	4.42275041009397\\
49	3.89903046926691\\
48	4.88087402636014\\
47	5.6151516523509\\
46	6.22433167543461\\
45	5.85197236349651\\
44	6.18122648730843\\
43	5.47468295211377\\
42	5.50833667651974\\
41	5.62576127258868\\
40	6.03359200197573\\
39	5.57647086138866\\
38	5.35019324150255\\
37	5.91478755927936\\
36	4.7872124287787\\
35	6.08668048624471\\
34	5.38724944452037\\
33	5.53881947635574\\
32	4.62674621057525\\
31	4.44120855343778\\
30	4.64994649643354\\
29	5.08259060423628\\
28	4.71391324140634\\
27	3.69037579321674\\
26	3.79581598446414\\
25	4.08747597393821\\
24	3.51055062634885\\
23	3.86143338100682\\
22	3.15997862217013\\
21	4.10600301843302\\
20	3.08922935675173\\
19	4.12073869400317\\
18	4.45028803801152\\
17	4.24799925529896\\
16	3.92024285624993\\
15	4.43620724117063\\
14	4.51656058827179\\
13	4.28767951186412\\
12	4.29042098284197\\
11	3.49929629606529\\
10	3.57655712958649\\
9	3.63199446706548\\
8	3.68106583454294\\
7	3.56667131280925\\
6	3.89814440607272\\
5	4.84126097052638\\
4	5.03547772616698\\
3	3.80312781930672\\
2	0\\
1	0\\
}--cycle;
\addlegendentry{\lblMVAuncertainty{5}}


==> figures/SMC_arrays_only.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%


%

%  ---------- PA ----------
\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=mycolor2x, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
0.59765306122449	0.40234693877551\\
0.59765306122449	0.59765306122449\\
0.40234693877551	0.59765306122449\\
0.40234693877551	0.40234693877551\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=mycolor2x, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
0.59765306122449	0.40234693877551\\
0.59765306122449	0.59765306122449\\
0.40234693877551	0.59765306122449\\
0.40234693877551	0.40234693877551\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=mycolor2x, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
0.59765306122449	0.40234693877551\\
0.59765306122449	0.59765306122449\\
0.59765306122449	0.59765306122449\\
0.59765306122449	0.40234693877551\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=mycolor2x, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
0.40234693877551	0.40234693877551\\
0.40234693877551	0.59765306122449\\
0.40234693877551	0.59765306122449\\
0.40234693877551	0.40234693877551\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=mycolor2x, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
0.59765306122449	0.40234693877551\\
0.40234693877551	0.40234693877551\\
0.40234693877551	0.40234693877551\\
0.59765306122449	0.40234693877551\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=mycolor2x, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
0.59765306122449	0.59765306122449\\
0.40234693877551	0.59765306122449\\
0.40234693877551	0.59765306122449\\
0.59765306122449	0.59765306122449\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.576530612244898	0.545918367346939\\
0.576530612244898	0.576530612244898\\
0.545918367346939	0.576530612244898\\
0.545918367346939	0.545918367346939\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.535714285714286	0.545918367346939\\
0.535714285714286	0.576530612244898\\
0.505102040816327	0.576530612244898\\
0.505102040816327	0.545918367346939\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.494897959183674	0.545918367346939\\
0.494897959183674	0.576530612244898\\
0.464285714285714	0.576530612244898\\
0.464285714285714	0.545918367346939\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.454081632653061	0.545918367346939\\
0.454081632653061	0.576530612244898\\
0.423469387755102	0.576530612244898\\
0.423469387755102	0.545918367346939\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.576530612244898	0.505102040816327\\
0.576530612244898	0.535714285714286\\
0.545918367346939	0.535714285714286\\
0.545918367346939	0.505102040816327\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.535714285714286	0.505102040816327\\
0.535714285714286	0.535714285714286\\
0.505102040816327	0.535714285714286\\
0.505102040816327	0.505102040816327\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.494897959183673	0.505102040816327\\
0.494897959183673	0.535714285714286\\
0.464285714285714	0.535714285714286\\
0.464285714285714	0.505102040816327\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.454081632653061	0.505102040816327\\
0.454081632653061	0.535714285714286\\
0.423469387755102	0.535714285714286\\
0.423469387755102	0.505102040816327\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.576530612244898	0.464285714285714\\
0.576530612244898	0.494897959183673\\
0.545918367346939	0.494897959183673\\
0.545918367346939	0.464285714285714\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.535714285714286	0.464285714285714\\
0.535714285714286	0.494897959183673\\
0.505102040816327	0.494897959183673\\
0.505102040816327	0.464285714285714\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.494897959183673	0.464285714285714\\
0.494897959183673	0.494897959183673\\
0.464285714285714	0.494897959183673\\
0.464285714285714	0.464285714285714\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.454081632653061	0.464285714285714\\
0.454081632653061	0.494897959183673\\
0.423469387755102	0.494897959183673\\
0.423469387755102	0.464285714285714\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.576530612244898	0.423469387755102\\
0.576530612244898	0.454081632653061\\
0.545918367346939	0.454081632653061\\
0.545918367346939	0.423469387755102\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.535714285714286	0.423469387755102\\
0.535714285714286	0.454081632653061\\
0.505102040816327	0.454081632653061\\
0.505102040816327	0.423469387755102\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.494897959183673	0.423469387755102\\
0.494897959183673	0.454081632653061\\
0.464285714285714	0.454081632653061\\
0.464285714285714	0.423469387755102\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
0.454081632653061	0.423469387755102\\
0.454081632653061	0.454081632653061\\
0.423469387755102	0.454081632653061\\
0.423469387755102	0.423469387755102\\
}--cycle;




%  ---------- PM ----------
\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=mycolor2x, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.471726405034202	3.89448150707502\\
-0.394481507075018	4.0282735949658\\
-0.528273594965798	4.10551849292498\\
-0.605518492924982	3.9717264050342\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=mycolor2x, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.471726405034202	3.89448150707502\\
-0.394481507075018	4.0282735949658\\
-0.528273594965798	4.10551849292498\\
-0.605518492924982	3.9717264050342\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=mycolor2x, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.471726405034202	3.89448150707502\\
-0.394481507075018	4.0282735949658\\
-0.394481507075018	4.0282735949658\\
-0.471726405034202	3.89448150707502\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=mycolor2x, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.605518492924982	3.9717264050342\\
-0.528273594965798	4.10551849292498\\
-0.528273594965798	4.10551849292498\\
-0.605518492924982	3.9717264050342\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=mycolor2x, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.471726405034202	3.89448150707502\\
-0.605518492924982	3.9717264050342\\
-0.605518492924982	3.9717264050342\\
-0.471726405034202	3.89448150707502\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=mycolor2x, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.394481507075018	4.0282735949658\\
-0.528273594965798	4.10551849292498\\
-0.528273594965798	4.10551849292498\\
-0.394481507075018	4.0282735949658\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-0.438641431420261	3.99403126030062\\
-0.423335308971281	4.02054224204913\\
-0.449846290719785	4.03584836449811\\
-0.465152413168764	4.0093373827496\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-0.473989407084932	4.01443942356593\\
-0.458683284635952	4.04095040531443\\
-0.485194266384456	4.05625652776341\\
-0.500500388833435	4.02974554601491\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-0.509337382749603	4.03484758683124\\
-0.494031260300623	4.06135856857974\\
-0.520542242049127	4.07666469102872\\
-0.535848364498106	4.05015370928022\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-0.459049594685567	3.95868328463595\\
-0.443743472236588	3.98519426638446\\
-0.470254453985091	4.00050038883344\\
-0.48556057643407	3.97398940708493\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-0.494397570350238	3.97909144790126\\
-0.479091447901259	4.00560242964976\\
-0.505602429649762	4.02090855209874\\
-0.520908552098741	3.99439757035024\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-0.529745546014909	3.99949961116656\\
-0.51443942356593	4.02601059291507\\
-0.540950405314433	4.04131671536405\\
-0.556256527763412	4.01480573361554\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-0.479457757950873	3.92333530897128\\
-0.464151635501894	3.94984629071978\\
-0.490662617250397	3.96515241316876\\
-0.505968739699377	3.93864143142026\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-0.514805733615544	3.94374347223659\\
-0.499499611166565	3.97025445398509\\
-0.526010592915068	3.98556057643407\\
-0.541316715364048	3.95904959468557\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-0.550153709280215	3.96415163550189\\
-0.534847586831236	3.9906626172504\\
-0.561358568579739	4.00596873969938\\
-0.576664691028719	3.97945775795087\\
}--cycle;

\node[centered, align=center, inner sep=0,color=mycolor2x]
at (axis cs:0.92,0.77) {$\scriptstyle \Delta\phi^{(j)}$};

\addplot [color=mycolor2x, line width=0.501pt, forget plot]
  table[row sep=crcr]{%
0.5001	0.5001\\
0.7501	0.5001\\
};










% arc:
\addplot [color=mycolor2x, line width=0.401pt, forget plot]
  table[row sep=crcr]{%
0.724926533154163	0.50893345854579\\
0.724406400089954	0.517753296538765\\
0.723540402814858	0.526545914428013\\
0.722329876633906	0.535297754634052\\
0.720776688090727	0.543995322453629\\
0.718883232089477	0.552625206867579\\
0.716652428202071	0.561174101219642\\
0.71408771616641	0.569628823734363\\
0.711193050582559	0.577976337842436\\
0.707972894815039	0.586203772282145\\
0.704432214110643	0.594298440945921\\
0.700576467942383	0.602247862441398\\
0.696411601591379	0.610039779336815\\
0.691944036979671	0.617662177061089\\
0.687180662768073	0.62510330242941\\
0.682128823734363	0.632351681765806\\
0.676796309448168	0.639396138594713\\
0.671191342260007	0.646225810874291\\
0.665322564623029	0.652830167744912\\
0.659199025766973	0.659199025766973\\
0.652830167744912	0.665322564623029\\
0.646225810874291	0.671191342260007\\
0.639396138594713	0.676796309448168\\
0.632351681765806	0.682128823734363\\
0.62510330242941	0.687180662768073\\
0.617662177061089	0.691944036979671\\
0.610039779336815	0.696411601591379\\
0.602247862441398	0.700576467942383\\
0.594298440945921	0.704432214110643\\
0.586203772282145	0.707972894815039\\
0.577976337842436	0.711193050582559\\
0.569628823734363	0.71408771616641\\
0.561174101219642	0.716652428202071\\
0.552625206867579	0.718883232089477\\
0.543995322453629	0.720776688090727\\
0.535297754634052	0.722329876633906\\
0.526545914428013	0.723540402814858\\
0.517753296538765	0.724406400089954\\
0.50893345854579	0.724926533154163\\
nan	nan\\
};

\addplot [color=mycolor2x, line width=0.501pt, forget plot]
  table[row sep=crcr]{%
-0.4999	4.0001\\
-0.2499	4.0001\\
};


% arc:
\addplot [color=mycolor2x, line width=0.401pt, forget plot]
  table[row sep=crcr]{%
-0.2749771018805	4.00598981336927\\
-0.275208354680221	4.01187559015466\\
-0.275593599910046	4.01775329653877\\
-0.276132573542138	4.02361890423522\\
-0.276824906190893	4.02946839324951\\
-0.277670123366094	4.03529775463405\\
-0.27866764579811	4.04110299323573\\
-0.279816789834894	4.046880130434\\
-0.281116767910523	4.05262520686758\\
-0.28256668908496	4.05833428514807\\
-0.284165559654657	4.06400345255838\\
-0.28591228383359	4.06962882373436\\
-0.28780566450426	4.0752065433276\\
-0.28984440403813	4.08073278864769\\
-0.292027105184961	4.08620377228215\\
-0.294352272030415	4.09161574469205\\
-0.296818311021281	4.09696499678187\\
-0.299423532057617	4.1022478624414\\
-0.302166149651058	4.10746072105841\\
-0.305044284148501	4.1126\\
-0.308055963020329	4.11766217706109\\
-0.31119912221228	4.12264378287838\\
-0.314471607560046	4.12754140330809\\
-0.317871176265637	4.13235168176581\\
-0.321395498434472	4.13707132152696\\
-0.325042158672182	4.14169708798621\\
-0.328808657739993	4.14622581087429\\
-0.332692414267586	4.15065438643074\\
-0.336690766522235	4.15497977953109\\
-0.340800974233027	4.15919902576697\\
-0.345020220468905	4.16330923347776\\
-0.349345613569257	4.16730758573241\\
-0.353774189125709	4.17119134226001\\
-0.358302912013787	4.17495784132782\\
-0.362928678473038	4.17860450156553\\
-0.367648318234194	4.18212882373436\\
-0.372458596691913	4.18552839243995\\
-0.377356217121619	4.18880087778772\\
-0.382337822938911	4.19194403697967\\
nan	nan\\
};





\node[centered, align=center, inner sep=0,color=white]
at (axis cs:-0.148,4.131) {$\scriptstyle \mathbf{\Delta}\varphi_{n}$};
\node[centered, align=center, inner sep=0,color=mycolor2x]
at (axis cs:-0.15,4.135) {$\scriptstyle \Delta\varphi_{n}$};








\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-2.59765306122449	0.40234693877551\\
-2.59765306122449	0.59765306122449\\
-2.40234693877551	0.59765306122449\\
-2.40234693877551	0.40234693877551\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-2.59765306122449	0.40234693877551\\
-2.59765306122449	0.59765306122449\\
-2.40234693877551	0.59765306122449\\
-2.40234693877551	0.40234693877551\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-2.59765306122449	0.40234693877551\\
-2.59765306122449	0.59765306122449\\
-2.59765306122449	0.59765306122449\\
-2.59765306122449	0.40234693877551\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-2.40234693877551	0.40234693877551\\
-2.40234693877551	0.59765306122449\\
-2.40234693877551	0.59765306122449\\
-2.40234693877551	0.40234693877551\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-2.59765306122449	0.40234693877551\\
-2.40234693877551	0.40234693877551\\
-2.40234693877551	0.40234693877551\\
-2.59765306122449	0.40234693877551\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-2.59765306122449	0.59765306122449\\
-2.40234693877551	0.59765306122449\\
-2.40234693877551	0.59765306122449\\
-2.59765306122449	0.59765306122449\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.5765306122449	0.545918367346939\\
-2.5765306122449	0.576530612244898\\
-2.54591836734694	0.576530612244898\\
-2.54591836734694	0.545918367346939\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.53571428571429	0.545918367346939\\
-2.53571428571429	0.576530612244898\\
-2.50510204081633	0.576530612244898\\
-2.50510204081633	0.545918367346939\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.49489795918367	0.545918367346939\\
-2.49489795918367	0.576530612244898\\
-2.46428571428571	0.576530612244898\\
-2.46428571428571	0.545918367346939\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.45408163265306	0.545918367346939\\
-2.45408163265306	0.576530612244898\\
-2.4234693877551	0.576530612244898\\
-2.4234693877551	0.545918367346939\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.5765306122449	0.505102040816327\\
-2.5765306122449	0.535714285714286\\
-2.54591836734694	0.535714285714286\\
-2.54591836734694	0.505102040816327\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.53571428571429	0.505102040816327\\
-2.53571428571429	0.535714285714286\\
-2.50510204081633	0.535714285714286\\
-2.50510204081633	0.505102040816327\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.49489795918367	0.505102040816327\\
-2.49489795918367	0.535714285714286\\
-2.46428571428571	0.535714285714286\\
-2.46428571428571	0.505102040816327\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.45408163265306	0.505102040816327\\
-2.45408163265306	0.535714285714286\\
-2.4234693877551	0.535714285714286\\
-2.4234693877551	0.505102040816327\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.5765306122449	0.464285714285714\\
-2.5765306122449	0.494897959183673\\
-2.54591836734694	0.494897959183673\\
-2.54591836734694	0.464285714285714\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.53571428571429	0.464285714285714\\
-2.53571428571429	0.494897959183673\\
-2.50510204081633	0.494897959183673\\
-2.50510204081633	0.464285714285714\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.49489795918367	0.464285714285714\\
-2.49489795918367	0.494897959183673\\
-2.46428571428571	0.494897959183673\\
-2.46428571428571	0.464285714285714\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.45408163265306	0.464285714285714\\
-2.45408163265306	0.494897959183673\\
-2.4234693877551	0.494897959183673\\
-2.4234693877551	0.464285714285714\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.5765306122449	0.423469387755102\\
-2.5765306122449	0.454081632653061\\
-2.54591836734694	0.454081632653061\\
-2.54591836734694	0.423469387755102\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.53571428571429	0.423469387755102\\
-2.53571428571429	0.454081632653061\\
-2.50510204081633	0.454081632653061\\
-2.50510204081633	0.423469387755102\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.49489795918367	0.423469387755102\\
-2.49489795918367	0.454081632653061\\
-2.46428571428571	0.454081632653061\\
-2.46428571428571	0.423469387755102\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-2.45408163265306	0.423469387755102\\
-2.45408163265306	0.454081632653061\\
-2.4234693877551	0.454081632653061\\
-2.4234693877551	0.423469387755102\\
}--cycle;
%\addplot [color=mycolor2x, line width=0.601pt, forget plot]
\addplot[-stealth, color=mycolor2x, line width=0.501pt,%
{-Stealth[inset=0pt, scale=0.6, angle'=25]}
]
  table[row sep=crcr]{%
-2.4999	0.5001\\
-2.4999	0.7501\\
};

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
5.28180692279891	1.94262141306433\\
5.20826053589394	2.12355070986085\\
5.02733123909743	2.05000432295588\\
5.1008776260024	1.86907502615937\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
5.28180692279891	1.94262141306433\\
5.20826053589394	2.12355070986085\\
5.02733123909743	2.05000432295588\\
5.1008776260024	1.86907502615937\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
5.28180692279891	1.94262141306433\\
5.20826053589394	2.12355070986085\\
5.20826053589394	2.12355070986085\\
5.28180692279891	1.94262141306433\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
5.1008776260024	1.86907502615937\\
5.02733123909743	2.05000432295588\\
5.02733123909743	2.05000432295588\\
5.1008776260024	1.86907502615937\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
5.28180692279891	1.94262141306433\\
5.1008776260024	1.86907502615937\\
5.1008776260024	1.86907502615937\\
5.28180692279891	1.94262141306433\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
5.20826053589394	2.12355070986085\\
5.02733123909743	2.05000432295588\\
5.02733123909743	2.05000432295588\\
5.20826053589394	2.12355070986085\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.20817467054595	2.06767022105982\\
5.19664702369564	2.09602904500912\\
5.16828819974635	2.08450139815881\\
5.17981584659665	2.05614257420951\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.17036290528022	2.05230002525941\\
5.15883525842991	2.08065884920871\\
5.13047643448062	2.0691312023584\\
5.14200408133093	2.0407723784091\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.13255114001449	2.036929829459\\
5.12102349316418	2.0652886534083\\
5.09266466921489	2.05376100655799\\
5.1041923160652	2.02540218260869\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.09473937474876	2.02155963365859\\
5.08321172789845	2.04991845760789\\
5.05485290394916	2.03839081075758\\
5.06638055079947	2.01003198680828\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.22354486634636	2.02985845579409\\
5.21201721949605	2.05821727974339\\
5.18365839554676	2.04668963289308\\
5.19518604239707	2.01833080894379\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.18573310108063	2.01448825999368\\
5.17420545423032	2.04284708394298\\
5.14584663028103	2.03131943709267\\
5.15737427713134	2.00296061314338\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.1479213358149	1.99911806419327\\
5.13639368896459	2.02747688814257\\
5.1080348650153	2.01594924129226\\
5.11956251186561	1.98759041734296\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.11010957054917	1.98374786839286\\
5.09858192369887	2.01210669234216\\
5.07022309974957	2.00057904549185\\
5.08175074659988	1.97222022154255\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.23891506214677	1.99204669052836\\
5.22738741529646	2.02040551447766\\
5.19902859134717	2.00887786762735\\
5.21055623819748	1.98051904367806\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.20110329688104	1.97667649472795\\
5.18957565003074	2.00503531867725\\
5.16121682608144	1.99350767182694\\
5.17274447293175	1.96514884787765\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.16329153161531	1.96130629892754\\
5.15176388476501	1.98966512287684\\
5.12340506081571	1.97813747602653\\
5.13493270766602	1.94977865207723\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.12547976634959	1.94593610312713\\
5.11395211949928	1.97429492707643\\
5.08559329554998	1.96276728022612\\
5.09712094240029	1.93440845627682\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.25428525794718	1.95423492526264\\
5.24275761109688	1.98259374921193\\
5.21439878714758	1.97106610236162\\
5.22592643399789	1.94270727841233\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.21647349268145	1.93886472946223\\
5.20494584583115	1.96722355341152\\
5.17658702188185	1.95569590656121\\
5.18811466873216	1.92733708261192\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.17866172741573	1.92349453366181\\
5.16713408056542	1.95185335761111\\
5.13877525661612	1.9403257107608\\
5.15030290346643	1.91196688681151\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
5.14084996215	1.9081243378614\\
5.12932231529969	1.9364831618107\\
5.10096349135039	1.92495551496039\\
5.1124911382007	1.89659669101109\\
}--cycle;
%\addplot [color=mycolor2x, line width=0.601pt, forget plot]
\addplot[-stealth, color=mycolor2x, line width=0.501pt,%
{-Stealth[inset=0pt, scale=0.6, angle'=25]}
]
  table[row sep=crcr]{%
5.15466908094817	1.99641286801011\\
5.06052663167065	2.2280099302627\\
};

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
1.99734104438074	4.3771340715074\\
1.87540021922338	4.4719893939877\\
1.97025554170368	4.59393021914506\\
2.09219636686104	4.49907489666476\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
1.99734104438074	4.3771340715074\\
1.87540021922338	4.4719893939877\\
1.97025554170368	4.59393021914506\\
2.09219636686104	4.49907489666476\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
1.99734104438074	4.3771340715074\\
1.87540021922338	4.4719893939877\\
1.87540021922338	4.4719893939877\\
1.99734104438074	4.3771340715074\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
2.09219636686104	4.49907489666476\\
1.97025554170368	4.59393021914506\\
1.97025554170368	4.59393021914506\\
2.09219636686104	4.49907489666476\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
1.99734104438074	4.3771340715074\\
2.09219636686104	4.49907489666476\\
2.09219636686104	4.49907489666476\\
1.99734104438074	4.3771340715074\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
1.87540021922338	4.4719893939877\\
1.97025554170368	4.59393021914506\\
1.97025554170368	4.59393021914506\\
1.87540021922338	4.4719893939877\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
1.92920408323144	4.45689699128629\\
1.90504143623857	4.47569262982268\\
1.92383707477496	4.49985527681555\\
1.94799972176783	4.48105963827916\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
1.95426493461329	4.48911385394345\\
1.93010228762042	4.50790949247984\\
1.94889792615681	4.53207213947271\\
1.97306057314968	4.51327650093632\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
1.97932578599514	4.52133071660061\\
1.95516313900227	4.540126355137\\
1.97395877753866	4.56428900212987\\
1.99812142453153	4.54549336359348\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
1.9614209458886	4.43183613990444\\
1.93725829889573	4.45063177844083\\
1.95605393743212	4.4747944254337\\
1.98021658442499	4.45599878689731\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
1.98648179727045	4.4640530025616\\
1.96231915027758	4.48284864109799\\
1.98111478881397	4.50701128809086\\
2.00527743580684	4.48821564955447\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
2.0115426486523	4.49626986521876\\
1.98738000165943	4.51506550375515\\
2.00617564019582	4.53922815074802\\
2.03033828718869	4.52043251221163\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
1.99363780854576	4.40677528852259\\
1.96947516155289	4.42557092705898\\
1.98827080008928	4.44973357405185\\
2.01243344708215	4.43093793551546\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
2.01869865992761	4.43899215117975\\
1.99453601293474	4.45778778971614\\
2.01333165147113	4.48195043670901\\
2.037494298464	4.46315479817262\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
2.04375951130946	4.47120901383691\\
2.01959686431659	4.4900046523733\\
2.03839250285298	4.51416729936617\\
2.06255514984585	4.49537166082978\\
}--cycle;
%\addplot [color=mycolor2x, line width=0.601pt, forget plot]
\addplot[-stealth, color=mycolor2x, line width=0.501pt,%
{-Stealth[inset=0pt, scale=0.6, angle'=25]}
]
  table[row sep=crcr]{%
1.98389829304221	4.48563214532623\\
1.7865700092671	4.63912986004006\\
};

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-3.99734104438074	4.3771340715074\\
-3.87540021922338	4.4719893939877\\
-3.97025554170368	4.5939302191450\\
-4.09219636686104	4.49907489666476\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-3.99734104438074	4.3771340715074\\
-3.87540021922338	4.4719893939877\\
-3.97025554170368	4.59393021914506\\
-4.09219636686104	4.49907489666476\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-3.99734104438074	4.3771340715074\\
-3.87540021922338	4.4719893939877\\
-3.87540021922338	4.4719893939877\\
-3.99734104438074	4.3771340715074\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-4.09219636686104	4.49907489666476\\
-3.97025554170368	4.59393021914506\\
-3.97025554170368	4.59393021914506\\
-4.09219636686104	4.49907489666476\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-3.99734104438074	4.3771340715074\\
-4.09219636686104	4.49907489666476\\
-4.09219636686104	4.49907489666476\\
-3.99734104438074	4.3771340715074\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor1x, fill=white!20!black, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-3.87540021922338	4.4719893939877\\
-3.97025554170368	4.59393021914506\\
-3.97025554170368	4.59393021914506\\
-3.87540021922338	4.4719893939877\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-3.92920408323144	4.45689699128629\\
-3.90504143623857	4.47569262982268\\
-3.92383707477496	4.49985527681555\\
-3.94799972176783	4.48105963827916\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-3.95426493461329	4.48911385394345\\
-3.93010228762042	4.50790949247984\\
-3.94889792615681	4.53207213947271\\
-3.97306057314968	4.51327650093632\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-3.97932578599514	4.52133071660061\\
-3.95516313900227	4.540126355137\\
-3.97395877753866	4.56428900212987\\
-3.99812142453153	4.54549336359348\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-3.9614209458886	4.43183613990444\\
-3.93725829889573	4.45063177844083\\
-3.95605393743212	4.4747944254337\\
-3.98021658442499	4.45599878689731\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-3.98648179727045	4.4640530025616\\
-3.96231915027758	4.48284864109799\\
-3.98111478881397	4.50701128809086\\
-4.00527743580684	4.48821564955447\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-4.0115426486523	4.49626986521876\\
-3.98738000165943	4.51506550375515\\
-4.00617564019582	4.53922815074802\\
-4.03033828718869	4.52043251221163\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-3.99363780854576	4.40677528852259\\
-3.96947516155289	4.42557092705898\\
-3.98827080008928	4.44973357405185\\
-4.01243344708215	4.43093793551546\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-4.01869865992761	4.43899215117975\\
-3.99453601293474	4.45778778971614\\
-4.01333165147113	4.48195043670901\\
-4.037494298464	4.46315479817262\\
}--cycle;

\addplot[area legend, line width=0.201pt, draw=mycolor3x, fill=white!50!mycolor3x, forget plot]
table[row sep=crcr] {%
x	y\\
-4.04375951130946	4.47120901383691\\
-4.01959686431659	4.4900046523733\\
-4.03839250285298	4.51416729936617\\
-4.06255514984585	4.49537166082978\\
}--cycle;


%\addplot [color=mycolor2x, line width=0.601pt, forget plot]
%  table[row sep=crcr]{%
%-3.98369829304221	4.48563214532623\\
%-3.7863700092671	4.63912986004006\\
%};
%\addplot [color=black, only marks, mark=o, mark options={solid, black}, forget plot]
%  table[row sep=crcr]{%
%0	0\\
%};


\addplot[-stealth, color=black, line width=0.601pt,%
{-Stealth[inset=0pt, scale=1.05, angle'=25]}
]
  table[row sep=crcr]{%
0.05	0\\
0.4	0\\
};
\node[centered, align=center, inner sep=0]
at (axis cs:-0.1,0.4) {$\scriptstyle y$};

\addplot[-stealth, color=black, line width=0.601pt,%
{-Stealth[inset=0pt, scale=1.05, angle'=25]}
]
  table[row sep=crcr]{%
0	0.05\\
0	0.4\\
};
\node[centered, align=center, inner sep=0]
at (axis cs:0.4,-0.1) {$\scriptstyle x$};

\addplot [color=black, forget plot]
  table[row sep=crcr]{%
-1	-50\\
-1	50\\
};

%\addplot [color=mycolor2x, line width=0.601pt, forget plot]
\addplot[-stealth, color=mycolor2x, line width=0.501pt,%
{-Stealth[inset=0pt, scale=0.6, angle'=25]}
]
  table[row sep=crcr]{%
-3.98369829304221	4.48563214532623\\
-3.7863700092671	4.63912986004006\\
};

















\node[centered, align=center, inner sep=0,color=mycolor4x]
(aoa) at (axis cs:0.3,4.3) {$\scriptstyle \aoa{s}{s'\!\!}$};
\node[centered, align=center, inner sep=0,color=mycolor4x]
(aod) at (axis cs:0.254,1.25) {$\scriptstyle \aod{s}{s'\!\!}$};

\node [above, align=center, inner sep=0,color=mycolor4x]
at ([xshift=0,yshift=3mm]aoa) {\footnotesize AoA};
\node [above, align=center, inner sep=0,color=mycolor4x]
at ([xshift=0,yshift=3mm]aod) {\footnotesize AoD};

\addplot [color=mycolor4x, line width=0.401pt, forget plot]
  table[row sep=crcr]{%
0.487966068394054	1.07497195765995\\
0.475837540812444	1.07458788766533\\
0.463719818872747	1.07394796106734\\
0.451618299380086	1.07305246286669\\
0.439538371923589	1.07190179188661\\
0.427485416476052	1.0704964605953\\
0.415464800997894	1.06883709487765\\
0.403481879046452	1.06692443375653\\
0.391541987391699	1.06475932906358\\
0.379650443639436	1.06234274505995\\
0.367812543863014	1.05967575800673\\
0.356033560244656	1.05675955568572\\
0.344318738727407	1.05359543687037\\
0.332673296678783	1.05018481074739\\
0.321102420567133	1.04652919628912\\
0.309611263651776	1.04263022157706\\
0.298204943687916	1.03848962307676\\
0.286888540647377	1.03410924486447\\
0.275667094456164	1.02949103780585\\
0.264545602749856	1.02463705868711\\
0.253529018647838	1.01954946929902\\
0.242622248547354	1.0142305354741\\
0.231830149938372	1.00868262607753\\
0.221157529240233	1.00290821195207\\
0.210609139661035	0.996909864817724\\
0.200189679080728	0.990690256126331\\
0.189903787958841	0.984252155871805\\
0.179756047267789	0.977598431356484\\
0.169750976452663	0.970732045914131\\
0.159893031418437	0.963656057590172\\
0.150186602545458	0.956373617779748\\
0.140636012734133	0.948887969824197\\
0.131245515479655	0.941202447566584\\
0.122019292977651	0.933320473866923\\
0.112961454261579	0.925245559077759\\
0.104076033372707	0.916981299480782\\
0.0953669875634993	0.908531375685164\\
0.0868381955351897	0.899899550988353\\
0.0784934557103491	0.89108966970003\\
nan	nan\\
};
\addplot [color=mycolor4x, line width=0.601pt, forget plot]
  table[row sep=crcr]{%
0.5001	0.7751\\
0.5001	1.1001\\
};


\addplot [color=mycolor4x, line width=0.401pt, forget plot]
  table[row sep=crcr]{%
-0.19530032516557	4.48779256513787\\
-0.178567242064614	4.47693357545127\\
-0.162220889293616	4.4655007071251\\
-0.146280940011457	4.45350771984255\\
-0.13076657826238	4.44096904740101\\
-0.115696475887617	4.42789978034079\\
-0.101088770053454	4.41431564778328\\
-0.0869610414227947	4.40023299850071\\
-0.0733302929964841	4.38566878124005\\
-0.0602129296498621	4.37064052432482\\
-0.0476247383891706	4.35516631455949\\
-0.0355808693515789	4.33926477546157\\
-0.0240958175716951	4.32295504484789\\
-0.013183405536504	4.30625675180185\\
-0.00285676654973132	4.2891899930494\\
0.00687167107434717	4.27177530877228\\
0.0159901989686279	4.25403365788747\\
0.0244878428044305	4.23598639282272\\
0.0323543754993203	4.21765523381851\\
0.0395803295256032	4.19906224278729\\
0.0461570083046833	4.1802297967615\\
0.0520764966735667	4.16118056096244\\
0.0573316704109177	4.14193746152219\\
0.0619162048111988	4.12252365789152\\
0.0658245822965796	4.10296251496712\\
0.0690520990574511	4.08327757497138\\
0.0715948707135532	4.06349252911897\\
0.073449836988903	4.04363118910389\\
0.074614765394898	4.0237174584417\\
0.0750882539171599	4.00377530370113\\
0.0748697327028869	3.98382872565987\\
0.0739594647466826	3.96390173041911\\
0.0723585455740369	3.94401830051177\\
0.0700689019228391	3.92420236603903\\
0.0670932894245117	3.90447777586998\\
0.0634352892875522	3.88486826893902\\
0.0590993039874784	3.86539744567561\\
0.0540905519683627	3.84608873960067\\
0.0484150613623301	3.82696538912388\\
nan	nan\\
};
\addplot [color=mycolor4x, line width=0.601pt, forget plot]
  table[row sep=crcr]{%
-0.3624	4.23825698604072\\
-0.1999	4.51971524227066\\
};








\addplot[-stealth, color=mycolor2x, line width=0.501pt,%
{-Stealth[inset=0pt, scale=0.6, angle'=25]}
]
  table[row sep=crcr]{%
0.5001	0.5001\\
0.5001	0.7501\\
};
\addplot[-stealth, color=mycolor2x, line width=0.501pt,%
{-Stealth[inset=0pt, scale=0.6, angle'=25]}
]
  table[row sep=crcr]{%
-0.4999	4.0001\\
-0.3749	4.21660635094611\\
};

